DreamWaQ++: Obstacle-Aware Quadrupedal Locomotion With Resilient Multi-Modal Reinforcement Learning

Quadrupedal robots hold promising potential for applications in navigating cluttered environments with resilience akin to their animal counterparts. However, their floating base configuration makes them vulnerable to real-world uncertainties, yielding substantial challenges in their locomotion control. Deep reinforcement learning has become one of the plausible alternatives for realizing a robust locomotion controller. However, the approaches that rely solely on proprioception sacrifice collision-free locomotion because they require front-feet contact to detect the presence of stairs to adapt the locomotion gait. Meanwhile, incorporating exteroception necessitates a precisely modeled map observed by exteroceptive sensors over a period of time. Therefore, this work proposes a novel method to fuse proprioception and exteroception featuring a resilient multi-modal reinforcement learning. The proposed method yields a controller that showcases agile locomotion performance on a quadrupedal robot over a myriad of real-world courses, including rough terrains, steep slopes, and high-rise stairs, while retaining its robustness against out-of-distribution situations.

==> TRO-Dreamwaqpp-arxiv/accept/ablation.tex <==
\section{Ablation Study}\label{section:ablation}
\input{\MainPath/ablation/encoding}
\input{\MainPath/ablation/embedding_analyis}
\input{\MainPath/ablation/latent_modulation}
\input{\MainPath/ablation/correlation}
\input{\MainPath/ablation/failure}
\input{\MainPath/ablation/reconstruction}
\input{\MainPath/ablation/estimation}

==> TRO-Dreamwaqpp-arxiv/accept/ablation/correlation.tex <==
\subsection{Cross-Modal Feature Correlation}
    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/ablation_heatmap_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{Cross-modal feature correlations between proprioceptive and exteroceptive context vectors. The heatmap shows the correlation between the embedding features, where low correlation indicates substantial mismatches between proprioceptive and exteroceptive information.}
        \label{figure:ablation_heatmap}
    \end{figure}

    Cross-modal correlations between context vectors are visualized as heatmap plots in Fig.~\ref{figure:ablation_heatmap}, obtained by computing cross-correlations between embedding features. Low cross-modal correlation on irregular terrains indicates substantial mismatches between proprioceptive and exteroceptive information. Additionally, stronger correlations are observed within the exteroceptive data due to its direct observability, as opposed to proprioception, which can only approximate the terrain beneath the robot. In contrast, higher cross-modal correlations on flat terrain result from the similar predictions of terrain structure provided by both proprioceptive and exteroceptive inputs.

    Additionally, it can be observed that cross-modal correlation is higher on high stairs than on low stairs. This is because, on high stairs, the robot’s feet are more likely to be in contact with the surface, providing more accurate proprioceptive information. In contrast, on low stairs, the robot’s feet are more often in the air, leading to less accurate proprioceptive feedback. This discrepancy between proprioceptive and exteroceptive information results in lower cross-modal correlation on low stairs compared to high stairs.


    % Cross-modal correlations between context vectors are visualized as heatmap plots in Fig.~\ref{figure:results_terrain}D, which was obtained by computing the cross-correlation between the embedding features. The low amount of cross-modal correlation on irregular terrains indicates that there are high mismatches between proprioceptive and exteroceptive information. Additionally, stronger cross-correlations are observed within the exteroceptive data due to its direct observability, unlike proprioception, which can only approximate the terrain beneath the robot. In contrast, increased cross-modal correlations on flat terrain can be attributed to the fact that, in such environments, both proprioceptive and exteroceptive inputs yield similar predictions of the terrain's structure~(extended results are presented in section~\ref{supp:embedding_analysis}).

==> TRO-Dreamwaqpp-arxiv/accept/ablation/embedding_analyis.tex <==
\subsection{Embedding Analysis}
    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/results_embedding_new_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{~Embedding visualization of the multi-modal context encoded by the proposed context encoder in different environments using PacMAP~\cite{wang2021understanding}. The highly disentangled multi-modal context serves as an informative prior for informing about the environment to the policy.}
        \label{figure:ablation_embedding}
    \end{figure}

    The visualized embeddings in Fig.~\ref{figure:ablation_embedding} reveal a distinctive ellipsoidal pattern in the proprioceptive context $\textbf{z}^\mathrm{p}_t$, attributed to the dynamic motion of the robot's feet, as $\textbf{z}^\mathrm{p}_t$ integrates various proprioceptive measurements. Notably, the ellipsoid’s size diminishes on more challenging terrains, likely reflecting the robot’s foot swing period. The controller adjusts by orchestrating quicker foot swings over difficult terrains, ensuring frequent ground contact to enhance locomotion stability.

    In contrast, the exteroceptive context $\textbf{z}^\mathrm{e}_t$ displays clearer inter-class separation among environments compared to $\textbf{z}^\mathrm{p}_t$. However, similarities among some embeddings likely result from simplified exteroceptive input, primarily 3D voxels ahead of the robot. The exteroceptive encoder effectively captures relevant geometric features, filtering out unnecessary details from raw 3D points.

    For the multi-modal context $\textbf{z}^\mathrm{pe}_t$, which fuses proprioceptive and exteroceptive inputs, Fig.~\ref{figure:ablation_embedding} displays distinct clusters based on terrain difficulty. Embeddings from \texttt{flat}, \texttt{easy stairs}, and \texttt{irregular} terrains are partially clustered near the origin due to similarities in obstacle height, despite differences in obstacle placement and density. However, significant disentanglement is evident within the \texttt{easy stairs} and \texttt{irregular} terrain clusters, facilitated by proprioceptive information capturing terrain properties under the robot.

    Simultaneously, the circular pattern from $\textbf{z}^\mathrm{p}_t$ persists in $\textbf{z}^\mathrm{pe}_t$, aiding in the correction of unreliable exteroceptive data. This feature contributes to the clear separation between \texttt{easy stairs} and \texttt{irregular} terrains, underscoring exteroception's auxiliary role in adapting the robot's gait to avoid upcoming obstacles.

    % The visualized embeddings in Fig.~\ref{figure:results_terrain}A show a distinctive ellipsoidal pattern from the proprioceptive context $\textbf{z}^\mathrm{p}_t$, that can be attributed to the dynamic motion of the robot's feet, as $\textbf{z}^\mathrm{p}_t$ is constructed through a mixture of proprioceptive measurements. Notably, the size of the ellipsoid tends to diminish when navigating more challenging terrains. We posit that the ellipsoid's radius resembles the robot's foot swing period. The controller tends to orchestrate more rapid foot swings as the robot traverses difficult terrains to ensure frequent foot contact with the ground and to promote locomotion stability. 

    % Meanwhile, the exteroceptive context $\textbf{z}^\mathrm{e}_t$, exhibits clearer inter-class distance among embeddings from different environments, compared with that of $\textbf{z}^\mathrm{p}_t$. However, a considerable amount of embeddings share similarities that likely arises from the simplified exteroceptive input, primarily consisting of 3D voxels in front of the robot. The exteroceptive encoder efficiently captures important geometric features by ignoring irrelevant details in raw 3D points.

    % Finally, we investigated the multi-modal context $\textbf{z}^\mathrm{pe}_t$, which is the fusion of proprioceptive and exteroceptive contexts. The plot in Fig.~\ref{figure:results_terrain}A shows discernible clusters that are dependent on the difficulty of the terrain. It is noteworthy that some portion of embeddings from the \texttt{flat}, \texttt{easy stairs}, and \texttt{irregular} terrains are clustered near the origin of the plot. This is because those terrains share similar properties in terms of obstacle height, but differ in terms of the placement and density of the obstacles. However, a large portion of the embeddings from \texttt{easy stairs} and \texttt{irregular} terrains have a clear disentanglement, which is attributed to the proprioceptive information that can capture small details of terrain under the robot.

    % Simultaneously, the circular pattern inherent to $\textbf{z}^\mathrm{p}_t$ remains discernible in $\textbf{z}^\mathrm{pe}_t$, which assists in correcting unreliable exteroceptive data. Thus, leading to a clear disentanglement between \texttt{easy stairs} and \texttt{irregular} terrains. This finding underscores the auxiliary nature of exteroception, altering the gait of the robot to avoid obstacles ahead of it.


==> TRO-Dreamwaqpp-arxiv/accept/ablation/encoding.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Ablation study on the impact of different architectures and regularization losses on the policy performance. The \protect\hlbest{best}, \protect\hlsecond{second best}, and \protect\hlworst{worst} performing methods for each test environment and metric are highlighted accordingly.}
    \label{table:ablation_encoding}
    \begin{tabular}{lccccccccc}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} 
        &\multicolumn{3}{c}{\textbf{Success rates}~$\textbf{[\%]}\uparrow$} 
        &\multicolumn{3}{c}{\textbf{Traveled distance}~$\textbf{[m]}\uparrow$} 
        &\multicolumn{3}{c}{\textbf{Calf collisions}~$\downarrow$} 
        \\ 
        
        &\multicolumn{1}{c}{Stairs-easy}
        &\multicolumn{1}{c}{Stairs-hard}
        &\multicolumn{1}{c}{Discrete}
        &\multicolumn{1}{c}{Stairs-easy}
        &\multicolumn{1}{c}{Stairs-hard}
        &\multicolumn{1}{c}{Discrete}
        &\multicolumn{1}{c}{Stairs-easy}
        &\multicolumn{1}{c}{Stairs-hard}
        &\multicolumn{1}{c}{Discrete} \\
        \hline\hline
        
        \textbf{Architecture} \\[0.1ex]
        \multicolumn{1}{l}{No memory}  
        & \alignedcell{white}{98.7} & \alignedcell{white}{85.1} & \alignedcell{second}{99.6} & \alignedcell{white}{8.4 \pm 1.2} & \alignedcell{white}{5.8 \pm 3.5} & \alignedcell{white}{11.5 \pm 0.9} & \alignedcell{worst}{30.1 \pm 0.8} & \alignedcell{worst}{35.2 \pm 10.2} & \alignedcell{worst}{27.4 \pm 20.1}  \\ 

        \multicolumn{1}{l}{Implicit memory}
        & \alignedcell{second}{99.1} & \alignedcell{white}{92.5} & \alignedcell{white}{99.5} & \alignedcell{white}{9.1 \pm 0.7} & \alignedcell{white}{8.8 \pm 1.3} & \alignedcell{white}{9.8 \pm 0.5} & \alignedcell{white}{24.1 \pm 5.1} & \alignedcell{white}{37.8 \pm 4.3} & \alignedcell{white}{15.9 \pm 2.7}  \\ 

        \multicolumn{1}{l}{No latent fusion}
        & \alignedcell{worst}{90.2} & \alignedcell{worst}{60.7} & \alignedcell{worst}{94.3} & \alignedcell{worst}{6.5 \pm 1.3} & \alignedcell{worst}{3.4 \pm 3.1} & \alignedcell{worst}{9.3 \pm 0.8} & \alignedcell{white}{22.3 \pm 2.1} & \alignedcell{white}{25.3 \pm 2.3} & \alignedcell{white}{13.5 \pm 2.6}  \\ 
        \midrule

        \textbf{Regularization} \\[0.1ex]
        \multicolumn{1}{l}{w/o contrastive loss}
        & \alignedcell{white}{98.4} & \alignedcell{second}{93.1} & \alignedcell{white}{99.2} & \alignedcell{second}{9.8 \pm 0.5} & \alignedcell{second}{8.9 \pm 1.4} & \alignedcell{white}{12.2 \pm 0.4} & \alignedcell{second}{12.3 \pm 1.8} & \alignedcell{second}{23.7 \pm 0.7} & \alignedcell{second}{8.4 \pm 0.9}  \\ 

        \multicolumn{1}{l}{w/o versatility gain}
        & \alignedcell{white}{98.2} & \alignedcell{white}{89.4} & \alignedcell{white}{99.3} & \alignedcell{white}{9.7 \pm 0.3} & \alignedcell{white}{8.8 \pm 1.5} & \alignedcell{second}{12.4 \pm 0.5} & \alignedcell{white}{15.2 \pm 0.5} & \alignedcell{white}{31.5 \pm 1.1} & \alignedcell{white}{11.3 \pm 1.4}  \\ 
        \midrule

        \multicolumn{1}{l}{DreamWaQ++}
        & \alignedcell{best}{99.5} & \alignedcell{best}{97.8} & \alignedcell{best}{99.8} & \alignedcell{best}{10.3 \pm 0.8} & \alignedcell{best}{9.5 \pm 1.2} & \alignedcell{best}{12.5 \pm 0.1} & \alignedcell{best}{10.5 \pm 0.4} & \alignedcell{best}{18.3 \pm 2.5} & \alignedcell{best}{5.8 \pm 0.2}  \\ 
        \bottomrule
    \end{tabular}
\end{table*}



\subsection{Quantitative Analysis on Policy Performance}
We evaluated the effectiveness of various multi-modal encoding strategies for learning a context representation that captures the dynamics of a quadrupedal robot. This ablation study examines the impact of various encoding methods on both policy performance and training dynamics. We trained several variants of the multi-modal context encoder, each using a different strategy as follows:

\begin{itemize}
    \item \textbf{No memory.} This variant does not use any memory structure; the encoder processes only the current proprioceptive and exteroceptive measurements.
    
    \item \textbf{Implicit memory.} This variant employs an LSTM to implicitly encode the history of proprioceptive and exteroceptive inputs without explicitly storing past information.
    
    \item \textbf{No latent fusion.} In this variant, proprioceptive and exteroceptive features are simply concatenated, with no dedicated fusion mechanism—treating them as separate input modalities.
    
    % \item \textbf{Latent fusion transformer.} This variant uses a transformer-based architecture to fuse proprioceptive and exteroceptive features.
    
    \item \textbf{DreamWaQ++ w/o contrastive loss.} This variant trains DreamWaQ++ without the contrastive loss which is used to align the latent representations of proprioceptive and exteroceptive features.
    
    \item \textbf{DreamWaQ++ w/o versatility gain.} This variant trains DreamWaQ++ without the versatility gain which encourages the policy to explore a wider range of actions and behaviors.
\end{itemize}

We evaluated all variants in a simulated environment using $1,\!000$ robots; each of the robots commanded to walk forward for $20~\textrm{s}$. The evaluations were conducted in three test environments: 
\begin{itemize}
    \item \textbf{Stairs-easy}. Continuous stairs with a step height of $10~\textrm{cm}$.
    \item \textbf{Stairs-hard}. Continuous stairs with a step height of $20~\textrm{cm}$.
    \item \textbf{Discrete}. Discrete obstacle terrain with obstacle heights ranging from $5~\textrm{cm}$ to $25~\textrm{cm}$.
\end{itemize}

For each variant, we report the average success rate, the average distance traveled, and the total number of calf collisions across the test environments. The results are summarized in Table~\ref{table:ablation_encoding}.

The results presented in Table~\ref{table:ablation_encoding} validate that DreamWaQ++ consistently outperforms all other variants across all test environments and evaluation metrics. Notably, we observed that the latent fusion mechanism plays a critical role: the variant without latent fusion exhibited the lowest success rates and shortest traveled distances despite not having the highest number of calf collisions. This suggests that latent fusion is crucial for maintaining robustness and stability, especially in situations where proprioceptive and exteroceptive inputs are inconsistent.

We also observed that the memory plays a significant role in collision avoidance. The variant without any memory structure resulted in the highest number of calf collisions across all environments. While the implicit memory variant performed worse than DreamWaQ++, it still achieved a reasonable level of performance, suggesting that even approximate temporal encoding can help improve safety.

Furthermore, in terms of regularization, the ablation study highlights the importance of both the contrastive loss and the versatility gain in DreamWaQ++. Removing the contrastive loss led to modest declines in all metrics, underscoring its value in aligning the latent spaces of proprioceptive and exteroceptive inputs, thereby improving policy learning. In contrast, removing the versatility gain resulted in more substantial performance degradation. This component encourages the policy to explore a broader range of behaviors. Without it, the policy tends to converge to a narrower action distribution, reducing adaptability and robustness in diverse terrains.






==> TRO-Dreamwaqpp-arxiv/accept/ablation/estimation.tex <==
\subsection{State Estimation Accuracy}
We evaluate the proprioceptive-based state estimation accuracy of DreamWaQ++ which utilizes an MLP-mixer architecture, and compare it with other common approaches such as fully connected networks~\cite{nahrendra2023dreamwaq} and RNN-based architectures~\cite{ji2022concurrent}. Since accurate state estimation is crucial for constructing the hierarchical exteroceptive memory, we also evaluate how different state estimation architectures impact the reconstruction quality for the exteroceptive input.

We conducted a controlled experiment in a simulated stair environment, where the robot traverses a staircase with step heights uniformly sampled from the range $[0.1,~0.3]~\textrm{m}$. To isolate perception performance, the robot was commanded to move forward at a constant speed of $0.5~\textrm{m/s}$. Subsequently, we measured the absolute reconstruction error across $187$ height points in the robot's surrounding area. The results are summarized in Table~\ref{table:state_estimation_accuracy}. All measurements represent the mean over $5~\textrm{s}$ of continuous walking using $1,\!000$ simulated robots.

\begin{table}[ht!]
    \centering
    \caption{State estimation and terrain reconstruction accuracy.}
    \label{table:state_estimation_accuracy}
    \begin{tabular}{lcccc}
        \toprule
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Architecture}}} 
        &\multicolumn{3}{c}{\textbf{Estimation error} $\downarrow$}
        &\multicolumn{1}{c}{\textbf{Reconstruction}} \\

        
        &\multicolumn{1}{c}{$v_x~\textrm{[m/s]}$}
        &\multicolumn{1}{c}{$v_y~\textrm{[m/s]}$}
        &\multicolumn{1}{c}{$v_z~\textrm{[m/s]}$}
        &\multicolumn{1}{c}{\textbf{error}~$\textrm{[m]}$ $\downarrow$} \\
        \midrule
        
        MLP         & $0.0571$ & $0.0739$ & $0.0715$ & $0.1978$ \\
        RNN         & $0.0497$ & $0.0613$ & $0.0514$ & $0.1253$ \\
        MLP-mixer   & $0.0363$ & $0.0331$ & $0.0385$ & $0.0674$ \\
        \bottomrule
    \end{tabular}
\end{table}

The results indicate that the MLP-mixer architecture outperforms both the fully connected MLP and RNN-based architectures in terms of state estimation accuracy, achieving the lowest error across all velocity components. This superior performance is attributed to the MLP-mixer's ability to effectively capture temporal dependencies and interactions among different proprioceptive modalities, resulting in a more accurate representation of the robot's state. Furthermore, the improved state estimation contributes to a more precise reconstruction of the surrounding terrain, as shown by the lowest reconstruction error among the evaluated architectures.


==> TRO-Dreamwaqpp-arxiv/accept/ablation/failure.tex <==
\subsection{Locomotion under Exteroception Failure}\label{supp:exteroception_failure}
    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/results_failures.png}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{Locomotion under exteroception failures. (a)~The robot swiftly adapts its gait when climbing the stairs under normal exteroception condition. Meanwhile, (b)~the robot's foot collides with the stairs and yield a foot-trapping reflex when white noise is provided as exteroception input. (c)~In an extreme failure case, the robot adapts to the detached camera by making contact with the ground using its feet and knees to ensure a stable pose.}
        \label{figure:supp_stairs_swing}
    \end{figure}

    Fig.~\ref{figure:supp_stairs_swing} shows the emergent behaviors of DreamWaQ++ when climbing stairs. This experiment ablates foot swing adaptation by providing the policy with a white noise input. The robot is commanded to climb the stairs under both conditions. The red arrows in Fig.~\ref{figure:supp_stairs_swing}(a) illustrate the foot swing motion of the robot when exteroception functions normally, allowing the robot to adapt its foot swing trajectory to climb two stairs at once. In contrast, when the robot receives white noise input, as in Fig.~\ref{figure:supp_stairs_swing}(b), the robot's foot tends to collide with the stairs. However, the robot adapts with a foot-trapping reflex, dragging its foot along the stair's vertical surface before placing it on the next step.

    Additionally, the experiment in Fig.~\ref{figure:supp_stairs_swing}(c) shows the robot climbing large rocks by swinging its feet extensively, resulting in strong vibrations. These vibrations eventually caused the camera to fall, yielding depth point cloud measurements with significant calibration error. The problem worsens when the camera becomes completely detached from the robot (see Fig.~\ref{figure:supp_stairs_swing}(c-4)). Under these conditions, the controller no longer receives new data streams. Interestingly, the robot adapts its gait to move by making contact with the ground using its feet and knees (Fig.~\ref{figure:supp_stairs_swing}(c-5)). This motion results in a more stable pose, with the robot adapting additional ground contacts to handle high-risk locomotion when exteroception becomes extremely unreliable.



    % Fig.~\ref{figure:supp_stairs_swing} shows the emergent behaviors of DreamWaQ++ when climbing stairs. This experiment ablates the foot swing adaptation by providing the policy with a white noise input. The robot is commanded to climb the stairs under both conditions. The red arrows in Fig.~\ref{figure:supp_stairs_swing}A illustrate the foot swing motion of the robot when the exteroception works normally, enabling the robot to adapt its foot swing trajectory to climb two stairs at once. In contrast, when the robot receives white noise input as in Fig.~\ref{figure:supp_stairs_swing}B, the robot's foot tens to collide with the stairs. However, the robot adapts with a foot-trapping reflex to climb the stairs by dragging its foot along the stair's vertical surface before placing it on the next step.

    % The experiment in Fig.~\ref{figure:supp_stairs_swing}(c) and \mvfive show the robot climbing large rocks by largely swinging its feet, resulting in strong vibrations. The vibrations eventually caused the camera to fall, yielding depth point cloud measurements with a large calibration error. The problem is exacerbated when the camera is completely detached from the robot (see Fig.~\ref{figure:supp_stairs_swing}(c-4)). In this condition, the controller does not receive new data streams. Interestingly, the robot adapts its gait to move by making contact with the ground with its feet and knees (Fig.~\ref{figure:supp_stairs_swing}(c-5)). This motion results in a more stable pose, owing to the additional contacts adapted by the robot to deal with high-risk locomotion when the exteroception is extremely unreliable. 

==> TRO-Dreamwaqpp-arxiv/accept/ablation/latent_modulation.tex <==
\subsection{Latent Modulation for Gait Control}
    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/results_modulation_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{(a)~Boxplots of the multi-modal contexts in an irregular terrain, showing the distribution of embeddings activation from the multi-modal context and highlighting the contrast between activations in the exteroceptive context. Latent modulation on some exteroceptive embedding proportionally affects the gait height. (b)~The robot exhibits different locomotion styles when particular latent variables ($41$, $42$, $55$, and $64$th embeddings) were scaled with (c)~$0.1$, (d)~$1.0$, and (e)~$3.0$ times of its original value.}
        \label{figure:ablation_gait}
    \end{figure}

    Fig.~\ref{figure:ablation_gait} illustrates the distribution of each latent feature as the robot traversed irregular terrains. Embedding indices from \texttt{1} to \texttt{32} correspond to $\textbf{z}^\mathrm{p}_t$, and indices from \texttt{33} to \texttt{64} correspond to $\textbf{z}^\mathrm{e}_t$. While $\textbf{z}^\mathrm{p}_t$ features display a uniform distribution, $\textbf{z}^\mathrm{e}_t$ contains four embeddings with distinct scaling differences compared to other exteroceptive features. This finding raises the question: \textit{Do these four exteroceptive embedding features correlate with the robot’s foot swing motion?}

    To address this question, we conducted an experiment by modulating these four $\textbf{z}^\mathrm{e}_t$ features. The results in Fig.~\ref{figure:ablation_gait}(b) indicate a clear trend: \textit{scaling up the latent feature decreases gait frequency while increasing gait height, and vice versa}. The resulting gait pattern resembles that used in stair-climbing scenarios, suggesting that the multi-modal context encoder effectively activates key latent variables that directly influence gait. A limitation of this approach is that the activated latent variables may vary across training seeds, as they are learned in an unsupervised manner with multiple randomizations. However, upon convergence, these critical latent features reliably emerge within the latent space.


    % Fig.~\ref{figure:ablation_gait} represents the distribution of each latent feature when the robot traversed irregular terrains. The embedding indices from \texttt{1} to \texttt{32} and from \texttt{33} to \texttt{64} correspond to $\textbf{z}^\mathrm{p}_t$ and $\textbf{z}^\mathrm{e}_t$, respectively. While the features of $\textbf{z}^\mathrm{p}_t$ show a similar distribution, the features of $\textbf{z}^\mathrm{e}_t$ exhibit four embeddings with distinct differences in scale compared with other exteroceptive embedding features. This finding raises a question: \textit{Do these four exteroceptive embedding features correlate with the foot swing motion of the robot?}

    % To address this question, we conducted an experiment in which we modulated the four features of $\textbf{z}^\mathrm{e}_t$. The results presented in Fig.~\ref{figure:ablation_gait}C reveal a notable trend: \textit{when the latent feature is modulated by scaling it up, the gait frequency decreases while the gait height increases, and conversely}. The gait pattern obtained by this latent scale-up is akin to that used in stair-climbing scenarios. This finding suggests that the multi-modal context encoder effectively activates critical latent variables that directly influence the gait pattern. A limitation of this property is that the activated latent variables may not be consistent over different training seeds due to the latent features are learned in an unsupervised manner with multiple randomization. However, upon convergence, these critical latent features will noticeably emerge among the latent features.

==> TRO-Dreamwaqpp-arxiv/accept/ablation/reconstruction.tex <==
\subsection{Terrain Reconstruction}\label{supp:recons}
    We decoded the latent features from the context encoder recorded during the asynchronous stair race experiment to reconstruct the terrain map, as shown in Fig.~\ref{figure:supp_recons}. The reconstructed terrain map resembles the ground truth terrain map constructed with~\cite{oh2024trip}.

    However, the reconstructed map is less accurate than the ground truth due to three factors:
    \begin{enumerate}
        \item The robot’s exteroception is limited to front-facing 3D points, and the encoder’s memory is not long-term.
        \item The encoder-decoder structure lacks residual connections, as in~\cite{hoeller2023anymal}, focusing the latent representation on relevant features.
        \item Variational autoencoder regularization in the latent space prioritizes feature disentanglement over precise reconstruction.
    \end{enumerate}
    Nonetheless, this slight reduction in reconstruction accuracy is acceptable, as the primary goal of the context encoder is to learn a structured representation for control rather than to fully reconstruct the terrain map.


    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/ablation_recons_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{(a)~An snapshot of the scene during the asynchronous stair race using DreamWaQ++. (b)~The terrain map is reconstructed from the recorded latent features and the ground truth terrain map is constructed using~\cite{oh2024trip}. The white points are the forward 3D scan input, while the reconstruction points surrounding the robots are colored based on the height relative to the robot's base.}
        \label{figure:supp_recons}
    \end{figure}

    We further evaluated the impact of the backbone sequence model on the controller's performance by comparing the controller’s performance across different sequence models. Performance was assessed by measuring the accuracy of future joint position predictions, as shown in Fig.~\ref{figure:supp_nextstate}.

    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/recons_error_models_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{Future state prediction error using different models and varying robot velocities. The MLP-mixer model used in DreamWaQ++ shows comparable performance to the Transformer model while being more lightweight and computationally efficient.}
        \label{figure:supp_nextstate}
    \end{figure}

    The results in Fig.~\ref{figure:supp_nextstate} show that the proposed MLP-mixer architecture performs comparably to the Transformer model. The MLP-mixer offers the advantage of being more lightweight and computationally efficient than the Transformer. As indicated by the curve, the prediction error increases with the robot's velocity due to the more dynamic nature of the motion, which requires higher accuracy in future state predictions.



==> TRO-Dreamwaqpp-arxiv/accept/ablation/reconstruction_origin.tex <==
\subsection{Terrain Reconstruction}\label{supp:recons}
    We decoded the latent features from the context encoder recorded in the asynchronous stair race experiment to reconstruct the terrain map. The reconstructed terrain map is shown in Fig.~\ref{figure:supp_recons} and \mvone0. The reconstructed terrain map resembles the ground truth terrain map constructed using~\cite{oh2024trip}.

    However, note that the reconstructed terrain map is not as accurate as the ground truth terrain map due to three reasons: 
    \begin{enumerate}
        \item The robot's exteroception is limited to the front-facing 3D points, and the memory retained by the encoder is not a long term memory.
        \item The encoder-decoder structure does not use a residual connection, similar to~\cite{hoeller2023anymal} to allow learning of only relevant features to the latent representation.
        \item The regularization in the latent space using a variational autoencoder is expected to reduce the reconstruction accuracy while improving disentanglement of the latent features. 
    \end{enumerate}
    Nevertheless, a slight reduction in the reconstruction accuracy is acceptable because the primary goal of the context encoder is to learn a structured representation that can be used for control, rather than to reconstruct the complete terrain map accurately.

    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/supp/supp_recons_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{\textbf{Reconstructed terrain map.} The terrain map is reconstructed from the latent features recorded during the asynchronous stair race using DreamWaQ++. The ground truth terrain map is constructed using~\cite{oh2024trip}. The white points are the forward 3D scan input, while the reconstruction points surrounding the robots are colored based on the height relative to the robot's base.}
        \label{figure:supp_recons}
    \end{figure}

    We further evaluate the impact of the backbone sequence model on the controller's performance. We compared the performance of the controller with and with different sequence models by measuring the accuracy of future joint position prediction. The results are shown in Fig.~\ref{figure:supp_nextstate}.

    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/recons_error_models_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{Future state prediction error using different models and varying robot velocities. The MLP-mixer model used in DreamWaQ++ shows comparable performance to the Transformer model while being more lightweight and computationally efficient.}
        \label{figure:supp_nextstate}
    \end{figure}

    The results in Fig.~\ref{figure:supp_nextstate} show that the proposed MLP-mixer architecture model works as well as the Transformer model. The advantage of using the MLP mixer is that it is more lightweight and computationally efficient than the Transformer model. From the curve, we can see that the prediction error increases as the robot's velocity increases. This is because the robot's motion becomes more dynamic and the model has to predict the future state more accurately.


==> TRO-Dreamwaqpp-arxiv/accept/acknowledgments.tex <==
\section*{Acknowledgments}
\paragraph{Funding:} 
\begin{enumerate}
    \item Korea Evaluation Institute of Industrial Technology~(KEIT) grant funded by the Korea Government~(MOTIE) (No. 20018216, ``Development of Mobile Intelligence SW for Autonomous Navigation of Legged Robots in Dynamic and Atypical Environments for Real Application''
    \item BK21 FOUR funded by the Ministry of Science and ICT, Republic of Korea.
\end{enumerate}


\paragraph{Author contributions:}
\begin{enumerate}
    \item Conceptualization: IMAN, HM
    \item Methodology: IMAN
    \item Software: IMAN, MO, SHL
    \item Validation: IMAN, MO, BY, DL, HWL, SHL
    \item Formal analysis: IMAN, HL
    \item Baseline reproduction: IMAN, DL, HWL, SHL:
    \item Investigation: IMAN, MO, BY, DL, HWL, SHL
    \item Resources: HM
    \item Data curation: IMAN, MO, SHL, DL
    \item Writing - original draft: IMAN
    \item Writing - review \& editing: IMAN, MO, BY, DL, SHL, HWL, HL, HM
    \item Visualization: IMAN, MO, HL, SHL
    \item Supervision: HM
    \item Project administration: IMAN, HM
    \item Funding acquisition: HM
    
\end{enumerate}

\paragraph{Competing interests:}The authors declare that they have no competing interests.

\paragraph{Data and materials availability:}All data needed to support the conclusions of this manuscript are included in the main text or Supplementary Materials.\ref{section:supp}


==> TRO-Dreamwaqpp-arxiv/accept/authors.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{figures/authors/Aswin.jpg}}]{I Made Aswin Nahrendra}
    received the B.S. and M.S. degrees in electrical engineering from Bandung Institute of Technology, Bandung, Indonesia, in 2018 and 2019, respectively. He received the Ph.D. degree in robotics program and electrical engineering from Korea Advanced Institute of Science and Technology (KAIST), Daejeon, Korea, in 2024. He was a postdoctoral fellow in the Information \& Electronics Research Institute, KAIST, Daejeon, Republic of Korea from 2024 to 2025. He is currently a research scientist in the Physical AI Team, AI Research Center at KRAFTON. His research interests include reinforcement learning, control, and robot learning for legged robots.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{figures/authors/bhyu.jpeg}}]{Byeongho Yu}
	received the M.S. and Ph.D. degrees in Electrical Engineering from Korea Advanced Institute of Science and Technology (KAIST), Daejeon, Korea, in 2021 and 2025, respectively. He is currently the CEO of URobotics. His research interests are primarily in the field robotics, including visual-inertial-leg odometry and state estimation for legged robots, with a particular focus on robust autonomy in unstructured environments.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{figures/authors/mhoh.JPG}}]{Minho Oh}
	received the B.S. degree in convergence engineering from Daegu Gyeongbuk Institute of Science and Technology (DGIST), Daegu, Korea, in 2020, and the M.S. degree in electrical engineering from the Korea Advanced Institute of Science and Technology (KAIST), Daejeon, Korea, in 2021. He is currently pursuing the Ph.D. degree in electrical engineering, KAIST, and leads the spatial intelligence team as the CTO of URobotics. His research interests include SLAM and terrain traversability mapping for enhanced autonomous navigation.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{figures/authors/dklee.jpeg}}]{Dongkyu Lee}
	received the B.S. degree in Electrical and Computer Engineering from the University of Seoul, Seoul, Korea, in 2021, and the M.S. degree in the Robotics Program from the Korea Advanced Institute of Science and Technology (KAIST), Daejeon, Korea, in 2023. He is currently pursuing the Ph.D. degree in Electrical Engineering at KAIST and is currently the CTO of URobotics Corp. His research interests include robot navigation, path planning, decision-making, and robot learning.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{figures/authors/shlee.JPG}}]{Seunghyun Lee}
	received the B.S. and M.S. degrees in the school of electrical engineering from Korea Advanced Institute of Science and Technology (KAIST), Daejeon, Republic of Korea, in 2022 and 2024, respectively. He is currently pursuing the Ph.D. degree at Urban Robotics Lab in the school of electrical engineering, KAIST. His research interests include legged robot locomotion and deep reinforcement learning.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{figures/authors/hwlee.jpeg}}]{Hyeonwoo Lee}
	received the B.S. and M.S. degrees in mechanical engineering from Yonsei University, Seoul, Republic of Korea, in 2020 and 2022, respectively. He is currently pursuing the Ph.D. degree in electrical engineering from the Korea Advanced Institute of Science and Technology with the Urban Robotics Lab. His research interests include reinforcement learning, motion and path planning for quadruped robots, and visual navigation.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.0in]{figures/authors/hyungtae.jpg}}]{Hyungtae Lim}
	received the B.S. degree in mechanical engineering, and M.S. and Ph.D. degrees in electrical engineering from the Korea Advanced Institute of Science and Technology (KAIST), Daejeon, Republic of Korea, in 2018, 2020, and 2023, respectively. He was a postdoctoral fellow in the Information \& Electronics Research Institute, KAIST, Daejeon, Republic of Korea from 2023 to 2024. He is currently a postdoctoral associate in the Laboratory for Information \& Decision Systems~(LIDS), Massachusetts Institute of Technology~(MIT), Cambridge, MA, USA.
    His research interests include SLAM (simultaneous localization and mapping), 3D registration, 3D perception, long-term map management, deep learning, and spatial AI.
\end{IEEEbiography}
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{figures/authors/mh.jpg}}]{Hyun Myung}
	received the B.S., M.S., and Ph.D. degrees in electrical engineering from the Korea Advanced Institute of Science and Technology (KAIST), Daejeon, Korea, in 1992, 1994, and 1998, respectively. He was a Senior Researcher with the Electronics and Telecommunications Research Institute, Daejeon, from 1998 to 2002, a CTO and the Director with the Digital Contents Research Laboratory, Emersys Corporation, Daejeon, from 2002 to 2003, and a Principle Researcher with the Samsung Advanced Institute of Technology, Yongin, Korea, from 2003 to 2008. Since 2008, he has been a Professor with the Department of Civil and Environmental Engineering, KAIST, and he was the Chief of the KAIST Robotics Program. From 2019, he is a Professor with the School of Electrical Engineering. His current research interests include autonomous robot navigation, SLAM (simultaneous localization and mapping), spatial AI/ML, and swarm robots.
\end{IEEEbiography}

==> TRO-Dreamwaqpp-arxiv/accept/control/problem.tex <==
\subsection{Problem Formulation}
The control problem is formulated in a partially observable Markov decision process~(POMDP) setting with a goal to maximize the expected discounted future rewards, which in turn resulting in a policy:

\begin{equation}
    \pi=\argmax_{\textbf{a}} E\left[\sum_{t=0}^{\infty}\gamma^t r_t\right],
    \label{eq:pi}
\end{equation}
where $\textbf{a}$, $\gamma$, and $r$ are the action, discount factor, and rewards, respectively. This objective is optimized using the proximal policy optimization (PPO)~\cite{schulman2017proximal} algorithm, while also taking into account the auxiliary objectives related to the perception pipeline.

We leveraged a privileged learning setting using an asymmetric actor-critic architecture, following~\cite{nahrendra2023dreamwaq}. The actor, i.e. the policy receives partial and noisy observations ($\textbf{o}^\mathrm{p}_t$), akin to the real-world observations and the multi-modal context ($\textbf{z}^\mathrm{pe}_t$) as its input. The policy network runs at a rate of $50~\mathrm{Hz}$, generating a target joint position that is tracked by a low-level PD controller, running at $200~\mathrm{Hz}$, to generate the joint torque commands. 

==> TRO-Dreamwaqpp-arxiv/accept/control/skill_discovery.tex <==
\subsection{Skill Discovery}\label{section:skill_discovery}

We incorporate an unsupervised RL objective through mutual information (MI) maximization for promoting skill discovery. This objective allows the emergence of novel behaviors while preserving stable behaviors induced by the handcrafted reward functions. Specifically, we maximize the MI between visited states and the latent variable inferred by the multi-modal context encoder. 

The MI objective is introduced as a regularization term in the PPO loss function. We call this objective as \textit{versatility gain}, which seeks to be maximized for inducing versatile locomotion behaviors. Thus, the versatility gain can balance exploration, exploitation, and reconstruction. The versatility gain is defined as:
\begin{equation}\label{eq:versatility_gain}
    \mathcal{G}_\textrm{versatility}=\mathcal{I}(\textbf{o}^\textrm{pe}_t;\textbf{z}^\textrm{pe}_t)=\mathcal{H}(\textbf{z}^\textrm{pe}_t)-\mathcal{H}(\textbf{z}^\textrm{pe}_t|\textbf{o}^\textrm{pe}_t),
\end{equation}
where $\mathcal{I}(\cdot;\cdot)$, $\mathcal{H}(\cdot)$, and $\mathcal{H}(\cdot|\cdot)$ are the mutual information, Shannon entropy, and conditional entropy operators, respectively. \eqref{eq:versatility_gain} comprises two terms that were essential for training. The first term maximizes the variation of the inferred latent variables, thus, promoting the variation of skills that can be obtained during policy learning. The second term minimizes the entropy of the latent states given an observation, thus, acting as a denoising operation to filter out noisy observations by clustering intrinsically similar observations into a similar latent representation.

Generally, the encoder is trained to minimize the KL divergence between $\textbf{z}^\textrm{pe}_t$ and $\textbf{o}^\textrm{pe}_t$, i.e. $\mathcal{L}_\textrm{encoder} \approx D_\textrm{KL}\left(\textbf{z}^\textrm{pe}_t | \textbf{o}^\textrm{pe}_t\right)$, effectively compressing raw observations while maintaining the original data distribution. Subsequently, jointly training the networks using $\mathcal{G}_\textrm{versatility}$ and $\mathcal{L}_\textrm{encoder}$ maximizes:

\begin{align}
    \mathcal{J} &\triangleq \mathcal{G}_\textrm{versatility} - \lambda_\mathrm{e} \mathcal{L}_\textrm{encoder} \nonumber \\ 
                &= \mathcal{I}(\textbf{o}^\textrm{pe}_t;\textbf{z}^\textrm{pe}_t) - \lambda_\textrm{e} D_\textrm{KL}\left(\textbf{z}^\textrm{pe}_t | \textbf{o}^\textrm{pe}_t\right) \nonumber \\
                &= \mathcal{H}(\textbf{z}^\textrm{pe}_t)-\mathcal{H}(\textbf{z}^\textrm{pe}_t|\textbf{o}^\textrm{pe}_t) + \lambda_\textrm{e} \left[ \mathcal{H}(\textbf{z}^\textrm{pe}_t,\textbf{o}^\textrm{pe}_t) - \mathcal{H}(\textbf{z}^\textrm{pe}_t)\right] \nonumber \\
                &= \mathcal{H}(\textbf{z}^\textrm{pe}_t)-\mathcal{H}(\textbf{z}^\textrm{pe}_t|\textbf{o}^\textrm{pe}_t) + \lambda_\textrm{e} \left[\mathcal{H}(\textbf{z}^\textrm{pe}_t|\textbf{o}^\textrm{pe}_t) + \mathcal{H}(\textbf{o}^\textrm{pe}_t) - \mathcal{H}(\textbf{z}^\textrm{pe}_t)\right] \nonumber \\
                &= \left(1 - \lambda_\textrm{e}\right) \mathcal{H}(\textbf{z}^\textrm{pe}_t) - \left(1 - \lambda_\textrm{e}\right) \mathcal{H}(\textbf{z}^\textrm{pe}_t|\textbf{o}^\textrm{pe}_t) + \lambda_\textrm{e} \mathcal{H}(\textbf{o}^\textrm{pe}_t), \label{eq:combined_objective}
\end{align} 
where $\mathcal{H}(\cdot,\cdot)$ is a cross-entropy operation and $\lambda_\textrm{e}\in\mathbb{R}^+$ is the scaling factor for $\mathcal{L}_\textrm{encoder}$. \eqref{eq:combined_objective} shows that choosing $\lambda_\textrm{e}=1$ leads to entropy maximization on the state visitation that subsequently promotes policy exploration and skill discovery during training. Furthermore, choosing $\lambda_\textrm{e}<1$ maximizes~$\mathcal{H}(\textbf{z}^\textrm{pe}_t)$ and minimizes~$\mathcal{H}(\textbf{z}^\textrm{pe}_t|\textbf{o}^\textrm{pe}_t)$, effectively diversifying the distribution of $\textbf{z}^\textrm{pe}_t$ while compressing $\textbf{o}^\textrm{pe}_t$. In practice, we set $\lambda_\textrm{e}=0.1$ for our experiments.

==> TRO-Dreamwaqpp-arxiv/accept/discussion.tex <==
\section{Conclusion}
    We have proposed DreamWaQ++, a resilient yet lightweight obstacle-aware locomotion controller that enhances the resilience of its precursor, DreamWaQ~\cite{nahrendra2023dreamwaq}. DreamWaQ++ reduces the need for expensive onboard computation and increases versatility by incorporating 3D point cloud data as an exteroceptive modality. Our experiments demonstrate that the proposed controller exhibits enhanced explainability, opening possibilities for integration with model-based counterparts or higher-level planning modules to enable greater autonomy. A promising avenue for future work involves integrating an active tilting mechanism into the camera mount using an additional servo motor. By simultaneously learning both locomotion and camera tilting, this approach could yield a controller that actively maximizes its observability, resembling the active sensing behavior of animals.


==> TRO-Dreamwaqpp-arxiv/accept/environment/adversarial_obs.tex <==
\subsection{Adversarial Observations}\label{section:adversarial}
    During training, we injected noise into the proprioceptive and exteroceptive observations to make the policy be robust against noisy real-world observations. For the proprioceptive observations, a uniform noise was injected at each time step. For the exteroceptive data, we defined three different noise ranges, constituting low, medium, and high noise levels. The proportion of robots that operate with these exteroceptive noise scales during training was set to $30\%$, $50\%$, and $20\%$, for the low, medium, and high noise levels, respectively.

    To handle erroneous extrinsic calibration between the exteroceptive sensor and the robot body frame, we also applied sensor alignment bias at the beginning of each episode to simulate extrinsic calibration error. This error encompasses biases in both the position and orientation of the sensor frame with respect to the robot body frame. The biases were sampled from a uniform distribution and consistently applied to the exteroceptive measurements throughout the episode. The ranges of the observation noises and sensor alignment biases are summarized in Table~\ref{table:observation_noise}.

    \begin{table}[t!]
    \centering
    % \captionsetup{justification=centering}
    \caption{Noise and sensor alignment bias parameters injected into the observation for the policy network during training.}
    \label{table:observation_noise}
    \begin{center}
    \begin{tabular}{lccc}
    \hline\hline
    Observation                        & Noise range ($\mu$) & Unit \\\hline
    Joint position  &                      $[-0.01, 0.01]$ & $\mathrm{rad}$     \\ 
    Joint velocity  &                      $[-1.5, 1.5]$ & $\mathrm{rad/s}$    \\ % $\mathrm{rad~s^{-1}}$    \\ 
    Body linear velocity &                 $[-0.1, 0.1]$ & $\mathrm{m/s}$   \\ % $\mathrm{m~s^{-1}}$   \\ 
    Body angular velocity &                $[-0.2, 0.2]$ & $\mathrm{rad/s}$   \\ 
    Gravity vector        &                $[-0.05, 0.05]$ & $\mathrm{m/s^{2}}$    \\ % $\mathrm{m~s^{-2}}$    \\
    Exteroceptive measurement (low)  &     $[0.0, 0.03]$ & $\mathrm{m}$\\
    Exteroceptive measurement (medium)  &     $[0.03, 0.1]$ & $\mathrm{m}$    \\
    Exteroceptive measurement (high)  &     $[0.1, 0.3]$ & $\mathrm{m}$    \\
    Exteroceptive bias roll             & $[-0.2, 0.2]$ &  $\mathrm{rad}$   \\
    Exteroceptive bias pitch           & $[-0.15, 0.15]$ &  $\mathrm{rad}$   \\
    Exteroceptive bias yaw              & $[-0.1, 0.1]$ &  $\mathrm{rad}$   \\
    Exteroceptive bias $\mathrm{x}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
    Exteroceptive bias $\mathrm{y}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
    Exteroceptive bias $\mathrm{z}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\


    \hline\hline
    \end{tabular}
    \end{center}
    \vspace{-0.cm}
    \end{table}

    

==> TRO-Dreamwaqpp-arxiv/accept/environment/curriculum.tex <==
\subsection{\textit{Curriculum}}
We leveraged three curricula during training, i.e., terrain, command, and reward curricula. For the terrain curriculum, various terrains were procedurally generated at the beginning of training to simulate obstacles the robot might encounter in real-world environments. The terrain curriculum utilized a game-inspired setting~\cite{rudin2021learning} with ten levels of difficulty. We primarily used terrains such as \texttt{rough}, \texttt{stairs}, \texttt{gaps}, and \texttt{discretized obstacle}, to introduce variation in exteroception, thereby increasing the diversity of training data for the multi-modal context encoder. An agent was promoted to the next level if it could traverse more than half the distance at the current level. If an agent failed to cover more than half the distance for ten consecutive episodes, it was demoted to the previous level. Agents that successfully completed all levels were randomly spawned within the ten levels, which prevented catastrophic forgetting and further diversified the training data.

The policy was trained to maximize command tracking rewards while satisfying style rewards (Table~\ref{table:reward_functions}), resulting in smooth and accurate robot motion. The curriculum followed a reward-based approach, automatically increasing the command velocity range when the velocity tracking reward, $r_{v_{x,y}} \in [0, 1]$, exceeded a set threshold, $r^\textrm{thres}_{v_{x,y}}$, which was defined as $0.9$.

Finally, the reward curriculum promotes safe behavior in real-world scenarios by gradually increasing the penalty for style rewards. Applying strong penalties to style rewards early in training can restrict exploration, leading to poor performance. However, without sufficient penalties, the robot may behave aggressively when noisy exteroceptive measurements are introduced in real-world settings. Therefore, a reward curriculum with exponentially increasing penalties over learning iterations was employed to facilitate stable learning. More details are provided in Section~\ref{supp:reward_functions}.


==> TRO-Dreamwaqpp-arxiv/accept/environment/domain_randomization.tex <==
\subsection{Domain Randomization}
    We randomized multiple physical properties of the robot and environment to facilitate sim-to-real transfer. Additionally, we employed Roll-Drop~\cite{campanaro2023roll} to encourage exploration and enhance robustness alongside physics randomization. Table~\ref{table:domain_randomization} summarizes the details of the physical properties and their randomization ranges.

    Additionally, we applied domain randomization to account for potential data asynchrony between proprioceptive and exteroceptive sensors caused by system delays. Such delays may arise from factors including data transmission latency, multithreaded execution on the robot, and hardware-induced timing jitter. These issues can violate the Markov property assumed in standard policy learning frameworks.

    To mitigate this, we randomly delay proprioceptive observations within a range of $[0, 15]~\mathrm{ms}$ during training. This strategy encourages the policy to treat minor mismatches between proprioceptive and exteroceptive inputs as observation noise, thereby increasing its robustness to sensor delays during deployment.

    While it is theoretically possible to extend the randomization range to further improve robustness, doing so can lead to overly conservative policies and degrade performance. Therefore, we set the maximum delay to $15~\mathrm{ms}$, which we found to be empirically appropriate given the computational constraints of our onboard hardware.


    \begin{table}[t!]
    \centering
    % \captionsetup{justification=centering}
    \caption{Domain randomization ranges applied in the simulation.}
    \label{table:domain_randomization}
    \begin{center}
    \begin{tabular}{lccc}
    \hline\hline
    Parameter                        & Randomization range & Unit \\\hline
    Payload                     & $[-1, 2]$ & $\mathrm{~kg}$     \\ 
    $K_p$ factor   & $[0.9, 1.1]$ & $\mathrm{~Nm~rad^{-1}}$    \\ 
    $K_d$ factor        & $[0.9, 1.1]$ & $\mathrm{~Nms~rad^{-1}}$   \\ 
    Motor strength factor        & $[0.9, 1.1]$ & $\mathrm{~Nm}$   \\ 
    Center of mass shift        & $[-50,50]$ & $\mathrm{~mm}$    \\
    Friction coefficient        & $[0.2, 1.25]$ & -    \\
    System delay                        & $[0.0, 15.0]$ &  $\mathrm{~ms}$   \\


    \hline\hline
    \end{tabular}
    \end{center}
    \vspace{-0.cm}
    \end{table}


==> TRO-Dreamwaqpp-arxiv/accept/environment/locomotion.tex <==
\subsection{Low-Level Control}
The policy and multi-modal context encoder networks run synchronously while processing asynchronous observations. Proprioceptive measurements are sampled at $200~\textrm{Hz}$, and exteroceptive measurements at $10~\textrm{Hz}$, with the controller integrating the latest measurements at $50~\textrm{Hz}$. To enhance robustness against asynchronous observations, latency randomization was applied during training. Detailed information on randomized latency for all measurements is available in Table~\ref{table:domain_randomization}.

The policy network generates target joint positions at $50~\textrm{Hz}$, which are then sent to a low-level proportional-derivative (PD) controller operating at $200~\textrm{Hz}$. Within the PD controller, target joint positions are converted into torque commands using proportional ($K_p$) and derivative ($K_d$) gains of $25$ and $0.7$, respectively. We made a custom interface using Pybind to access the Unitree SDK via our Python script that runs the RL policy and to send the target joint positions to the Unitree SDK using a ROS system. The Pybind interface then converts the target joint positions into torque commands, which are subsequently transmitted to the low-level motor controller.

==> TRO-Dreamwaqpp-arxiv/accept/environment/privileged.tex <==
\subsection{Privileged States}
    We utilized a robot-centric local height map as the privileged exteroception, sampled around the robot in a 2.5D grid where each cell represents terrain height. The grid dimensions are $w\!=\!1.1~\mathrm{m}$ by $h\!=\!1.7~\mathrm{m}$, with the first row positioned $0.9~\mathrm{m}$ ahead of the robot’s body frame, similar to the 3D voxel grid used for the multi-modal encoder input. The grid resolution is set to $5~\mathrm{cm}$.

    For privileged proprioception, we utilized ground-truth data and simulation measurements, including body-centric linear and angular velocities, gravity vector, joint positions and angular velocities, external disturbance forces and torques, foot positions relative to the robot's body frame, and physical properties of the robot. The physical properties include friction, motor damping, motor stiffness, motor strength ratio, additional payload, and the robot's center of mass shift.


==> TRO-Dreamwaqpp-arxiv/accept/environment/reward.tex <==
\subsection{Reward Functions}\label{training:reward_functions}
    We used the exact same rewards in~\cite{nahrendra2023dreamwaq}. On top of these rewards, we employed a reward curriculum to exponentially anneal some style rewards, i.e.~joint torque, joint velocity, joint acceleration, action rate, and smoothness rewards. We observed that although these style rewards are important to ensure sim-to-real transfer, they can lead to suboptimal policies that make the robot only learn basic locomotion skills. This is because the agent may become overly focused on maximizing immediate rewards induced by these joint-level regularization rewards. Therefore, we gradually annealed the weight of the regularization rewards to allow the agent to explore a wider range of behaviors and styles after it has learned the basic locomotion task. The annealing follows the following rule:

    \begin{equation}
        w_{i+1}=\lambda w_{i},
    \end{equation}
    where $w$ is the reward weight, $i$ is the learning iteration, and $\lambda$ is the annealing rate. We set $\lambda\!=0.998$
    and $w_0$ for the selected skill rewards are summarized in Table~\ref{table:reward_init}.
    % ===================================================================================

    % ===================================================================================
    \begin{table}[t!]
    % \begin{threeparttable}
    \centering
    \captionsetup{singlelinecheck=false}
    \caption{Initial weight $w_0$ for selected style rewards that were annealed using the reward curriculum.}
    \label{table:reward_init}

    \begin{center}
    \begin{tabular}{lll}
    \hline \hline
    Reward           & Weight ($w_0$)\\ \hline 
    Joint torque & $-5\!\times\!10^{-6}$ \\
    Joint velocity & $-6\!\times\!10^{-6}$ \\
    Joint acceleration & $-7.5\!\times\!10^{-8}$ \\
    Action rate & $-1.5\!\times\!10^{-5}$ \\
    Smoothness & $-1.5\!\times\!10^{-5}$ \\
    \hline \hline
    \end{tabular}
    \end{center}
    \end{table}
    % =================================================================================== 

==> TRO-Dreamwaqpp-arxiv/accept/environment/simulation.tex <==
\subsection{Simulation}
We utilized NVIDIA Isaac Gym Preview 3~\cite{makoviychuk2021isaac} as the simulator to train the controller and multi-modal context encoder networks, with training environments based on the Legged Gym library~\cite{rudin2021learning}. Domain randomization was applied across $3,\!500$ agents, completing training in approximately 11 hours on an NVIDIA A5000 GPU. The trained multi-modal context encoder and policy networks were then deployed without any fine-tuning on a physical robot or in the Gazebo simulator for the evaluations presented in this paper.


==> TRO-Dreamwaqpp-arxiv/accept/introduction.tex <==
\section{Introduction}
\noindent In the past decade, quadrupedal robots have revolutionized robotic applications in real-world environments thanks to their capability to traverse cluttered spaces, enabling diverse applications spanning exploration and inspection~\cite{gehring2021anymal,tranzatto2022cerberus,hong2022agile,arm2023scientific}. The growing interest in quadrupedal robot applications has been accompanied by advancements in control algorithms, which have evolved from traditional model-based control~\cite{jenelten2022tamols,bellicoso2017dynamic,gehring2017quadrupedal,bledt2018cheetah,hong2020real} to data-driven approaches such as deep reinforcement learning (RL)~\cite{lee2020learning,kumar2021rma,ji2022concurrent,nahrendra2023dreamwaq,choi2023learning,miki2022learning,gangapurwala2022rloc,yang2022learning,imai2022vision,agarwal2022legged,yang2023neural}.

Traditional model-based control pipelines for legged robots typically rely on a complex cascaded structure~\cite{jenelten2022tamols} that comprises accurate state estimation~\cite{bloesch2013state,camurri2020pronto,kim2021legged,kim2022step}, terrain mapping~\cite{fankhauser2018probabilistic,lim2021patchwork,lee2022patchwork++,oh2022travel,miki2022elevation}, and a whole-body controller optimizing the robot's foot trajectory~\cite{bellicoso2017dynamic,gehring2017quadrupedal,bledt2018cheetah,hong2020real}. However, these pipelines can be computationally intensive for real-time inference and often require strict assumptions, such as collision-free and non-slip conditions. Although simplified models are sometimes used to reduce problem complexity, they potentially aggravate the performance.

\begin{figure}[t!]
    \centering 
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=1.0\textwidth]{figures/reduced/main_red.pdf}
    \end{subfigure}
    % \captionsetup{font=footnotesize}
    \caption{The locomotion controller trained using DreamWaQ++ allows a quadrupedal robot to perform agile and resilient locomotion over various obstacles and terrains. The controller exhibits versatile gaits such as (a)~ascending and (b)~descending over a flight of stairs, (c)~performing a leap motion, (d)~probing when faced with an uncertain dip, (e)~crossing a gap, (f)~adapting to unseen deformable disastrous terrain, (g)~balancing on movable platforms, and~(h)~climbing a $35^\circ$ slope. Note that all these behaviors are embodied in a single neural network without specialized training for a particular scenario.}
    \label{figure:dreamwaqpp_main_fig}
\end{figure}


As opposed to model-based control, deep RL methods reformulate the optimization problem into offline optimization during training by learning a decision-making policy that implicitly plans future control actions based on given observations. Notably, a blind locomotion controller, relying only on proprioception, demonstrates impressive robustness across various terrain profiles~\cite{lee2020learning,kumar2021rma,ji2022concurrent,nahrendra2023dreamwaq,choi2023learning}. However, the resilience of blind locomotion controllers is inherently limited, as they require collisions between the robot's legs and the environment to sense obstacle properties and adjust the gait accordingly.

To advance blind locomotion controllers, an efficient fusion of proprioception and exteroception to learn a robust quadrupedal locomotion controller is actively studied in the legged robotics community~\cite{miki2022learning,gangapurwala2022rloc,yang2022learning,imai2022vision,agarwal2022legged,yang2023neural}. Naturally, animals have an agile locomotion behavior, owing to their ability to observe the terrain ahead using their eyes and quickly plan their effective gait for traversing the terrain. Therefore, incorporating exteroception for the gait planning of legged robots is paramount for eliciting agile behaviors~\cite{ho2022people,di2019walking,chopra2018cognitively,killeen2017minimum}.

We propose DreamWaQ++, an obstacle-aware quadrupedal locomotion controller that specifically aims to tackle the following challenges: 1) a resilient controller with multi-modal perception capability and sensor-agnostic nature that can be integrated with various options of exteroceptive sensors, 2) an efficient control framework that enables real-time control and fast adaptation, 3) an efficient reinforcement learning (RL) pipeline with a single-stage learning procedure. By employing DreamWaQ++ on a Unitree Go1~\cite{unitreego1}, we demonstrated remarkable performance in traversing various challenging environments\mvonefoot as shown in \figinitref{figure:dreamwaqpp_main_fig}.

This paper is an evolved version of the conference paper~\cite{nahrendra2023dreamwaq}. We have extended the work by providing substantial improvement in the controller's performance and robustness in the following aspects:
\begin{itemize}
    \item Incorporation of a novel multi-modal perception module that fuses proprioception and exteroception. The module enables the controller to adapt to various terrains and obstacles, including stairs, gaps, and deformable terrains.
    \item Enhanced robustness via a multi-modal deep RL framework that enables the controller to efficiently leverage the multi-modal perception module for learning a robust locomotion policy in a single-stage learning procedure.
    \item Improved agility via skill discovery objectives that encourage the controller to learn versatile gaits for traversing diverse terrains and obstacles.
    \item Extensive evaluation on various challenging environments and robotics platforms, highlighting the robustness and scalability of the proposed controller.
    \item Ablation studies to analyze the framework's components and their contributions to the controller's performance, opening up new research directions for future work.
\end{itemize}


==> TRO-Dreamwaqpp-arxiv/accept/methods.tex <==
\section{The Proposed Learning Framework}

\input{\MainPath/methods/overview}
\input{\MainPath/methods/perception}
\input{\MainPath/methods/control}
\input{\MainPath/methods/environment}



==> TRO-Dreamwaqpp-arxiv/accept/methods/control.tex <==
% \section{Control Pipeline}\label{section:control}

% \input{\MainPath/control/problem}
\input{\MainPath/control/skill_discovery}
% \input{\MainPath/control/locomotion}

==> TRO-Dreamwaqpp-arxiv/accept/methods/environment.tex <==
\section{Implementation Details}
\input{\MainPath/environment/simulation}
\input{\MainPath/environment/locomotion}
% \input{\MainPath/environment/curriculum}
\input{\MainPath/environment/domain_randomization}
\input{\MainPath/environment/adversarial_obs}
\input{\MainPath/environment/privileged}
\input{\MainPath/environment/reward}








==> TRO-Dreamwaqpp-arxiv/accept/methods/overview.tex <==
\subsection{Overview}
    \begin{figure*}[t!]
        \centering 
        \begin{subfigure}[b]{0.98\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/main/overview.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{Overview of DreamWaQ++. The encoder has a hierarchical structure that consists of low-level raw measurement encoders and a spatio-temporal mixer.}
        \label{figure:dreamwaqpp}
    \end{figure*}
    DreamWaQ++ comprises a perception pipeline and a control pipeline, detailed throughout this section. All modules are jointly trained with a combination of objective functions that facilitate interaction between networks, promoting cooperative learning of informative latent features. This training approach resembles the context adaptation paradigm in a few-shot meta-RL setting~\cite{finn2017model,rakelly2019efficient}. Specifically, the context encoder is trained on a large dataset of simulated quadrupedal locomotion with extensive domain randomization, resembling the meta training phase. Subsequently, the learned context is used to condition the policy in real time, akin to the meta-testing phase. Simultaneously, the policy is trained to effectively control the robot, thereby mitigating the impact of poor context features and state estimation. All trained networks were deployed on a real-world quadrupedal robot with onboard sensors, without any fine-tuning. An overview of the entire framework is shown in Fig.~\ref{figure:dreamwaqpp}.

    The control problem is formulated in a partially observable Markov decision process~(POMDP) setting with a goal to maximize the expected discounted future rewards, which in turn results in a policy:

    \begin{equation}
        \pi=\argmax_{\textbf{a}} E\left[\sum_{t=0}^{\infty}\gamma^t r_t\right],
        \label{eq:pi}
    \end{equation}
    where $\textbf{a}$, $\gamma$, and $r$ are the action, discount factor, and rewards, respectively. This objective is optimized using the proximal policy optimization (PPO)~\cite{schulman2017proximal} algorithm, while also taking into account the auxiliary objectives related to the perception pipeline.


    We adopt a privileged learning setting using an asymmetric actor-critic architecture trained using the proximal policy optimization (PPO)~\cite{schulman2017proximal} algorithm. The actor, i.e. the policy receives partial and noisy observations ($\textbf{o}^\mathrm{p}_t$), akin to the real-world observations and the multi-modal context ($\textbf{z}^\mathrm{pe}_t$) as its input.  The critic, by contrast, receives a privileged state that are accessible only in simulation. The policy network runs at a rate of $50~\mathrm{Hz}$, generating a target joint position that is tracked by a low-level PD controller, running at $200~\mathrm{Hz}$, to generate the joint torque commands.

==> TRO-Dreamwaqpp-arxiv/accept/methods/perception.tex <==
% \section{Perception Pipeline}\label{section:perception}
% The proposed multi-modal context encoder is composed of three key modules as illustrated in Fig.~\ref{figure:dreamwaqpp} and detailed in the following sections. The multi-modal context encoder generates a cross-modal embedding that captures the robot's internal and external states that are utilized by the policy.

\input{\MainPath/perception/exteroceptive_memory}
\input{\MainPath/perception/exteroceptive_encoder}
\input{\MainPath/perception/proprioceptive_encoder}
\input{\MainPath/perception/mixer}
\input{\MainPath/perception/objectives}






==> TRO-Dreamwaqpp-arxiv/accept/perception/exteroceptive_encoder.tex <==
\subsection{Exteroceptive Encoder}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/reduced/ext_encoder_red.pdf}
	\end{subfigure}
	\caption{The exteroceptive encoder uses a PointNet-based architecture as its backbone. We designed a confidence filter layer that statistically learns a masking layer that cancels out unreliable point features before aggregating them into the exteroceptive context $\textbf{z}^\mathrm{e}_t$.}
	\label{figure:ext_encoder}
\end{figure}

We utilized 3D points as input to our framework to enable flexible compatibility with multiple sensor configurations, such as a 3D LiDAR sensor or depth camera. A PointNet-based architecture~\cite{qi2017pointnet} is employed to effectively extract information from the input point cloud, accommodating an arbitrary number of points while maintaining robustness to noise.

Although the max-pooling layers in PointNet enforce invariance to the number and order of input points in the point cloud, they can become detrimental when outliers and heavy noise dominate the input. This issue arises because the max-pooling operation aggregates point features indiscriminately. To address this, we employ a confidence filter layer following the backbone PointNet architecture (Fig.~\ref{figure:ext_encoder}). The confidence filter statistically rejects unreliable points in the latent space using a filtering operation, resulting in confidence-filtered points defined as:

\begin{equation}\label{eq:confidence_filter}
    \mathcal{C} \left( \textbf{o}^{\mathrm{e},K}_t \right) = \psi^\textrm{e} \left( \textbf{o}^{\mathrm{e},K}_t \right) \cdot\left( 1 - \tanh \left( \sigma \left( \textbf{o}^{\mathrm{e},K}_t\right) \right) \right),
\end{equation}
where $ \psi^\textrm{e} \left(\cdot\right)$ is the backbone PointNet layer, and $\sigma(\cdot)$ is a standard deviation operator that statistically assesses the diversity of the input point cloud. A hyperbolic tangent operation, $\tanh(\cdot)$, is used to smoothly set an upper bound of $\sigma \left( \textbf{o}^{\mathrm{e},K}_t \right)$ to one. Each point feature, $\psi\left(\textbf{o}^{\mathrm{e},K}_t\right)$, is fed into a shared confidence mask layer that outputs confidence masks based on the statistics of the raw points. The confidence mask outputs a value close to $1$ for high-variance features and a value close to $0$ for low-variance features, due to the $\tanh$ layer. Following \eqref{eq:confidence_filter}, $\mathcal{C} \left( \textbf{o}^{\textrm{e},K}_t \right)$ removes high-variance features, such as outliers, while preserving low-variance features. The filtered point features are then aggregated using max-pooling to obtain the exteroceptive context $\textbf{z}^\mathrm{e}_t$.


==> TRO-Dreamwaqpp-arxiv/accept/perception/exteroceptive_memory.tex <==
\subsection{Hierarchical Exteroceptive Memory}
Employing exteroceptive measurements in a controller presents distinct challenges due to the low-frequency nature of the sensor, which operates at approximately two to five times lower than the control loop and proprioceptive sensors. This asynchrony introduces non-negligible delays into the control loop, yielding degraded performance.

We circumvent this issue using a memory structure that generates a denser point cloud, $\textbf{o}^{\mathrm{e},K}_t$, around the robot by concatenating points from the last $K$ measurements, each transformed to the robot's current position using $SE(3)$ transformations. Unlike approaches such as~\cite{hoeller2022neural,hoeller2023anymal}, which employ U-Net-based architectures for full scene reconstruction, we use autoregression solely to estimate the $SE(3)$ transformation of the robot’s body frame over time. This method avoids computationally intensive reconstruction while still providing temporally dense exteroception for the controller.

The $SE(3)$ transformation is updated at each control loop iteration by combining the IMU's orientation measurement with the integration of the body linear velocity $\textbf{v}_t$ predicted by the state estimation network, which leverages the history of the robot’s proprioception as detailed in Section~~\ref{section:proprioceptive_encoder}. This transformation process enables temporal extrapolation of the latest exteroceptive measurements by aligning previous points with the robot’s current frame, forming the basis of a memory structure that is then fed into the exteroceptive encoder. The exteroceptive observation is formally defined as follows:

\begin{equation}
    \textbf{o}^{\mathrm{e},K}_t = \textbf{o}^\mathrm{e}_t \concat \hat{\textbf{o}}^\mathrm{e}_{t-1} \concat \cdots \concat \hat{\textbf{o}}^\mathrm{e}_{t-K}, 
  \end{equation}
   where $\textbf{o}^\mathrm{e}_t$ is the most recent exteroceptive observation at time $t$. $\hat{\textbf{o}}^\mathrm{e}_{t-K}$ is the previous exteroceptive observation at $t-K$, which has been transformed to the robot's body frame at time $t$, which is defined as
  \begin{equation}
    \hat{\textbf{o}}^\mathrm{e}_{t-k} = \prescript{t-k}{t-K}{T}^{-1}\cdot \textbf{o}^\mathrm{e}_{t-K},
  \end{equation}
where $\textbf{o}^\mathrm{e}_{t-k}$ is the exteroceptive observation measured at time $t-k$~$\left(k\in[0, K]\right)$, and $\prescript{t-k}{t-K}{T}$ is the $SE(3)$ transformation of the robot's pose from time $t$ to $t-k$. 

As the state estimation network only predicts the body linear velocity, we integrate this velocity over $k$ steps using Euler integration to estimate the robot's position transformation. Although drift may accumulate in the pose estimate over time, we found that this is not significant because the integration is reset every $K$ steps when a new exteroceptive measurement is received. Moreover, we also randomized the exteroceptive sensor pose with respect to the robot body frame during training and applied several levels of exteroception noise to enhance the policy's robustness against erroneous local pose estimation and exteroception data~(Section~\ref{section:adversarial}).

In this work, we set the exteroception sampling rate to $10~\textrm{Hz}$, resulting in $K=5$ for constructing the exteroceptive memory. While higher sampling rates are theoretically possible depending on the choice of sensor, we selected $10~\textrm{Hz}$ due to practical constraints. In particular, higher rates might be slightly unreliable due to data processing latency on the limited onboard computing resources. Moreover, using $10~\textrm{Hz}$ sampling rate also allows us to change the sensor into LiDAR without the need to retrain the policy, as commercial 3D LiDAR sensors typically operate at $10~\textrm{Hz}$.



==> TRO-Dreamwaqpp-arxiv/accept/perception/mixer.tex <==
\subsection{Multi-Modal Mixer}
The multi-modal mixer network was implemented using an MLP-mixer architecture, where the input features are treated as tokens and the time frames are treated as channels. Both the token-mixing and channel-mixing MLPs consist of two hidden layers with 256 hidden units each and employ ELU activation functions. 

To stabilize learning, we apply layer normalization separately to the proprioceptive and exteroceptive latent features before passing them into the multi-modal mixer. This normalization step ensures that the two modalities are on a comparable scale, thereby facilitating more effective fusion.

The multi-modal mixer was trained end-to-end alongside all other networks in DreamWaQ++, as shown in Fig.~\ref{figure:dreamwaqpp}. However, this setup presents a trade-off in numerical stability during the early stages of training.

A straightforward solution is to balance the weights of the reconstruction loss and KL divergence in $\mathcal{L}_\mathrm{VAE}$. In variational inference, the prior distribution of the latent state is typically assumed to follow a normal distribution. Strong minimization of latent loss during training can help the encoder better approximate the latent space, enhancing training stability. However, this approach risks posterior collapse, wherein the encoder neglects critical input details, impairing the policy’s ability to detect and respond to small environmental obstacles. To address this, we introduced a constrained reparameterization trick, defined as follows:

\begin{equation}
    \textbf{z} \sim N(g_{\mu}(\textbf{x}),g_{\sigma}(\textbf{x})),
\end{equation}
where $\textbf{z}$ is a stochastic latent vector and $\textbf{x}$ is the input to the encoder network $g$. The subscripts $\mu$ and $\sigma$ indicate the outputs of $g(x)$ that correspond to the mean and standard deviation of the latent distribution, respectively. $\textbf{z}$ is sampled from a Gaussian distribution $N(\cdot,\cdot)$ with mean $g_{\mu}(\textbf{x})$ and standard deviation $g_{\sigma}(\textbf{x})$. 

During the reparameterization step, we imposed hard constraints on the standard deviation of the distribution, ensuring $\sigma_\mathrm{min} \leq g_{\sigma}(\textbf{x}) \leq \sigma_\mathrm{max}$. This constraint guarantees numerically stable samples that can be reliably propagated to subsequent network layers. By implementing this simple yet effective solution, we achieve greater training stability without compromising the policy’s final performance. Empirically, we set $\sigma_\mathrm{min}\!=\!0$ and $\sigma_\mathrm{max}\!=\!5$ to facilitate stable training. This constrained reparameterization trick is applied across all encoder networks that use a stochastic layer.


==> TRO-Dreamwaqpp-arxiv/accept/perception/objectives.tex <==
\subsection{Learning Objectives}
We trained the multi-modal context encoder using three losses: an estimation loss, $\mathcal{L}_\textrm{est}$, a proprioceptive variational auto-encoder (VAE) loss, $\mathcal{L}^\textrm{p}_\textrm{VAE}$, and an exteroceptive VAE loss,  $\mathcal{L}^\textrm{e}_\textrm{VAE}$. These losses are combined and included as an auxiliary term in the policy loss.


\subsubsection{Estimation Loss}\label{section:estimation_loss}
The estimation loss is used to train the proprioceptive encoder to explicitly estimate the body velocities of the robot, $\tilde{\textbf{v}}_t$.  The estimation objective was formulated using mean-squared-error (MSE) loss as:
\begin{equation}
  \mathcal{L}_\text{est}=\mathrm{MSE}(\tilde{\textbf{v}}_t,\textbf{v}_t),
\end{equation}
where $\textbf{v}_t$ as the ground-truth (GT) body velocity of the robot in the robot frame. We also adaptively bootstrap $\tilde{\textbf{v}}_t$ during policy training to improve the robustness of the policy~\cite{nahrendra2023dreamwaq}. To avoid exploiting inaccurate estimation in the early stage of training, a bootstrapping probability, $p_\text{boot}\!\in\![0,1]$, is computed by measuring the coefficient of variation, $CV(\cdot)$ of the cumulative rewards $\textbf{R}\in\mathbb{R}^{m\times1}$. The probability is formulated as 
\begin{equation}
  p_\text{boot}= 1 - \tanh(CV(\textbf{R})).
  \label{eqn:adaboot}
\end{equation}


\subsubsection{VAE Loss} 
The multi-modal context encoder is trained using an unsupervised method with two reconstruction tasks. First, the proprioceptive encoder is trained to reconstruct the future observation,  $\tilde{\textbf{o}}_{t+1}$, to encourage the predictive nature of the network. We employ $\beta$-VAE loss for the proprioceptive encoder, formulated as 
\begin{equation}
  \mathcal{L}^\textrm{p}_\text{VAE} = \mathrm{MSE}(\tilde{\textbf{o}}_{t+1},\textbf{o}_{t+1}) + \beta D_\text{KL}(q(\textbf{z}^\textrm{p}_t|\textbf{o}^{\mathrm{p},H}_t)\parallel p(\textbf{z}^\textrm{p}_t)),
\end{equation}
where the first term is the reconstruction loss and the second term is the latent regularization loss expressed with a Kullback-Leibler (KL) divergence operation. The latent regularization is scaled with $\beta=5.0$ to encourage disentanglement~\cite{nahrendra2023dreamwaq,higgins2016beta}. The prior distribution of the proprioceptive context $p(\textbf{z}^\textrm{p}_t)$ is parameterized using a Gaussian distribution and the posterior distribution $q(\textbf{z}^\textrm{p}_t|\textbf{o}^H_t)$ is approximated using a neural network, i.e. via the encoder network. 

Second, the exteroceptive and multi-modal context encoders are trained with an exteroceptive VAE loss, formulated as 
\begin{equation}
  \mathcal{L}^\textrm{e}_\text{VAE} = \mathrm{MSE}(\tilde{\textbf{h}}_{t},\textbf{h}_{t}) + \beta D_\text{KL}(q(\textbf{z}^\textrm{pe}_t|\textbf{o}^\textrm{pe}_t)\parallel p(\textbf{z}^\textrm{pe}_t)),
\end{equation}
where $\textbf{z}^\textrm{pe}_t=f_{\psi_{\mathrm{mix}}}(\textbf{z}^\textrm{p}_t \concat \textbf{z}^\textrm{e}_t)$ is the output of the multi-modal context encoder, as a result of feeding the concatenation of the proprioceptive and exteroceptive context vectors into the mixer network, $f_{\psi_{\mathrm{mix}}}(\cdot)$. $\textbf{o}^\textrm{pe}_t = \textbf{o}^{\textrm{p},H}_t \concat \textbf{o}^{\textrm{e},K}_t$ is the observable proprioception and exteroception. The ground-truth robot-centric height scan, $\textbf{h}_{t}$, is obtained from the simulator, and $\tilde{\textbf{h}}_{t}$ is its reconstruction, which can be obtained via a decoder network that receives $\textbf{z}^\textrm{pe}_t$ as its input.
 
A large value of $\beta$ imposes a strong latent regularization, thus, limiting the reconstruction accuracy, and vice versa. Although it is only a single parameter, tuning $\beta$ is non-trivial and lack of intuition. Therefore, we propose an adaptive $\beta$ scheduling method to ease its tuning procedure by scaling it with a factor, $k$, computed as:
\begin{equation}
    k=\exp{\left(\delta\cdot(\tau-\mathcal{L}_\textrm{recon})\right)},
\end{equation}
where $\delta > 0$ is the learning rate for $k$, $\tau$ is the allowed reconstruction error threshold, and $\mathcal{L}_\textrm{recon}$ is the reconstruction loss. Subsequently, $\beta$ is updated using the following rule:
\begin{equation}
    \beta \leftarrow \begin{cases}
        \beta_\textrm{min} & \text{if } k\beta \leq \beta_\textrm{min}, \\
        k\beta & \text{if } \beta_\textrm{min} \leq k\beta \leq \beta_\textrm{max}, \\
        \beta_\textrm{max} & \text{if } k\beta > \beta_\textrm{max}.
    \end{cases}
\end{equation}
Intuitively, $k$ is updated at every iteration depending on the reconstruction loss of the VAE network. When the reconstruction error exceeds a certain threshold, $\tau$, then $\beta$ is scaled down to allow learning of more accurate reconstruction. In contrast, when the reconstruction error is below the given threshold, $\beta$ is scaled up to allow learning of more disentangled latent representation.

\subsubsection{Contrastive Loss}
Prior works trained an adaptation encoder using a regression loss to explicitly predict environment properties~\cite{kumar2021rma,lee2020learning}. However, this approach might suffer from \textit{realizability gap}~\cite{fu2022deep} caused by insufficient observations to reconstruct the environment properties. To circumvent this issue, we tighten the distribution gap between the learned latent representations of policy's observations and critic's privileged observations, rather than requiring the policy to infer the privileged information via regression. We employ a contrastive learning framework by matching the distribution of the privileged latent features used for the critic with the latent features inferred from partial observations used for the actor within an asymmetric actor-critic setup. We define the contrastive loss as: 
\begin{align}
    \mathcal{L}_\mathrm{contrastive} = &\lambda\left\|\textbf{z}^\textrm{pe}_t - g_{\theta_\mathrm{h}}(\textbf{h}_t)\right\|_2^2 \nonumber \\
    &+ (1-\lambda)\left\|\max(0, m-(\textbf{z}^\textrm{pe}_t - \textbf{z}^\textrm{random}_t))\right\|_2^2,\label{eq:contrastive_loss}
\end{align}
where $g_{\theta_\mathrm{h}}(\textbf{h}_t)$ is the encoded ground-truth height scan, which is used as the positive anchor for the contrastive loss. Meanwhile, $\textbf{z}^\textrm{random}_t$ is a random latent feature sampled from $\mathcal{U}[-1.0,1.0]$, which is used as the negative anchor. The parameters $m\!\in\!\mathbb{R}^+$ and $\lambda\!\in\![0, 1]$ are the margin for the negative pair separation and scaling factor, respectively. This contrastive loss forces the multi-modal latent feature to match the encoded ground-truth height scan, while also distancing the latent feature from an unstructured representation labeled by the uniformly random latent feature.

==> TRO-Dreamwaqpp-arxiv/accept/perception/proprioceptive_encoder.tex <==
\subsection{Proprioceptive Encoder}\label{section:proprioceptive_encoder}
The proprioceptive encoder is based on the context-aided estimator network (CENet)~\cite{nahrendra2023dreamwaq}, modified by replacing standard fully connected layers with an MLP-mixer architecture~\cite{tolstikhin2021mlp}. This modification enables interactions across different proprioceptive modalities over multiple time frames, enhancing both the explicit estimation and latent representation of proprioception. To achieve this, we treat the proprioceptive features as tokens and the time frames as channels, enabling the MLP-mixer to learn interactions across different proprioceptive modalities and temporal dimensions. We employ MLPs with two hidden layers, each consisting of 256 hidden units, and use ELU activation functions for both the token-mixing and channel-mixing MLPs.

The encoder receives a stack of temporal observations at time $t$ over the past $H$ measurements as $\textbf{o}^{\mathrm{p},H}_t=\begin{bmatrix}\textbf{o}^\mathrm{p}_t\ \textbf{o}^\mathrm{p}_{t-1}\;\cdots\;\textbf{o}_{t-H} \end{bmatrix}^T$, allowing the policy to infer context with short-term memory. Specifically, we set $H\!=\!5$, with the policy running at $50~\textrm{Hz}$, providing a memory window of $100~\textrm{ms}$.

The proprioceptive encoder is trained to output a distribution over latent states using variational inference~\cite{higgins2016beta}, supporting exploratory learning and serving as a denoising mechanism to aid domain adaptation. This stochastic latent representation significantly reduces the sim-to-real gap, resulting in smooth and robust real-world control~\cite{nahrendra2023dreamwaq}. 

The latent vector $\textbf{z}^{\mathrm{p}}_t$ is used as input to the multi-modal mixer and for body velocity estimation via an additional estimation layer following the encoder. The body velocity estimation layer is a fully connected layer with 256 hidden units and ELU activation, which predicts the body linear velocity $\hat{\textbf{v}}_t$ using the loss function in Section~\ref{section:estimation_loss}.


==> TRO-Dreamwaqpp-arxiv/accept/related_works.tex <==
\section{Related Works}
In recent years, research on legged locomotion has made significant progress, largely driven by advancements in simulation-based policy learning through deep reinforcement learning. Earlier works in the field primarily focused on blind locomotion strategies, aiming to ensure reliable sim-to-real transfer by minimizing actuator model discrepancies~\cite{hwangbo2019learning} and incorporating adaptation mechanisms to handle environmental variations~\cite{lee2020learning,kumar2021rma,ji2022concurrent,nahrendra2023dreamwaq}. These approaches relied predominantly on proprioceptive inputs to control the robot's movement. However, due to their limited perceptual capabilities, these methods often struggle in more complex dynamic environments.

To address these limitations, exteroceptive perception has been incorporated into the locomotion pipeline to enable policies that are not only stable but also aware of the surrounding terrain geometry, particularly near the robot’s legs~\cite{miki2022learning,gangapurwala2022rloc,agarwal2022legged,loquercio2023learning}. Recent studies have utilized raw egocentric depth vision for locomotion~\cite{yang2022learning,imai2022vision,agarwal2022legged,yang2023neural,cheng2023parkour}to mimic the locomotion abilities of animals. However, elevation map–based approaches~\cite{miki2022learning,gangapurwala2022rloc,hoeller2023anymal} have proven to be superior, particularly in situations where depth vision is unreliable due to limited field of view~(FoV).

In addition to exteroception, memory-based architectures such as long short-term memory (LSTM) and gated recurrent units (GRU) have become primary components in the success of recent perceptive locomotion controllers~\cite{miki2022learning,margolis2022rapid,ji2022concurrent,choi2023learning} to mitigate partial observability. However, training recurrent network models often suffers from vanishing gradients due to the backpropagation through time (BPTT) mechanism~\cite{werbos1990backpropagation}. As a workaround, variants of convolutional neural network (CNN) architectures have been used as a viable option to handle sequential data~\cite{lee2020learning,kumar2021rma}. However, CNNs are prone to inductive bias, which assumes that neighboring data points are more likely to be related than others. This inductive bias hinders a neural network’s ability to freely learn the positional relationships between features in unstructured time-series data. More recently, attention-based sequence models, such as transformers~\cite{vaswani2017attention,melo2022transformers}, have shown potential as viable alternatives for constructing memory in locomotion tasks~\cite{yang2022learning}.

Utilizing large and expressive models such as transformers is effective for learning complex policies in high-dimensional action spaces~\cite{melo2022transformers}. However, these models typically require large amounts of training data and are more susceptible to real-time inference constraints due to their computational overhead. To effectively balance perception, memory, and fast reaction speed, we propose a multi-modal mixer architecture that combines the strengths of both lightweight MLPs and attention-based mechanisms. This architecture enables efficient processing of both proprioceptive and exteroceptive inputs, allowing the policy to learn a robust and adaptable locomotion strategy.

However, memory alone is sometimes insufficient for achieving resilient locomotion behavior if the learned latent representation obtained from memory does not account for explorative behavior that promotes skill discovery. Without an adequate skill discovery strategy, the latent representation may lead the policy to overfit to a limited range of behaviors, resulting in a conservative policy that struggles to adapt to diverse environmental changes~\cite{li2023versatile,rakelly2021mutual}. Therefore, we propose two regularization techniques that balance accurate perception learning while also promoting explorative behavior. 

==> TRO-Dreamwaqpp-arxiv/accept/results.tex <==
\section{Experimental Results}
    \input{\MainPath/results/hardware}
    \input{\MainPath/results/stair_climbing}
    \input{\MainPath/results/obstacle}
    \input{\MainPath/results/uncertainties}
    \input{\MainPath/results/ood}
    \input{\MainPath/results/scalability}
    \input{\MainPath/results/large_obstacles}

==> TRO-Dreamwaqpp-arxiv/accept/results/hardware.tex <==
\subsection{Hardware Settings}\label{section:hardware}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/reduced/hardware_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{Hardware setup for robots (a)~R1, (b)~R2, (c)~R3, and (d)~R4. R1 was equipped with an Intel RealSense D435f camera, R2 was not equipped with any exteroceptive sensor and used only for blind locomotion, R3 was equipped with an Ouster OS-01 LiDAR, and R4 was equipped with two Livox Mid-360 LiDARs.}
	\label{figure:hardware}
\end{figure}

All networks were trained to control a Unitree Go1~\cite{unitreego1} robot. For the experiments, we used robots with different exteroception configurations, as shown in Fig.~\ref{figure:hardware}. Robots R1, R3, and R4 are Unitree Go1 robots with different exteroception setups, while Robot R2 is a Unitree A1 robot without exteroception.

Robot R1 was equipped with an Intel RealSense D435f camera tilted $45^\circ$ downward, streaming data at $15~\textrm{Hz}$ to the onboard Jetson Xavier NX. To protect cables from potential damage during falls, a canopy was added, increasing the payload by approximately $0.5~\textrm{kg}$.

Robot R2, a Unitree A1 without exteroception, was used to compete against Robot R1. The blind locomotion policy, DreamWaQ~\cite{nahrendra2023dreamwaq} was deployed on the A1 robot because it has similar morphology and motor properties to the Go1, while offering higher torque. Consequently, the Unitree A1 is expected to perform comparably, if not better, than the Unitree Go1 with DreamWaQ, as it can apply additional torque to manage collisions during stair climbing.

Robot R3 was equipped with an Intel NUC PC and an Ouster OS-01 LiDAR. This configuration was used to evaluate the generalization and transferability of the learned controller on a robot with different exteroceptive sensors, resulting in an additional payload of approximately $3.0~\textrm{kg}$. Finally, a fourth robot, R4, equipped with an Intel NUC PC and two Livox Mid-360 LiDARs, was utilized for further experiments in an asynchronous race setting shown in Figs.~\ref{figure:results_stairs}(c)-(e). The additional payloads on R3 and R4 are approximately $2.5~\textrm{kg}$.


% To validate this claim, we conducted an additional race between Unitree A1 and Go1 robots, both controlled by a DreamWaQ policy trained with identical reward parameters. This race, recorded in \mvnine, showed the A1 and Go1 completing the course in $52$ and $60$ seconds, respectively, with both robots commanded to move at $0.8~\mathrm{m/s}$.

==> TRO-Dreamwaqpp-arxiv/accept/results/large_obstacles.tex <==
\subsection[Overcoming Large Obstacles]{Overcoming Large Obstacles\protect\mveightfoot}\label{supp:parkour}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/reduced/results_large_obstacles_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{We trained DreamWaQ++ for (a)~Unitree Go1, (b)~ANYmal-C, and (c)~Hound to climb obstacles with a height of $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, $1.5~\mathrm{m}$, respectively. (d)~A real world experiment was conducted using a Go1 robot with a $2.5~\mathrm{kg}$ payload on top of it.}
	\label{figure:supp_parkour_sim}
\end{figure}

Recently, there has been increasing interest in training quadrupedal robots for complex tasks such as jumping and leaping~\cite{hoeller2023anymal,zhuang2023robot}. These skills require robots to maximize actuator limits and perform highly agile motions. We further assessed the scalability of DreamWaQ++ for overcoming obstacles higher than the robot itself. We trained the Go1, ANYmal-C, and Hound robots in environments with extreme obstacle heights up to $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, and $1.5~\mathrm{m}$, respectively. To enable learning of this agile skill, we made two modifications: (1) reducing the velocity tracking reward scale from $1.0$ to $0.1$, and (2) increasing the versatility gain scaling in the loss function from $0.1$ to $0.2$. Snapshots of the learned obstacle-climbing motions in simulation and real-world scenarios are shown in Fig.~\ref{figure:supp_parkour_sim}.

These modifications were complementary; without scaling up the versatility gain, reducing the velocity tracking reward alone led to a policy that resisted forward movement, while increasing versatility gain alone resulted in a conservative gait lacking skill discovery. Together, these adjustments allowed the policy to learn flexible gaits, yielding the agility required for complex tasks such as parkour.

Results in Fig.~\ref{figure:supp_parkour_sim} illustrate how controllers on different robots produce distinct motions for overcoming large obstacles. In Fig.~\ref{figure:supp_parkour_sim}(a), Go1 uses a jumping motion due to its small size. In contrast, ANYmal-C initially contacts the obstacle wall with its front legs (Fig.~\ref{figure:supp_parkour_sim}(b-2)), then uses them as anchors to climb (Fig.~\ref{figure:supp_parkour_sim}(b-3)). ANYmal-C’s large joint range and torque limits enable it to climb obstacles up to $1.5~\mathrm{m}$. Hound swings its right front leg widely to anchor on top, then propels itself upward with the rear legs (Fig.~\ref{figure:supp_parkour_sim}(c-4)).

In a real-world experiment shown in Fig.~\ref{figure:supp_parkour_sim}(d), we validated the sim-to-real robustness of the controller. A Go1 robot with an additional $2.5~\mathrm{kg}$ payload successfully climbed a $41~\mathrm{cm}$ obstacle, a soft sofa block representing a deformable surface not encountered in training.

In Fig.~\ref{figure:supp_parkour_sim}(e), the robot was placed on a $50~\mathrm{cm}$ stage, preventing simple terrain probing. Upon command, the robot leaped forward, avoiding rear leg collisions with the stage edges. This leap was facilitated by the velocity tracking relaxation, allowing the robot to pause at the edge (Fig.~\ref{figure:supp_parkour_sim}(e-2)) before initiating the leap. The robot kicks forward with its front legs, propels with the rear legs (Fig.~\ref{figure:supp_parkour_sim}(e-3)), and folds the rear legs to avoid collision (Fig.~\ref{figure:supp_parkour_sim}(e-4)). This demonstrates the versatility of the learned controller, serving as a prior adaptable to complex tasks.


==> TRO-Dreamwaqpp-arxiv/accept/results/large_obstacles_origin.tex <==
\subsection{\mveightref{Overcoming Large Obstacles}}\label{supp:parkour}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/reduced/results_large_obstacles_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{We trained DreamWaQ++ for (a)~Unitree Go1, (b)~ANYmal-C, and (c)~Hound to climb obstacles with a height of $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, $1.5~\mathrm{m}$, respectively. (d)~A real world experiment was conducted using a Go1 robot with a $2.5~\mathrm{kg}$ payload on top of it.}
	\label{figure:supp_parkour_sim}
\end{figure}

Recently, there has been a growing interest in training quadrupedal robots for more complex tasks such as jumping and leaping~\cite{hoeller2023anymal,zhuang2023robot}. These skills require the quadruped robot to maximize its actuator limit and orchestrate highly-agile motions. We further assessed the scalability of DreamWaQ++ in learning a skill required for overcoming obstacles that are higher than the robot. We trained the Go1, ANYmal-C, and Hound robots in an environment with extreme obstacle heights, reaching up to $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, and $1.5~\mathrm{m}$, respectively. To allow learning of such an agile skill, we need to do some modifications, i.e., 1) relaxing the velocity tracking reward scale from $1.0$ to $0.1$, and 2) increasing the versatility gain scaling in the total loss function from $0.1$ to $0.2$. A snapshot of the learned obstacle climbing motion in simulation and the real world is shown in Fig.~\ref{figure:supp_parkour_sim} and \mveight.

We found that the two modifications are complimentary. Relaxing the velocity tracking reward without scaling up the versatility gain ends up with a policy that resists moving forward. On the other hand, doubling the versatility gain without relaxing the velocity tracking reward results in a policy that moves forward but with a conservative gait due to lack of skill discovery. This modification allowed the policy to learn more flexible gaits, yielding higher agility for accomplishing more complex tasks such as parkour.

The results in Fig.~\ref{figure:supp_parkour_sim} illustrate how controllers on different robots produce distinct motions when overcoming large obstacles. In Fig.~\ref{figure:supp_parkour_sim}A, Go1 utilizes a jumping motion to overcome the obstacle, given its small posture. In contrast, ANYmal-C employs its front legs to establish initial contacts with the wall of the obstacle (Fig.~\ref{figure:supp_parkour_sim}B-2) and then uses those legs as anchors to climb (Fig.~\ref{figure:supp_parkour_sim}B-3). Thanks to its large allowable joint positions and torque operation limits, ANYmal-C can climb obstacles as high as $1.5~\mathrm{m}$. Hound, on the other hand, firstly swings its right front leg widely and places it on top of the obstacle as an anchor. Subsequently, it uses its rear legs to propel its body upward (Fig.~\ref{figure:supp_parkour_sim}C-4) and successfully reaches the top of the obstacles.

The real-world experiment in Fig.~\ref{figure:supp_parkour_sim}D was conducted to validate the sim-to-real robustness of the learned controller. Utilizing a Go1 robot with an additional $2.5\mathrm{kg}$ payload, the controller successfully enables the robot to climb a $41~\mathrm{cm}$ obstacle. Notably, the obstacle is a soft sofa block, representing a deformable surface not encountered during training.

In Fig.~\ref{figure:supp_parkour_sim}(e) and \mvfour, the robot was positioned on a $50~\mathrm{cm}$ stage, making it impossible for a small quadruped, with a calf length shorter than $30~\mathrm{cm}$, to simply probe the terrain. Therefore, when commanded to move forward, the robot made a leap motion, allowing it to move away from the stage while avoiding collision between the rear legs with the edges of the stage. This leap motion was also made possible by the velocity tracking relaxation strategy that allows the robot to stop at the edge of the stage~(Fig.~\ref{figure:supp_parkour_sim}(e-2)) for initiating the leap motion. Subsequently, the robot performs a kick using both front legs, then propels the movement forward using both rear legs~(Fig.~\ref{figure:supp_parkour_sim}(e-3)). Soon after, the robot also folds its rear legs to avoid collision with the stage~(Fig.~\ref{figure:supp_parkour_sim}(e-4)). This highlights the versatility of the learned controller as a prior that can be adapted for more complex tasks.

==> TRO-Dreamwaqpp-arxiv/accept/results/obstacle.tex <==
\subsection[Obstacle Awareness]{Obstacle Awareness\protect\mvthreefoot}

    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/results_awareness_red.pdf}
        \end{subfigure}
        \captionsetup{font=footnotesize}
        \caption{(a)~Affordance-aware locomotion when ascending stairs with rise of $25~\textrm{cm}$ on the left and $20~\textrm{cm}$ on the right side of the robot. (b)~Emergent behavior to quickly and efficiently climb stairs with long foot swing motion, compared with a regular case (c)~where the robot could not overcome two stair steps at once because the rear foot was located around the middle of the stair step.}
        \label{figure:results_awareness}
    \end{figure}
    

    \subsubsection{Obstacle Negotiation}
        In Fig.~\ref{figure:results_awareness}(a), the controller demonstrated affordance-awareness when navigating terrains of varying difficulty. The robot was given a forward velocity command of $0.6~\mathrm{m/s}$ with a zero yaw rate command. Initially, when commanded to move toward the middle of the stairs (Fig.~\ref{figure:results_awareness}(a-2)), the robot moved toward the lower stair rise on the right side, opting for a less risky path. Subsequently, as the left and right stairs overlapped, a lower step appeared on the left side (Fig.~\ref{figure:results_awareness}(a-6)). The robot quickly adapted its path toward these easier steps, resisting the zero yaw rate command, thereby demonstrating the controller’s ability to learn and perceive the affordances of different obstacles.


    \subsubsection{Foot Swing Adaptation}
        Fig.~\ref{figure:results_awareness}(b) illustrates the performance of the proposed controller on stairs with a $15~\textrm{cm}$ rise. Typically, the controller directs the robot to swing its feet, stepping on each stair sequentially. However, when a foot approaches the edge of a stair, the robot extends its swing phase (indicated by red arrows in Fig.~\ref{figure:results_awareness}(b)), allowing the rear foot to overcome a combined rise of $30~\textrm{cm}$. In contrast, as shown in Fig.~\ref{figure:results_awareness}(c), the robot steps normally when the rear foot is positioned near the middle of the initial stair step. This adaptive behavior suggests that the controller retains a form of memory of the structure beneath the robot, leveraging fused information from the network architecture.


    \subsubsection{Quantitative Performance Assessment}
        \begin{figure}[t!]
            \centering 
            \begin{subfigure}[b]{0.48\textwidth}
                \includegraphics[width=1.0\textwidth]{figures/reduced/results_stairs_quant_red.pdf}
            \end{subfigure}
            \captionsetup{font=footnotesize}
            \caption{Success rate~(SR) comparison measured on each algorithm by simulating $1,\!000$ robots to climb sequence of stairs. The SR is defined as the percentage of the number of robots that reached the last stair within $10~\mathrm{s}$ over the total number of robots.}
            \label{figure:results_stairs_quant}
        \end{figure}

        We compared DreamWaQ++ with a visual locomotion controller based on ViNL~\cite{kareer2023vinl}, training the baseline with the same parameters as DreamWaQ++ but without the navigation pipeline from~\cite{kareer2023vinl}. Additionally, we used only the teacher network to achieve upper-bound performance, noting that this network has access to the ground truth height map around the robot, which we refer to as \textit{ViL-teacher}.

        We simulated $1,000$ robots climbing stairs with increasing rises, as shown in Fig.~\ref{figure:results_stairs_quant}. Using a stair run of $0.3~\mathrm{m}$—a common real-world dimension—and an extended run of $0.6~\mathrm{m}$ to represent low-slope, high-rise obstacles, the results in Fig.~\ref{figure:results_stairs_quant} indicate that DreamWaQ++ achieved success rates $20\!-\!40\%$ higher than the baseline with ground truth height map access. This finding suggests that accurate height map information alone is insufficient for high-performance locomotion, similar to animals' ability to climb without constant visual feedback.

        This improvement is attributed to versatile skill learning promoted by the proposed versatility gain function~$\mathcal{L}_\mathrm{versatility}$, which serves as an intrinsic reward encouraging exploration. Without this gain, the policy lacks exploratory behavior, often resulting in a conservative approach that fails to handle unseen terrains effectively.

==> TRO-Dreamwaqpp-arxiv/accept/results/ood.tex <==
\subsection{Out-of-distribution Adaptation}
\subsubsection[Reacting to Sudden Changes of Foothold]{Reacting to Sudden Changes of Foothold\protect\mvfivefoot}
\begin{figure}[t!]
    \centering 
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=1.0\textwidth]{figures/reduced/results_foothold.png}
    \end{subfigure}
    % \captionsetup{font=footnotesize}
    \caption{Adaptation to sudden changes of foothold. (a)~The robot is externally disturbed by quickly removing the platform it is stepping on. (b)~An abrupt change in the robot's perception made the controller rapidly alter the robot's joints at around $t\!=\!2.5~\mathrm{s}$ to (c)~enlarge the robot's support polygon for ensuring a safe and stable landing. (d)~A 2D embedding visualization using \textit{pairwise controlled manifold approximation projection} (PaCMAP)~\cite{wang2021understanding} shows how the multi-modal context dynamically changes over time and capture changes in the environment, providing informative contexts to swiftly adapt the policy.}
    \label{figure:results_adaptation}
\end{figure}

We evaluated the controller's adaptability to unexpected environmental changes, such as deformable and movable surfaces, which were not encountered during training. In Fig.~\ref{figure:results_adaptation}(a), the robot initially moves toward a movable cart. Upon stepping onto the cart, an abrupt kick is applied, propelling the cart away from the robot.

The controller’s swift response, shown in Fig.~\ref{figure:results_adaptation}(a-4), involved manipulating the front hip joints (Fig.~\ref{figure:results_adaptation}(b-4)) to create a support polygon approximately $20.12\%$ larger than in normal locomotion (Fig.~\ref{figure:results_adaptation}(c)), ensuring a safe landing after the platform was unexpectedly removed.

Fig.~\ref{figure:results_adaptation}(d) visualizes the multi-modal contexts, forming a circular pattern corresponding to foot motion events in Fig.~\ref{figure:results_adaptation}(a). When the cart is kicked at $t\!=\!2.4~\mathrm{s}$ (Fig.~\ref{figure:results_adaptation}(a-3)), the contexts form a new cluster (upper left of Fig.~\ref{figure:results_adaptation}(d)). Subsequently, a distinct cluster appears (bottom left of Fig.~\ref{figure:results_adaptation}(d)) at Fig.~\ref{figure:results_adaptation}(a-4), with fewer embeddings as the policy quickly handles the situation. The embeddings then return to the original circular pattern after the robot lands safely, resuming normal locomotion at $t\!=\!3.2~\mathrm{s}$.


\subsubsection[Climbing Over a Steep Slope]{Climbing Over a Steep Slope\mvsixfoot}
\begin{figure}[t!]
    \centering 
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=1.0\textwidth]{figures/reduced/results_slope_red.pdf}
    \end{subfigure}
    % \captionsetup{font=footnotesize}
    \caption{Comparison of torque exertions when climbing a $35^\circ$ slope using (a)~DreamWaQ and (b)~DreamWaQ++. The annotations on top of the boxplot in~(c) indicate the significance level measured using a paired $t$-test method}
    \label{figure:results_slope}
\end{figure}

Fig.~\ref{figure:results_slope}(c) compares the torque exertion of controllers trained with DreamWaQ and DreamWaQ++ (see Figs.~\ref{figure:results_slope}(a) and~(b)). Both controllers were trained exclusively on rough slopes up to $10^\circ$, while in this experiment, the robot was tasked with climbing a $35^\circ$ slope. DreamWaQ's policy attempts to maintain a flat body orientation (Fig.~\ref{figure:results_slope}(b)), as it was trained with a blind locomotion controller to generalize across various terrains. Although broadly effective, this approach results in conservative behavior and greater torque exertion on the rear legs (Fig.~\ref{figure:results_slope}(a)) to uphold the flat base pose.

In contrast, the DreamWaQ++ policy employs a crawling gait with a reduced body height relative to the slope surface, aligning the robot’s base orientation with the slope inclination, which enhances stability and reduces torque on the rear legs, as shown in Fig.~\ref{figure:results_slope}(b). DreamWaQ++'s terrain perception enables flexible gait adaptation rather than a conservative approach. Notably, rear leg torque in DreamWaQ++ is approximately $1.5$ times lower than in DreamWaQ, demonstrating DreamWaQ++'s superior out-of-distribution adaptation.


==> TRO-Dreamwaqpp-arxiv/accept/results/scalability.tex <==
\subsection[Scalability to Other Platforms]{Scalability to Other Platforms\protect\mvsevenfoot}\label{supp:scalability}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/reduced/multirobot_success_rev_red.pdf}
	\end{subfigure}
	\caption{Success rates for climbing different obstacles using various quadrupedal robots. We trained DreamWaQ++ for Unitree Go1, ANYmal-C, and Hound. The maximum stair rise imposed during training for all robots is $27~\mathrm{cm}$.}
	\label{figure:supp_multi_robot}
\end{figure}

We evaluated the scalability of DreamWaQ++ by applying it to legged robots with different morphologies and sizes by training controllers for ANYmal-C~\cite{hutter2016anymal} and Hound~\cite{shin2022design} robots. Note that we used the same reward functions and its corresponding weights. Particularly, we adjusted only the robot-specific parameters such as the robot models, the motor operation limit, motor stiffness and damping parameters, desired foot clearance, desired body height, and maximum foot contact force.

\figinitref{figure:supp_multi_robot} presents the success rates of three different robots climbing stairs with varying runs and rises. For the Go1 robot, we used run values of $0.3~\mathrm{m}$ and $0.6~\mathrm{m}$, while for ANYmal-C and Hound, we used $0.6~\mathrm{m}$ and $1.0~\mathrm{m}$ runs to accommodate their longer trunk sizes. Success rates were measured from $1,\!000$ simulated robots, defined as the percentage reaching the last stair within $10~\mathrm{s}$.

As expected, Hound’s extensive joint operation range enabled it to traverse more challenging terrains than the Go1 and ANYmal-C, achieving an $80\%$ success rate on $42~\mathrm{cm}$-high stairs. Notably, the robots were only trained on obstacles up to $27~\mathrm{cm}$ in height, underscoring the strong adaptability of DreamWaQ++. The controller’s exploratory training maximizes hardware capability, with reward functions invariant to hardware differences.

This evaluation highlights DreamWaQ++'s versatility across various legged robots. Despite the sensitivity of deep RL algorithms to reward parameters, DreamWaQ++ demonstrated easy adaptability to different platforms without additional tuning.


% We assessed the scalability of DreamWaQ++ with applications to legged robots with various morphologies and sizes. We used DreamWaQ++ to train a controller for an ANYmal-C~\cite{hutter2016anymal} and Hound~\cite{shin2022design} robots. Note that we used the same rewards and its corresponding weights as in supplementary section~\ref{supp:reward_functions} and only changed the robot's model as well as their motor's stiffness and damping parameter. A compilation of these robots navigating over stairs is provided in \mvseven. 

% \figinitref{figure:supp_multi_robot} shows the success rates of three different robots on climbing stairs with various runs and rises. For the Go1 robot, we used a run value of $0.3~\mathrm{m}$ and $0.6~\mathrm{m}$, while for ANYmal-C and Hound, we used a run value of $0.6~\mathrm{m}$ and $1.0~\mathrm{m}$ to accommodate for their long trunk size. The success rates are measured from $1,\!000$ simulated robots, which is defined as the percentage of the number of robots that can reach the last stair within $10~\mathrm{s}$ over the total number of robots.

% As expected, the large joint operation range of Hound enabled it to traverse more difficult terrains compared with the Go1 and ANYmal-C robot, allowing it to traverse up to $42~\mathrm{cm}$-high stairs with an $80\%$ success rate. It is also noteworthy that during training, the robots are faced only with a maximum obstacle height of $27~\mathrm{cm}$, and this result highlights the strong adaptability of the controller trained with DreamWaQ++. Thanks to the explorative behavior during training, DreamWaQ++ also maximizes the hardware's capability and the reward functions are invariant to the hardware variations.

% This evaluation successfully highlights the versatility of DreamWaQ++ for its applications to various legged robots. Although deep RL algorithms are notoriously sensitive to reward parameters for different robots, we discovered that DreamWaQ++ can be easily adopted to different platforms with no further tuning effort. 

==> TRO-Dreamwaqpp-arxiv/accept/results/stair_climbing.tex <==
\subsection{Fast Locomotion over Obstacles}
    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/results_race_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
            \vspace{-0.2cm}
        \caption{(a)~A head-to-head race between the proposed controller against baselines. (b)~3D map visualization of the race environment. Asynchronous stair-climbing experiments were conducted to ensure fairness, where the robot was controlled using (c)~DreamWaQ++, (d)~DreamWaQ, and (e)~Unitree Go1's built-in controller. The white mask on the stair indicates the same stair plate that each robot interacted with over the four successive snapshots. (f)~Velocity estimation error comparison in the stair-climbing task. The **** annotation indicates the significance level computed using a paired $t$-test.}
        \label{figure:results_stairs}
    \end{figure}

    \subsubsection[Head-to-head Racing Across Stairs]{Head-to-head Racing Across Stairs\protect\mvtwofoot}
    We benchmarked the proposed controller against DreamWaQ~\cite{nahrendra2023dreamwaq} (a baseline blind locomotion controller) and the robot's built-in perceptive controller~\cite{unitreego1} in a head-to-head stair-climbing race as shown in Fig.~\ref{figure:results_stairs}(a). 

    The experimental setup consisted of fifty stairs, and we used robots R1, R2, and R3 as described in Section~\ref{section:hardware}. Robots R1, R2, and R3 were controlled by DreamWaQ++, DreamWaQ, and Unitree's built-in controller, respectively. All robots started from the same point before the stairs, except for R3, which was placed one stair ahead due to the built-in controller's difficulty with the height of the first step. For safety reasons, all robots were manually controlled by a human operator.

    Robot R1 quickly outperformed the others, gaining a lead shortly after the starting point, as shown in Fig.~\ref{figure:results_stairs}(b). To mitigate frequent stumbles, robot R2 was commanded at a linear velocity of $1.2~\mathrm{m/s}$ but continued to experience tracking errors due to frequent missteps on stair edges. In contrast, robot R1 adaptively adjusted its gait and foot placement, enabling faster traversal at a lower velocity command of approximately $1.0~\mathrm{m/s}$. Robot~R3, however, struggled with stair climbing due to latency in its perceptive controller’s reaction time, which depends on a local environmental map and limits both speed and agility.

    The race concluded when one robot reached the final stair to assess overall reachability (Fig.~\ref{figure:results_stairs}(b)). Robot R1 completed the race in $35~\mathrm{s}$, covering a horizontal distance of approximately $30.03~\mathrm{m}$ and a height of $7.38~\mathrm{m}$. By the same timestamp, R2 had covered about $20.05~\mathrm{m}$ horizontally and $5.44~\mathrm{m}$ in height, while R3 failed to finish after stumbling and covering only $6.38~\mathrm{m}$ horizontally and $2.44~\mathrm{m}$ in height. This experiment highlights the superior agility of the proposed controller in handling continuous obstacles.


    \subsubsection[Asynchronous Race]{Asynchronous Race\protect\mvtenfoot}
    We conducted additional asynchronous experiments using robot R4 (Fig.~\ref{figure:hardware}(d)) with autonomous navigation to ensure consistent path planning during stair climbing. This experiment aimed to validate the performance of DreamWaQ++ in a more controlled setting, where the same robot hardware was tested using both DreamWaQ and DreamWaQ++. Key snapshots highlighting the robot's movements are shown in Figs.~\ref{figure:results_stairs}(c)-(e).

    A discernible behavior between DreamWaQ++ and DreamWaQ is in their gait adaptation. DreamWaQ++ raises the body and extends foot swing to step securely on the stairs (Fig.~\ref{figure:results_stairs}(c)), whereas DreamWaQ often collides and drags the foot along the stair edge before stepping (Fig.~\ref{figure:results_stairs}(d)), resulting in reduced efficiency and more frequent stumbles. The built-in controller uses a fixed gait, lacking spatial memory and adaptability, leading to rear leg stumbles (Fig.~\ref{figure:results_stairs}(e)).

    We also measured state estimation errors for DreamWaQ++ and DreamWaQ during these experiments. This error, defined as the absolute difference between ground truth and estimated velocities, was computed using a LiDAR odometry algorithm~\cite{xu2022fast}. As shown in Fig.~\ref{figure:results_stairs}(f), DreamWaQ++ demonstrated significantly lower estimation errors, indicating superior position estimation and gait adaptation—crucial for efficient stair climbing and enhanced stability and robustness.


==> TRO-Dreamwaqpp-arxiv/accept/results/uncertainties.tex <==
\subsection[Uncertainty Awareness and Adaptation]{Uncertainty Awareness and Adaptation\protect\mvfourfoot}
    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/results_probing_rev_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{An emergent probing skill enables the robot to check the upcoming terrain when it poses a high risk and uncertainty. (a)~A sequence of the robot's movement to probe the upcoming terrain. (b)~Corresponding velocity commands and estimation, showing how the controller resists the given command and allocates time for the robot to check for the terrain. (c)~Significant knee flexion-extension~(KFE) motions indicated by a sudden change in the calf joint angle, revealing the emergent adaptive behavior as a novel probing skill.}
        \label{figure:results_probing}
    \end{figure}

    Fig.~\ref{figure:results_probing} demonstrates an emergent locomotion behavior of the proposed controller when traversing terrains with significant height differences. Figs.~\ref{figure:results_probing}(a)-(c) visualize snapshots of the robot's motion, commanded and estimated base velocity, and joint angles, respectively. When confronted with a stage featuring a large elevation difference, the controller could not accurately gauge the terrain height near the robot's front feet. In response, the robot deliberately stops before the ridge (Fig.~\ref{figure:results_probing}(a-2)) and orchestrates its feet to probe the terrain characteristics (Fig.~\ref{figure:results_probing}(a-3)). Upon detecting solid ground, the robot continues moving forward and confidently descends from the edge of the stage (Fig.~\ref{figure:results_probing}(a-4)). Subsequently, the robot spreads its rear legs and uses them as anchors, reducing the impact on the front legs upon landing.

    

   

==> TRO-Dreamwaqpp-arxiv/accept/supplementaries.tex <==
\section{Supplementaries}\label{section:supp}

\begingroup
% \renewcommand{\thesubsection}{S\arabic{subsection}}

% \renewcommand{\figurename}{Fig.}
% \renewcommand{\thefigure}{S\arabic{figure}}
% \captionsetup[figure]{labelfont=bf,labelsep=period,font=normalsize}

% \renewcommand{\thetable}{S\arabic{table}}
% \captionsetup[table]{labelfont=bf,labelsep=period,font=normalsize}

% \setcounter{figure}{0}


\subsection{Nomenclature}\label{supp:nomenclature}
\begin{table}[h!]
    \small
    \begin{tabular}{ll}
        \textbf{Notations} \\
        $(\cdot)^\textbf{des}$ & Target or desired value\\
        $(\cdot)^\textbf{cmd}$ & Command value\\
        $\textbf{g}$ & Gravity vector projected on the robot's body frame\\
    \end{tabular}
\end{table}

\begin{table}[h!]
    \small
    \begin{tabular}{ll}
        \textbf{Operators} \\
        $\mathrm{exp(\cdot)}$ & Exponential function\\
        $\mathrm{var(\cdot)}$ & Variance function\\
         $\mathrm{\sigma(\cdot)}$ & Standard deviation function\\
    \end{tabular}
\end{table}

\begin{table}[H]
    \small
    \begin{tabular}{ll}
        \textbf{Abbreviations} \\
        IMU & Inertial measurement unit\\
        HAA & Hip abduction/adduction\\
        HFE & Hip flexion/extension\\
        KFE & Knee flexion/extension\\
        FR & Front right\\
        FL & Front left\\
        RR & Rear right\\
        RL & Rear left\\
        MLP & Multi-layer perceptron\\
        PaCMAP & Pairwise controlled manifold approximation projection\\
        PD & Proportional and derivative\\
        POMDP & Partially observable Markov decision process\\
        PPO & Proximal policy optimization\\
        t-SNE & t-distributed stochastic neighbor embedding\\
        VAE & Variational autoencoder\\
    \end{tabular}
\end{table}


\begin{table*}[h!]
    \centering
    \caption{\textbf{Summary of state-of-the-art algorithms}. \textit{Versatility} indicates whether the learned controller can be flexibly used for various tasks, e.g.~using a teleoperation or with a high-level planner. \textit{Computation} indicates the number of onboard processor(s) used on the robot to infer the whole locomotion controller, including the processor(s) used for preprocessing the exteroceptive measurement. \textit{Exteroception} indicates what type of exteroceptive measurement is required as an input.  \textit{Training stage} indicates the number of separate training procedures. Training stage~$\!=\!1$ means that there is no pre-training or fine-tuning of the networks using additional training instances. Training stage~$\!>\!1$ means additional training instances are required such as distillation, fine-tuning, and pre-training of some auxiliary modules.}
    \small
    \begin{tabular}{|c|c|c|c|c|c|} \hline 
         \multirow{2}{*}{Algorithm}&   \multirow{2}{*}{Robot}& \multicolumn{2}{|c|}{Deployment}&  \multirow{2}{*}{Exteroception}& Training\\ \cline{3-4}
         \multirow{2}{*}{} & \multirow{2}{*}{} &  Versatility&Computation& \multirow{2}{*}{}&stage\\\hline
         Miki \textit{et al}.~\cite{miki2022learning}&   ANYmal-C& \cmark&  1 (GPU)&Elevation map&  2\\ \hline 
         Agarwal \textit{et al}.~\cite{agarwal2022legged}&   Unitree A1& \xmark&  1&Depth image&  2\\ \hline 
         Yang \textit{et al}.~\cite{yang2023neural}&   Unitree A1& \xmark&  1& Depth image&  2\\ \hline 
         Hoeller \textit{et al}.~\cite{hoeller2023anymal}&   ANYmal-D& \cmark&  2& Surround pointcloud& 6\\ \hline 
		 Cheng \textit{et al}.~\cite{cheng2023parkour}&   Unitree A1& \cmark&  2& Depth image& 2\\ \hline 
         DreamWaQ++ (ours)&   Unitree Go1& \cmark&  1& Forward pointcloud&  1\\ \hline
    \end{tabular}
    
    \label{table:comparison}
\end{table*}

\subsection{Problem formulation}
We formulate the problem as a partially observable Markov decision process (POMDP) because, in the real world, the robot has no direct access to the exact state of the environment. We try to solve the problem by leveraging few shot meta--reinforcement learning (meta--RL) via task inference, which trains a separate network that can predict the task or context of the environment leveraging a few data points in conjunction with the policy network.

The environment is a POMDP defined by the tuple $\mathcal{M}=(\mathcal{S},\mathcal{O},\mathcal{A},d_0,p,r,\gamma)$. The full state, partial observation, and action are continuous, and defined by $\mathcal{\textbf{s}\in\mathcal{S}}$, $\mathcal{\textbf{o}\in\mathcal{O}}$, and $\mathcal{\textbf{a}\in\mathcal{A}}$, respectively. Generally, every environment with different physical properties, such as the robot's hardware, terrain properties, and commanded velocity, is categorized as a different POMDP sampled from a task distribution $P(\mathcal{M})$.

The environment starts with an initial state distribution, $d_0(\textbf{s}_0)$; progresses with a system dynamics $p(\textbf{s}_{t+1}|\textbf{s}_{t},\textbf{a}_{t})$; and obtains a reward, $r:\mathcal{S}\times\mathcal{A}\to\mathcal{R}$ for every action at a given state. The discount factor is defined by $\gamma\in[0,1)$. 

The goal of meta--RL in our problem setting is to learn a context encoder network, $\phi(\textbf{z}|\textbf{o},\textbf{a})$, that can infer the task in a form of a context vector, $\textbf{z}$, given available observations and actions. 
% In this paper, we define a temporal observation at time $t$ over the past $H$ measurements as $\textbf{o}^H_t=\begin{bmatrix}\textbf{o}_t & \textbf{o}_{t-1} \dots \textbf{o}_{t-H} \end{bmatrix}^T$. 

Prior works have enjoyed the benefit of task inference for fast adaptation of the learned control policy in the real world by explicitly training a context encoder that predicts some physical properties of the world, such as ground friction and restitution~\cite{kumar2021rma,lee2020learning,miki2022learning}. However, those works assumed that the contexts were available in training time. Although this relaxed assumption can facilitate learning, it also limits the solution space of the context. Moreover, as some context might not be directly identifiable from a short history of observations, the context encoder may fail to generate an informative context~\cite{xie2022robust}. 

In contrast, we trained a context encoder in an unsupervised manner. In DreamWaQ~\cite{nahrendra2023dreamwaq}, the context encoder is built upon the $\beta$--variational autoencoder ($\beta$--VAE) architecture that predicts the future observations. The advantages of leveraging $\beta$--VAE in DreamWaQ's framework are twofold. First, a higher degree of latent disentanglement induced by the $\beta$--VAE enables distinguishable task inference, which significantly helps learning and adaptation. Second, the stochastic network architecture makes the context encoder more robust to epistemic uncertainty when given out of distribution (OOD) observations.

In this work, the context encoder is trained jointly with a height reconstructor network to build a map using a stream of historical proprioceptive and exteroceptive data. This method is theoretically possible because it is built on the idea of simultaneous localization and mapping~(SLAM) where accumulated geometrical feature points along with odometry can be fused to build a map around the robot. More specifically, the context encoder in DreamWaQ++ consists of three attention mechanisms, i.e.~cross--modal, temporal, and spatial attentions.




% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable} 
\centering
% \captionsetup{font=footnotesize, singlelinecheck=false}
\caption{\textbf{Hardware comparison}. The hardware parameters are obtained by measuring the official open-sourced 3D model of the corresponding robot~\cite{unitreea1,unitreego1}.}
\label{table:hardware_comparison}
\begin{center}
\begin{tabular}{lcc}
\hline \hline
Parameter           & Unitree A1~\cite{unitreea1} & Unitree Go1~\cite{unitreego1} \\ \hline 
Total weight (kg)       & $12$ & $13$      \\ 
Base length (m)         & $0.27$ & $0.38$      \\ 
Base width (m)          & $0.19$ & $0.19$      \\ 
Base height (m)         & $0.11$ & $0.11$      \\ 
Standing height (m)     & $0.4$ & $0.4$      \\ 
Thigh length (m)        & $0.2$ & $0.2$      \\ 
Calf length (m)         & $0.2$ & $0.2$      \\ 
Max. hip torque (Nm)    & $33.5$ & $23.7$      \\ 
Max. thigh torque (Nm)  & $33.5$ & $23.7$      \\ 
Max. calf torque (Nm)   & $33.5$ & $33.5$      \\ 
 

\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

\subsection{Real-world Stair-climbing Race}\label{supp:race}
The race experiment was conducted on a long-flight of stairs. \figinitref{supp:race} visualizes the stair characteristics used in the experiment.
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_race_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Geometrical details of the stairs used for robot race experiment.}}
	\label{figure:supp_race}
\end{figure}

To support the race experiments, we conducted additional asynchronous experiments where robot R4~(Fig.~\ref{figure:supp_hardware}C) was used to deploy the controllers. Robot~R4 was also controlled with an autonomous navigation module to ensure consistent path planning while climbing the stairs. The experiments videos are summarized in \mvone0, and a few snapshots of the experiments that highlight the robot's motions are shown in Fig.~\ref{figure:supp_async_race}. Robot~R4 was controlled using (\textbf{A})~DreamWaQ++, (\textbf{B})~DreamWaQ, and (\textbf{C})~Unitree Go1's built-in controller. The robot, controlled by DreamWaQ++, managed to climb the stairs with minimum leg and body collisions by adaptively raising its body and foot swing height. In contrast, the robot controlled with DreamWaQ experienced a series of stumbles, although it managed to climb the stairs due to the robust nature of the controller. The robot controlled by the Unitree Go1's built-in controller could climb the stairs but often got stuck due to the lack of adaptability in the controller.

One discernible behavior between DreamWaQ++ and DreamWaQ lies in its gait adaptation. DreamWaQ++ adapts its gait by raising its body and swinging its foot further to step on the stairs (see Fig.~\ref{figure:supp_async_race}A), while DreamWaQ tends to collide the robot foot with the stairs and then drag it along the stair's vertical surface before placing it on the next step (see Fig.~\ref{figure:supp_async_race}B). This behavior is less efficient and may cause the robot to stumble. On the other hand, the robot with Unitree Go1's built-in controller tends to use a fixed gait pattern, which is less adaptive to the stairs' geometry and lacks spatial memory, causing its rear leg to stumble multiple times (see Fig.~\ref{figure:supp_async_race}C).

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_async_race_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Asynchronous stair-climbing experiments.} The robot was controlled using (\textbf{A}) DreamWaQ++, (\textbf{B}) DreamWaQ, and (\textbf{C})  Unitree Go1's built-in controller. The white mask on the stair indicates the same stair plate that each robot interacted with over the four successive snapshots. The full asynchronous race experiment is available in \mvone0.}
	\label{figure:supp_async_race}
\end{figure}

We also measured the state estimation error of the robot controlled by DreamWaQ++ and DreamWaQ during the asynchronous experiments. The state estimation error is the absolute error between the ground truth and estimated velocities. The ground truth data was obtained using a LiDAR odometry algorithm~\cite{xu2022fast}. The results are shown in Fig.~\ref{figure:supp_error_track}. The robot controlled by DreamWaQ++ exhibits a lower state estimation error compared to the robot controlled by DreamWaQ with a significant difference. This result indicates that the robot controlled by DreamWaQ++ can better estimate its position and adapt its gait to the stairs' geometry, which is crucial for climbing stairs efficiently, yielding a more stable and robust locomotion.

\begin{figure}[h!]
	\centering 
	\begin{subfigure}[b]{0.38\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_vel_error_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Velocity estimation error comparison in the stair-climbing task.} The **** annotation indicates a significant difference between the two controllers as measured by a paired $t$-test.}
	\label{figure:supp_error_track}
\end{figure}

\subsection{Blind locomotion on stairs}\label{supp:dreamwaq}
We evaluate the performance of a blind locomotion controller trained using DreamWaQ~\cite{nahrendra2023dreamwaq} when traversing a series of stairs with $15\!\sim\!18~\mathrm{cm}$ high rise as shown in Fig.~\ref{figure:supp_dreamwaq}. Although the robot initially managed to climb the stairs, it became unstable due to a series of stumbles and eventually fell down before reaching the end of the stairs. We discovered that the most risky stumbles were when the two front legs stumbled at the same time, making the robot lose its balance. This result highlights the importance of exteroception for a legged robot to proficiently traverse through obstacles.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_stairs_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Illustrations of blind locomotion failure in a stair-climbing scenario.} A series of stumbles made the robot cannot preserve its stability and eventually fell down.}
	\label{figure:supp_dreamwaq}
\end{figure}

\subsection{Climbing a long flight of stairs}\label{supp:long_stairs}

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_long_stairs_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Stairs climbing experiments}. The robot is commanded to climb a long flight of (\textbf{A})~straight and (\textbf{B})~curved stairs.}
	\label{figure:supp_long_stairs}
\end{figure}

\figinitref{figure:supp_long_stairs}E shows snapshots of the robot climbing $39$ steps of stairs, yielding a total elevation of $5.46~\textrm{m}$ and inclination of $25.76^{\circ}$. We used a blind locomotion controller trained using DreamWaQ as a baseline comparison. While the blind locomotion controller initially managed to overcome the stairs, its performance quickly deteriorated due to numerous stumbles (see supplementary section~\ref{supp:dreamwaq}). In contrast, the controller trained using DreamWaQ++ (Fig.~\ref{figure:supp_long_stairs}E) allowed the robot to swiftly climb the stairs with minimum leg and body collisions by adaptively raising its body and foot swing height. The robot reached the top of the stairs in $47~\textrm{s}$, stressing the importance of exteroception on locomotion over a long flight of stairs that necessitates fast adaptation of the robot's gait to minimize stumbles.

\subsection{Paired $t$-test on slope climbing}\label{supp:t-test}
The significance of the difference between torque exertion of each joint in Fig.~\ref{figure:results_adaptation}F was measured using a paired $t$-test method. The annotations on the figure are defined based on the resulting $p$-values. We follow the standard rule defined in Table~\ref{table:t-test}. The $p$-values were corrected using the Bonferroni correction method~\cite{florian_charlier_2022_7213391} and presented in Table~\ref{table:p-value}.

% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\caption{Description for $p$-value annotation~\cite{florian_charlier_2022_7213391}.}
\centering
% \captionsetup{justification=centering}

\label{table:t-test}
\begin{center}
\begin{tabular}{lll}
\hline \hline
Annotation           & Criteria \\ \hline 
ns (not significant)  &                      $0.05 < p \leq 1.0$ \\
$*$  &                      $0.01 < p \leq 0.05$ \\
$**$  &                      $0.001 < p \leq 0.0$ \\
$***$  &                      $0.0001 < p \leq 0.001$ \\
$****$  &                      $ p \leq 0.0001$ \\
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\centering
% \captionsetup{justification=centering}
\caption{$p$-value results of data reported in Fig.~\ref{figure:results_adaptation}.}
\label{table:p-value}

\begin{center}
\begin{tabular}{llc}
\hline \hline
Joint           & $p$-value & Signficance \\ \hline 
FR Thigh  &                      $1.0$ 			& ns\\  
FR Calf  &                      $0.4464$ & ns\\  
FL Thigh  &                      $1.0$ & ns\\  
FL Calf  &                      $1.0$ & ns\\  
RR Thigh  &                      $0.001244$ & **\\  
RR Calf  &                      $0.00009325$ & ****\\  
RL Thigh  &                      $0.00001922$ & ****\\  
RL Calf  &                      $1.0$ & ns\\  
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================


\subsection{Exteroception preprocessing}\label{supp:exteroception_preprocessing}
In this work, we employ a voxel grid representation as the input for the policy. The voxel grid encompasses downsampled robot-centric 3D points obtained from an exteroceptive sensor mounted on the robot. The voxels are obtained via voxel-grid filtering with a leaf size of $0.05~\mathrm{m}$. We assume accurate extrinsic calibration parameters are available to transform the measured 3D points from the sensor frame to the body frame. We set the exteroceptive measurements to be within a grid with its row and column size of $w\!=\!1.1~\mathrm{m}$ and $h\!=\!0.5~\mathrm{m}$, respectively. The first row of the grid is located $0.9~\mathrm{m}$ in front of the robot, yielding a grid with 10 rows and 22 columns by dividing the size with the leaf size.

\subsection{Constrained reparameterization trick}\label{supp:constrained_reparam}
The multi-modal encoder architecture encompasses multiple stochastic layers within the encoders and multi-modal mixer networks, offering advantages such as enhanced robustness and increased exploration capabilities. However, a trade-off arises with numerical stability during the early stages of training. 

A straightforward solution is to balance the weight of the reconstruction loss and KL divergence in $\mathcal{L}_\mathrm{VAE}$. In variational inference, the prior distribution of the latent state is often assumed to follow a normal distribution. The stability issue can be mitigated by putting more emphasis on the latent loss during training. This approach ensures that the encoder learns a better approximation of the latent space while preserving the ability to reconstruct the input data accurately.

However, strongly matching the posterior and prior distributions via the latent loss can lead to another issue where the encoder tends to neglect important details in the input point cloud. This deficiency makes the policy unable to detect and respond to small obstacles in the environment effectively. To overcome this challenge, we introduced a constrained reparameterization trick, defined as

\begin{equation}
    \textbf{z} \sim N(g_{\mu}(\textbf{x}),g_{\sigma}(\textbf{x})),
\end{equation}
where $\textbf{z}$ is a stochastic latent vector and $\textbf{x}$ is the input of the encoder network $g$. The subscripts $\mu$ and $\sigma$ indicate the outputs of $g(x)$ that correspond to the mean and standard deviation of the latent distribution, respectively. $z$ is sampled from a Gaussian distribution $N(\cdot,\cdot)$ with mean $g_{\mu}(\textbf{x})$ and standard deviation $g_{\sigma}(\textbf{x})$. 

During this reparameterization step, we imposed hard constraints on the standard deviation of the distribution, such that $\sigma_\mathrm{min}\leq g_{\sigma}(\textbf{x}) \leq \sigma_\mathrm{max}$. This constraint ensures that the generated samples are numerically stable and can be reliably propagated to the subsequent layers of the network. By implementing this simple yet effective solution, the learning process becomes much more stable without compromising the final performance of the learned policy. Empirically, we set $\sigma_\mathrm{min}=0$ and $\sigma_\mathrm{max}=5$ to promote stable training. This constrained reparameterization trick is employed on all encoder networks that utilize a stochastic layer.


\subsection{Training environment details} \label{supp:training_env}
\subsubsection{\textit{Simulation}}
We used NVIDIA Isaac Gym~\cite{makoviychuk2021isaac} preview 3 as the simulator for training the controller and multi-modal context encoder networks. The training environments were built upon the Legged Gym library~\cite{rudin2021learning}. We employed domain randomization over $3,\!500$ agents, which took about 11 hours of training on an NVIDIA A5000 GPU. Afterwards, the trained networks were deployed without any fine-tuning on a real or simulated robot in the Gazebo simulation for the evaluations presented in this paper. 

\subsubsection{\textit{Control pipeline}}
The policy and multi-modal context encoder networks ran synchronously while receiving asynchronous observations. Proprioceptive measurements were sampled at $200~\textrm{Hz}$, whereas exteroceptive measurements were sampled at $10~\textrm{Hz}$. The controller integrated the most recent measurements, operating at $50~\textrm{Hz}$. To enhance the robustness of the controller against the asynchronous observations, we employed latency randomization during training. Detailed information regarding the randomized latency for all measurements is provided in Table~\ref{table:domain_randomization}.

The policy network generated target joint positions at a rate of $50~\textrm{Hz}$, which were subsequently transmitted to a low-level proportional-derivative (PD) controller operating at $200~\textrm{Hz}$. Within the PD controller, the target joint positions were converted into torque commands, employing proportional ($K_p$) and derivative ($K_d$) control gains of $25$ and $0.7$, respectively. These computed torque commands were subsequently relayed to the low-level motor controller integrated within our customized Unitree Legged SDK.


% \begin{itemize}
%     \item \textbf{Rough slopes} are generated by
%     \item \textbf{Stairs}
%     \item \textbf{Gaps}
%     \item \textbf{Random discrete}
% \end{itemize}

\subsubsection{\textit{Curriculum}}
We leveraged three curriculums during training, i.e.~terrain, command, and reward curriculums. For the terrain curriculum, several terrains were procedurally generated at the beginning of training to simulate various obstacles the robot might encounter in the real world. The terrain curriculum utilized the game-inspired curriculum setting~\cite{rudin2021learning} with ten different levels of difficulty. We generally utilized \texttt{rough}, \texttt{stairs}, \texttt{gaps}, and \texttt{discretized obstacle} terrains to introduce variations in the exteroception, which could induce diversity in the training data for the multi-modal context encoder. An agent was promoted to the next level if it could traverse more than half of the distance at the current level. When an agent failed to traverse more than half of the distance at the current level for more than ten episodes, it was demoted to the previous level. If an agent successfully walked through all levels, it will be randomly spawned within the ten levels, preventing catastrophic forgetting and diversifying the training data.
 
The policy was trained to maximize the command tracking rewards while satisfying style rewards (Table~\ref{table:reward_functions}), resulting in smooth and accurate robot motion. The curriculum was a reward-based one, which automatically increased the command velocity range when the velocity tracking reward, $r_{v_{x,y}}\in[0, 1]$, surpassed a given threshold, $r^\textrm{thres}_{v_{x,y}}$, which was set to $0.9$. 

Finally, the reward curriculum ensures safe behavior in the real world by gradually increasing the penalty for the style rewards. Applying strong penalties to the style rewards at early training can restrict exploration, resulting in poor performance. However, without a strong penalty, the robot tends to behave aggressively once noisy exteroceptive measurements are taken as inputs in the real world. Hence, a reward curriculum that exponentially grows over learning iteration was utilized to facilitate stable learning. More details are provided in section~\ref{supp:reward_functions}.

\subsubsection{\textit{Domain randomization}}
We randomized multiple physical properties of the robot and the environment to facilitate sim--to--real transfer. Additionally, we employed Roll-Drop~\cite{campanaro2023roll} to encourage exploration and robustness on top of physics randomization. Details of the physical properties and its randomization ranges are provided in Table~\ref{table:domain_randomization}.

\begin{table}[t!]
\centering
% \captionsetup{justification=centering}
\caption{Domain randomization ranges applied in the simulation.}
\label{table:domain_randomization}
\begin{center}
\begin{tabular}{lccc}
\hline\hline
Parameter                        & Randomization range & Unit \\\hline
Payload                     & $[-1, 2]$ & $\mathrm{~kg}$     \\ 
$K_p$ factor   & $[0.9, 1.1]$ & $\mathrm{~Nm~rad^{-1}}$    \\ 
$K_d$ factor        & $[0.9, 1.1]$ & $\mathrm{~Nms~rad^{-1}}$   \\ 
Motor strength factor        & $[0.9, 1.1]$ & $\mathrm{~Nm}$   \\ 
Center of mass shift        & $[-50,50]$ & $\mathrm{~mm}$    \\
Friction coefficient        & $[0.2, 1.25]$ & -    \\
System delay                        & $[0.0, 15.0]$ &  $\mathrm{~ms}$   \\


\hline\hline
\end{tabular}
\end{center}
\vspace{-0.cm}
\end{table}


\subsubsection{\textit{Adversarial observation}}
We injected noises into the proprioceptive and exteroceptive observations. For the proprioceptive observations, a uniform noise was injected at each time step. 
% The magnitude of noises for each observation \rvc{is} summarized in Table~\ref{table:observation_noise}. 
For the exteroceptive data, we classified three different noise ranges, constituting low, medium, and high noises. The proportion of these exteroceptive noise scales was set to $30\%$, $50\%$, and $20\%$, respectively.
The magnitude of noises for each observation is summarized in Table~\ref{table:observation_noise}. 

\begin{table}[t!]
\centering
% \captionsetup{justification=centering}
\caption{Noise parameters injected into the observation for the policy network during training.}
\label{table:observation_noise}
\begin{center}
\begin{tabular}{lccc}
\hline\hline
Observation                        & Noise range ($\mu$) & Unit \\\hline
Joint position  &                      $[-0.01, 0.01]$ & $\mathrm{rad}$     \\ 
Joint velocity  &                      $[-1.5, 1.5]$ & $\mathrm{rad/s}$    \\ % $\mathrm{rad~s^{-1}}$    \\ 
Body linear velocity &                 $[-0.1, 0.1]$ & $\mathrm{m/s}$   \\ % $\mathrm{m~s^{-1}}$   \\ 
Body angular velocity &                $[-0.2, 0.2]$ & $\mathrm{rad~^{-1}}$   \\ 
Gravity vector        &                $[-0.05, 0.5]$ & $\mathrm{m/s^{2}}$    \\ % $\mathrm{m~s^{-2}}$    \\
Exteroceptive measurement (low)  &     $[0.0, 0.03]$ & $\mathrm{m}$\\
Exteroceptive measurement (medium)  &     $[0.03, 0.1]$ & $\mathrm{m}$    \\
Exteroceptive measurement (high)  &     $[0.1, 0.3]$ & $\mathrm{m}$    \\


\hline\hline
\end{tabular}
\end{center}
\vspace{-0.cm}
\end{table}


Although observation noise is often easily handled by a controller that leverages only proprioception if trained with sufficient domain randomization,  the learned controller exhibited increased sensitivity to disturbances in exteroception, primarily attributed to the rich information contained within exteroceptive measurements. Several issues, such as inaccurate extrinsic calibration and sensor noise, significantly deteriorated the controller's robustness. In robotics, auto-calibration is a highly desirable attribute, capable of enhancing system robustness. Consequently, we aimed to integrate this capability into the proposed multi-modal context encoder.

To achieve this, we trained the multi-modal context encoder to explicitly predict extrinsic calibration errors within the exteroception data. This explicit error prediction serves a dual purpose within our framework. First, it provides guidance to human operators, enabling them to recalibrate the extrinsic parameters effectively. Concurrently, the multi-modal context encoder learns to discern and mitigate the impact of this calibration error, thus producing more accurate exteroception reconstructions. This proactive approach enhances the overall performance and resilience of the proposed system in the presence of exteroceptive disturbances.

Throughout the training process, we introduced a randomization procedure for the extrinsic calibration parameters within the $SE(3)$ coordinate system at the beginning of each episode. These calibration parameters served as ground-truth values, challenging the multi-modal context encoder to predict them accurately. We proposed a customized perturbation model for the exteroception because we are exploiting the robot-centric height scan as the input for the encoder. The perturbation model consists of i) noise, ii) sensor alignment error, and iii) pruning.

\paragraph{Noise model}
The noise model is designed to mimic the characteristics of range measurement sensors such as LiDAR \rvc{sensors} or depth cameras. First, the distance between the sampled 3D robot-centric points to the body frame of the robot is measured as $\textbf{d}_t=[d^1_t\;\cdots{}\;d^i_t\;\cdots{}\;d^I_t] \in \mathbb{R}^{1 \times I}$, where $i$ indicates the $i$-th element and $I$~is the number of points per scan. 
Then, for the $i$-th point, an anisotropic Gaussian noise is applied to the point set $\textbf{p}_t=[\textbf{p}^1_t\;\cdots\;\textbf{p}^i_t\;\cdots\;\textbf{p}^I_t]\in\mathbb{R}^{3 \times I}$, where $\textbf{p}^i_t=\begin{bmatrix} x^i_t & y^i_t &  z^i_t \end{bmatrix}$. The Gaussian noise is centered at the nominal noise level, and the variance is scaled according to the distance of each point to the robot. Practically, exteroceptive measurements in the real world exhibit higher noise when the terrains are very close to the sensor. Therefore, we formulate each noisy point as

\begin{equation}
    \textbf{p}^i_t = 
    \begin{bmatrix}
    x^i_t + \mathcal{N}\left(\mu_x, \sigma^2_x\right)\\
    y^i_t + \mathcal{N}\left(\mu_y, \sigma^2_y\right)\\
    z^i_t + \mathcal{N}\left(\mu_z, \sigma^2_z\right)\\
    \end{bmatrix},
    \label{eq:noise_model}
\end{equation}
where $\mu$  and $\sigma^2$ are the nominal noise level and noise variance, respectively, with the subscripts $x$, $y$, and $z$ indicating that the elements correspond to the $x$, $y$, and $z$ axes. These noise parameters were sampled from a uniform distribution within the range specified in Table~\ref{table:point_noise} at the beginning of every episode. Afterwards, the point-wise noise in~\eqref{eq:noise_model} was sampled at every time step.

\begin{table}[t!]
\centering
% \captionsetup{justification=centering}
\caption{Point noise parameters during training.}
\label{table:point_noise}
\begin{center}
\begin{tabular}{cccc}
\hline\hline
Parameter                        & Range & Unit \\\hline
$\mu_x$  &                      $[0.0, 2.0]$ & $\mathrm{cm}$     \\ 
$\mu_y$  &                      $[0.0, 2.0]$ & $\mathrm{cm}$    \\ % $\mathrm{rad~s^{-1}}$    \\ 
$\mu_z$ &                       $[0.0, 5.0]$ & $\mathrm{cm}$   \\ % $\mathrm{m~s^{-1}}$   \\ 
$\sigma_x$ &                    $[0.0, 1.0]$ & $\mathrm{cm}$   \\ 
$\sigma_y$        &             $[0.0, 1.0]$ & $\mathrm{cm}$    \\ % $\mathrm{m~s^{-2}}$    \\
$\sigma_z$  &                   $[0.0, 3.0]$ & $\mathrm{cm}$\\


\hline\hline
\end{tabular}
\end{center}
\vspace{-0.cm}
\end{table}


\paragraph{Sensor alignment bias}
We applied sensor alignment bias at the beginning of each episode to simulate extrinsic calibration error. This error included positional and rotational errors, i.e. $\begin{bmatrix} \Delta x, & \Delta y, & \Delta z, & \Delta \mathrm{roll}, & \Delta \mathrm{pitch}, & \Delta \mathrm{yaw} \end{bmatrix}$. The alignment errors were sampled from a uniform distribution and consistently applied to the measured points throughout the episode. The alignment bias parameters are summarized in Table~\ref{table:alignment_bias}.


% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\centering
\captionsetup{singlelinecheck=false}
\caption{Sensor alignment bias between the body frame of exteroceptive sensor and robot.}
\label{table:alignment_bias}

\begin{center}
\begin{tabular}{ccc}
\hline \hline
\multicolumn{1}{c}{Parameter} & Error range & Unit  \\\hline 
$\mathrm{roll}$             & $[-0.2, 0.2]$ &  $\mathrm{rad}$   \\
$\mathrm{pitch}$            & $[-0.15, 0.15]$ &  $\mathrm{rad}$   \\
$\mathrm{yaw}$              & $[-0.1, 0.1]$ &  $\mathrm{rad}$   \\
$\mathrm{x}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
$\mathrm{y}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
$\mathrm{z}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
\hline \hline      
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

\paragraph{Pruning}
The major distinction between the height scans sampled in simulation and those obtained from real-world exteroceptive sensors is the presence of inherent blind spots in the latter. These blind spots can result from either the sensor's specifications or its placement on the robot, leading to occlusion by certain robot parts. One of the possible solutions to this problem is by employing raycasting from the sensor pose to the sampled height scan. However, this solution can be computationally expensive and greatly affect simulation time. In this work, we employed a simpler solution to eliminate or \textit{prune} parts of the exteroceptive data before it was fed into the multi-modal context encoder.

First, we construct a probability masking layer to prune the exteroceptive measurement that has been preprocessed using the method detailed in section~\ref{supp:exteroception_preprocessing}. During locomotion on the flat terrain, appropriately positioned exteroceptive sensors should effectively measure the terrain within a pre-defined grid area. However, the reliability of these measurements diminishes when the robot encounters obstacles or pits. To address this challenge, we introduced a probability masking technique that assigns a higher pruning probability to points that are distant and elevated or close and low to the robot. This pruning strategy makes a setting that allows the multi-modal context encoder to learn point completion from sparse exteroceptive inputs.

\subsubsection{\textit{Privileged states}}
For the privileged exteroception, we use a robot-centric local height map sampled around the robot. The local map is a 2.5D grid, where each value of the grid represents the height of the terrain on the corresponding grid. The grid is constructed with its row and column size of $w\!=\!1.1~\mathrm{m}$ and $h\!=\!1.7~\mathrm{m}$, respectively. The first row of the grid is located $0.9~\mathrm{m}$ in front of the robot's body frame, similar to the 3D voxel grid for the multi-modal encoder's input. The resolution of the grid is set to $5~\mathrm{cm}$.

For the privileged proprioception, we provide ground truth and noiseless measurements as follows:
\begin{enumerate}
    \item Gravity vector on the robot's body frame.
    \item Body linear and angular velocities.
    \item Joint positions and angular velocities.
    \item External disturbance force and torque applied to the robot's body frame.
    \item Physical properties (friction, motor damping, motor stiffness, motor strength ratio, additional payload, and the robot's center of mass).
    \item Foot position relative to the robot's body frame.
\end{enumerate}


\subsection{Reward functions}\label{supp:reward_functions}
Table~\ref{table:reward_functions} lists all the reward functions,~$\textbf{r}$, used in DreamWaQ++, which are mainly based on the rewards used in~\cite{nahrendra2023dreamwaq}. On top of these rewards, we also employed a reward curriculum to exponentially anneal some style rewards, i.e.~joint torque, joint velocity, joint acceleration, action rate, and smoothness rewards. The annealing rule follows the following formula:

\begin{equation}
    w_{i+1}=\lambda w_{i},
\end{equation}
where $w$ is the reward weight, $i$ is the learning iteration, and $\lambda$ is the annealing rate. We set $\lambda\!=0.998$
and $w_0$ for the selected skill rewards are summarized in Table~\ref{table:reward_init}.
% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable} 
\centering
\captionsetup{singlelinecheck=false}
\caption{Reward function elements and their corresponding weights. $\mathrm{exp(\cdot)}$ and $\mathrm{var(\cdot)}$ are exponential and variance operators, respectively. $(\cdot)^\mathrm{des}$ and $(\cdot)^\mathrm{cmd}$ indicate the desired and commanded values, respectively. $x, y,$ and $z$ are defined on the robot's body frame, with $x$ and $z$ pointing forward and upward, respectively. $\textbf{g}$, $\textbf{v}_{xy}$, $\omega_\mathrm{yaw}$, $h$, $p_{f,z,k}$, $v_{f,xy,k}$, and $\boldsymbol{\tau}$ are the gravity vector projected into the robot's body frame, linear velocity vector in the $xy$ plane, yaw rate, body height w.r.t. the ground, foot height, foot lateral velocity, and joint torque, respectively.}
\label{table:reward_functions}



\begin{center}
\begin{tabular}{lll}
\hline \hline
Reward           & Equation ($\textbf{r}$) & Weight ($w$) \\ \hline 
\multicolumn{3}{l} {\textit{Task rewards}}           \\ 
Lin. velocity tracking  & $\exp{\{-4(\textbf{v}^\mathrm{cmd}_{xy}-\textbf{v}_{xy})^{2}\}}$ & $1.0$      \\ 
Ang. velocity tracking & $\exp{\{-4(\omega^\mathrm{cmd}_\mathrm{yaw}-\omega_\mathrm{yaw})^{2}\}}$ & $0.5$ \\ \hline
\multicolumn{3}{l} {\textit{Style rewards}}           \\ 
Linear velocity ($z$) & $v^2_z$ & $-2.0$ \\
Angular velocity ($xy$) & $\boldsymbol{\omega}^2_{xy}$ & $-0.05$ \\
Uprightness & $|\textbf{g}|^2$ & $-0.2$ \\
Joint acceleration & $\boldsymbol{\ddot{\theta}}^2$ & $-2.5\!\times\!10^{-7}$ \\
Joint power & $|\boldsymbol{\tau}||\boldsymbol{\dot{\theta}}|$ & $-2\!\times\!10^{-5}$ \\
Body height & $(h^\text{des}-h)^2$ & $-1.0$ \\
Foot clearance & $(p^\text{des}_{f,z,k}-p_{f,z,k})^2\cdot v_{f,xy,k}$& $-0.01$ \\
Action rate & $(\textbf{a}_t - \textbf{a}_{t-1})^2$ & $-0.01$ \\
Smoothness & $(\textbf{a}_t - 2\textbf{a}_{t-1} + \textbf{a}_{t-2})^2$& $-0.01$ \\
Power distribution &$\mathrm{var}(\boldsymbol{\tau}\cdot\boldsymbol{\dot{\theta}})^2$ & $-10^{-5}$ \\ 
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\centering
\captionsetup{singlelinecheck=false}
\caption{Initial weight $w_0$ for selected style rewards that were annealed using the reward curriculum.}
\label{table:reward_init}



\begin{center}
\begin{tabular}{lll}
\hline \hline
Reward           & Weight ($w_0$)\\ \hline 
Joint torque & $-5\!\times\!10^{-6}$ \\
Joint velocity & $-6\!\times\!10^{-6}$ \\
Joint acceleration & $-7.5\!\times\!10^{-8}$ \\
Action rate & $-1.5\!\times\!10^{-5}$ \\
Smoothness & $-1.5\!\times\!10^{-5}$ \\
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================


\subsection{Embedding analysis}\label{supp:embedding_analysis}
\subsubsection{Evaluation setting}
We conducted an embedding analysis on the context vector generated by the encoder. This analysis was carried out using data acquired within a simulation-to-simulation (sim-to-sim) setup. In this setup, both the fully trained encoder and policy networks were deployed within a Gazebo simulator. We implemented four distinct terrain types to facilitate this evaluation, as depicted in Fig.~\ref{figure:supp_gazebo_terrain}. In this setting, the stair difficulties are parameterized by its \textit{rise} and \textit{run}, i.e.~its vertical and horizontal dimensions, respectively~\cite{barasuolstair}. Easy stairs have low rise and high run values, while hard stairs have high rise and low run values.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/gazebo_terrain_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Illustrations of terrains used for evaluation in the Gazebo simulator.} Four types of terrains were constructed to evaluate the change in values of the context features. 
    % Four types of terrains were constructed to evaluate the changes in values of the context features. 
    The world model employed for this evaluation is an adapted version of the simulation model utilized in the IEEE ICRA 2023 Autonomous Quadrupedal Robot Challenge~\cite{jacoff2023taking}.}
	\label{figure:supp_gazebo_terrain}
\end{figure}

\subsubsection{Visualization via dimension reduction}
We performed dimensionality reduction on the proprioceptive, exteroceptive, and multi-modal contexts to depict their distributions within a 2D space. While one of the prevailing approaches for embedding visualization involves t-distributed stochastic neighbor embedding (t-SNE)~\cite{van2008visualizing}, it is worth noting that t-SNE, despite yielding satisfactory cluster visualizations, is notably less efficient at capturing overarching embedding structures. Its emphasis lies predominantly on local structures, potentially leading to inadequate comprehension of meaningful information within multi-modal data. Consequently, this limitation of t-SNE may hinder the comprehensive insights required for thorough analysis.

Hence, we extended our approach to dimensionality reduction by employing PaCMAP~\cite{wang2021understanding}, a recently introduced technique that offers a more balanced preservation of both local and global embedding structures. In this manner, we achieved visualizations of the embeddings within a 2D space for diverse terrains (as exemplified in Fig.~\ref{figure:supp_gazebo_terrain}). The visualization results are presented in Fig.~\ref{figure:supp_embedding_noblind}.


\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_noblind_embedding_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{2D visualization of the embeddings after dimensionality reduction.}}
	\label{figure:supp_embedding_noblind}
\end{figure}


As anticipated, the t-SNE method effectively portrays the exteroceptive context, revealing discernible clusters that imply the disentangled latent representation of different terrains. However, interpreting the proprioceptive context poses challenges in providing a coherent understanding. Consequently, the visualization of the multi-modal context fails to yield significant insights, aside from distant clusters indicative of varying terrains encoded in the exteroceptive context.

Meanwhile, PaCMAP more explicitly captures fundamental intrinsic characteristics of the embedding~\cite{wang2021understanding}. Within the proprioceptive context, PaCMAP effectively illustrates circular clusters, which plausibly correspond to the cyclic gait patterns exhibited by the robot's feet. An interesting observation arises as the circular radius expands on less challenging terrains. Our conjecture aligns with the notion that this radius could indicate the gait's duty cycle or swing time, as on smoother terrains without obstacles, the robot's feet undergo extended swing durations.

Our embedding analysis showcases that the structured representation learning facilitated by our context encoder yields informative latent variables without necessitating explicit estimation of physical attributes. As postulated by Nahrendra \textit{et al.}~\cite{nahrendra2023dreamwaq}, the unsupervised representation learning mechanism empowers the encoder to encode informative latent features while maintaining dynamic feature interactions selectively. The mechanism inherent in our context encoder thus amalgamates the best of both approaches, eliminating the requirement for manual and explicit selection of estimated variables while concurrently generating structured and disentangled latent representations.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_blind_embedding_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{2D visualization of the dimension-reduced embeddings during blind locomotion.}}
	\label{figure:supp_embedding_blind}
\end{figure}

We extended our embedding analysis to the blind locomotion scenario using our framework. In this assessment, we collected data by disabling exteroception, providing constant flat terrain points, and commanding the robot to walk across various terrains, as depicted in Fig.~\ref{figure:supp_embedding_blind}. The t-SNE visualization outcomes, while potentially sufficient for the policy network, remain less straightforward for practical interpretation. Such results could mislead practitioners into erroneously concluding that the encoder has not effectively learned a disentangled context vector.

In contrast, the PaCMAP visualization method successfully captures meaningful structures within the proprioceptive context. During blind locomotion, the proprioceptive context plays an important role because it remains the sole modality that the policy can rely on. As illustrated in Fig.~\ref{figure:supp_embedding_blind}, the proprioceptive context captures local structures induced by the robot's feet motions similar to the non-blind scenario. This distinctiveness becomes more discernible upon mixing into a multi-modal context, even when fused with the false exteroceptive context obtained in the blind locomotion scenario.

\subsubsection{Effect of contrastive loss}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_contrastive_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Effect of contrastive loss in the learned embedding.} The embeddings are recorded from locomotion on flat, irregular, easy stairs, and hard stairs terrains. The comparison shows the nature of the embedding when the contrastive loss is removed or retained.}
	\label{figure:supp_contrastive}
\end{figure}

We further investigated the impact of the contrastive loss on the learned embedding. The contrastive loss is a crucial component in training the multi-modal context encoder because it encourages the encoder to learn a structured representation. To evaluate the effect of the contrastive loss, we trained the encoder without the contrastive loss and compared the learned embeddings with those obtained from the full training setup using the contrastive loss. The results are depicted in Fig.~\ref{figure:supp_contrastive}.

The comparison showed that the contrastive loss significantly influences the learned embedding. The embeddings obtained from the full training setup exhibit more structured and disentangled latent variables than those obtained without contrastive loss. Indeed, some structured patterns in the embeddings are still discernible without the contrastive loss, mostly attributed to the exteroceptive data that provides spatial information. However, it fails to capture lower-level circular patterns in the proprioceptive data, which is crucial for the robot's locomotion. This observation underscores the importance of contrastive loss in the training of the multi-modal context encoder, as it facilitates the learning of structured and disentangled latent variables essential for the robot's locomotion.


\subsubsection{Attribution of latent variables}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_attribution_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Boxplot of each embedding variable in the multi-modal context vector.} The embeddings are recorded from locomotion on \textbf{(A)} flat, \textbf{(B)} irregular, \textbf{(C)} easy stairs, and \textbf{(D)} hard stairs terrains.}
	\label{figure:supp_embedding_attribution}
\end{figure}
We utilized boxplots to portray the raw embedding values, facilitating the analysis of their distribution as the robot navigates diverse terrains. The boxplot depicted in Fig.~\ref{figure:supp_embedding_attribution} reveals intriguing trends within the exteroceptive context. Particularly noteworthy are four embedding variables ($41$, $42$, $55$, and $64$th embeddings) exhibiting significantly expansive distributions. We posit that these characteristics are closely tied to the robot's foot motion while traversing terrains of varying complexities. To substantiate this hypothesis, we conducted an experiment involving scaling these four embedding variables before being fed to the policy network. This scaling operation involved adjustments of $0.1$ and $3.0$ times their original values to investigate the effect that it may bring to the robot's foot motions.


\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/latent_modulation_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Latent modulation on some of the exteroceptive embedding proportionally affects the gait height.} The robot exhibits different locomotion styles when particular latent variables ($41$, $42$, $55$, and $64$th embeddings) were scaled with (\textbf{A}) $0.1$, (\textbf{B}) $1.0$, and (\textbf{C}) $3.0$ times of its original value. The difference resulted from this modulation is observable from the FR foot's $z$ position w.r.t. the base as shown in Fig.~\ref{figure:results_terrain}C.}
	\label{figure:supp_latent_modulation}
\end{figure}

This discovery shown in Fig.~\ref{figure:supp_latent_modulation} emphatically underscores the efficacy of structured representation learning, wherein essential physical attributes are embodied via an unsupervised approach. Moreover, this behavior offers a novel insight into the realm of interpretable learning-based control, countering the conventional notion of modern deep reinforcement learning as a ``black box'' system devoid of user-accessible modulations. Our findings demonstrate that structured representation learning engenders the acquisition of structured embeddings that can be flexibly modulated, enabling the generation of diverse behaviors by manipulating the intermediate embedding variables. This property opens up compelling possibilities for bridging the gap between learned locomotion controllers and their model-based counterparts. It also enables intuitive tuning by a human operator or a higher-level planner. 

Importantly, this property naturally emerged and was not explicitly specified during training or in the input command for the controller, distinguishing our work from that of Margolis~\textit{et al}.~\cite{margolis2022walk} that explicitly gives a style command into the policy network. Instead, this interpretable latent structure arose from the structured representation learning facilitated by the multi-modal context encoder within the proposed framework. 

However, we note that while the observed trend remains consistent, the indices of the modulated latent and its scale consistently change with different training seeds. This variability is expected because we do not enforce the learning of these variables in a supervised manner. 

% Instead, these variables are acquired through an unsupervised yet structured learning framework of the multi-modal context encoder, which enables the discovery of interpretable latent variables.

\subsubsection{Embedding feature-wise cross-correlation}
The heatmap plots shown in Fig.~\ref{figure:results_terrain}D underscore the efficiency of the multi-modal context encoder, which dynamically encodes multi-modal perception without any bias toward a particular modality. The multi-modal context encoder adaptively shifts its attention to modalities that provide the most informative priors for the policy. Furthermore, the notion of cross-modal correlation introduces interpretability on the uncertainties faced by the context encoder. This uncertainty measurement is particularly beneficial for higher-level modules. For instance, the uncertainty measurement can be leveraged by a traversability mapping module to adaptively shift its reliance on different sensor modalities for map update.


\subsection{Sensor--agnostic deployment}\label{supp:sensor_agnostic}
A fundamental strength of the policy trained using DreamWaQ++ is its sensor-agnostic property. The policy and context encoder were jointly trained in the simulation without any specific sensor model but only leveraged 3D points scan in front of the robot. Hence, the learned networks can be deployed on the real robot without any further training procedure. The only calibration required is the extrinsic parameters that transform 3D points from the sensor to the robot's body frame. This approach makes our method more simple and efficient than other existing works that rely on distilling a teacher policy into a student policy to bridge the gap between simulation and real-world exteroception. Furthermore, given that the context encoder was trained using 3D points as its input, it does not require any assumption on the number of points or grids. Instead, it will learn to infer the reliability of the exteroception and construct an informative latent feature for the policy. 

We performed an experiment using robot R3 to verify the adaptability of the learned controller to different sensor configurations. In this experiment, we built a local map surrounding the robot because we had access to stronger computation power, as well as an onboard LiDAR sensor on robot~R3. We constructed a local map of size $1.7\;\mathrm{m}\times1.1\;\mathrm{m}$ with a $0.1\;\mathrm{m}$ resolution. 

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_sensor_agnostic_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Sensor agnostic deployment.} (\textbf{A}) Adaptability of the perception networks in different exteroceptive data settings. Despite the controller being trained solely with front-facing points, as depicted in Fig.~\ref{figure:dreamwaqpp}, it demonstrates adaptability to 3D point inputs that encompass the robot (illustrated with red points). The reconstruction of these points (represented by blue points) accurately captures the geometric properties of the robot's surroundings.} (\textbf{B})~A real-world stair-climbing experiment, which validates the adaptability of the controller when different exteroceptive configurations are used for the controller.
	\label{figure:supp_sensor_agnostic}
\end{figure}

\figinitref{figure:supp_sensor_agnostic}A shows the local map input (red dots) and its reconstruction (blue dots). Despite never trained with such exteroceptive setting, the encoder and decoder networks can still reconstruct the map with a satisfactory accuracy. The adaptability of the controller was further verified through a stair-climbing experiment in Fig.~\ref{figure:supp_sensor_agnostic}B. The robot can resiliently climb the stairs and by utilizing a wider, yet sparse exteroceptive information, which has never been encountered during training.

\subsection{Details of hierarchical memory}\label{supp:hierarchical_memory}
The closest approach to our hierarchical memory approach is the neural scene representation method~\cite{hoeller2022neural}, where the robot's local map is reconstructed by introducing an autoregressive structure for predicting and generating the 3D reconstruction of the local map. The neural scene representation network receives the robot frame's transformation from a separate odometry module, current measured points, and previous 3D reconstruction. The key difference in our method is that we employed autoregression solely for explicit estimation of the $SE(3)$ transformation of the body frame of the robot over time. Our proposed method does not require a complex reconstruction method with high capacity network, but still able to provide a temporally dense exteroception.

This estimated transformation is then utilized to transform the last observed points into the robot's current frame. The $SE(3)$ transformation is available at each control loop iteration via the state estimation network, enabling temporal interpolation of the latest exteroceptive measurements. This interpolation forms the basis of a memory structure, which is subsequently fed into the exteroceptive encoder. The exteroceptive observation is formally defined as

\begin{equation}
  \textbf{o}^{\mathrm{e},K}_t = \textbf{o}^\mathrm{e}_t \concat \hat{\textbf{o}}^\mathrm{e}_{t-1} \concat \cdots \concat \hat{\textbf{o}}^\mathrm{e}_{t-K}, 
\end{equation}
 where $\textbf{o}^\mathrm{e}_t$ is the most recent exteroceptive observation at time $t$. $\hat{\textbf{o}}^\mathrm{e}_{t-K}$ is the previous exteroceptive observation at $t-K$, which has been transformed to the robot's body frame at time $t$, which is defined as
\begin{equation}
  \hat{\textbf{o}}^\mathrm{e}_{t-K} = \prescript{t}{t-K}{T}^{-1}\cdot \textbf{o}^\mathrm{e}_{t-K},
\end{equation}
where $\textbf{o}^\mathrm{e}_{t-K}$ is the exteroceptive observation measured at time $t-K$, and $\prescript{t}{t-K}{T}$ is the $SE(3)$ transformation of the robot's pose from time $t$ to $t-K$. 
% 

% By doing so, our approach yields a lightweight architecture that retains some memory of the exteroceptions without necessitating memory-based networks.

\subsection{Scalability to other platforms}\label{supp:scalability}
We assessed the scalability of DreamWaQ++ with applications to legged robots with various morphologies and sizes. We used DreamWaQ++ to train a controller for an ANYmal-C~\cite{hutter2016anymal} and Hound~\cite{shin2022design} robots. Note that we used the same rewards and its corresponding weights as in supplementary section~\ref{supp:reward_functions} and only changed the robot's model as well as their motor's stiffness and damping parameter. A compilation of these robots navigating over stairs is provided in \mvseven. 

\figinitref{figure:supp_multi_robot} shows the success rates of three different robots on climbing stairs with various runs and rises. For the Go1 robot, we used a run value of $0.3~\mathrm{m}$ and $0.6~\mathrm{m}$, while for ANYmal-C and Hound, we used a run value of $0.6~\mathrm{m}$ and $1.0~\mathrm{m}$ to accommodate for their long trunk size. The success rates are measured from $1,\!000$ simulated robots, which is defined as the percentage of the number of robots that can reach the last stair within $10~\mathrm{s}$ over the total number of robots.
% , where a success is defined as when the robot can reach the last stairs within $10~\mathrm{s}$.

As expected, the large joint operation range of Hound enabled it to traverse more difficult terrains compared with the Go1 and ANYmal-C robot, allowing it to traverse up to $42~\mathrm{cm}$-high stairs with an $80\%$ success rate. It is also noteworthy that during training, the robots are faced only with a maximum obstacle height of $27~\mathrm{cm}$, and this result highlights the strong adaptability of the controller trained with DreamWaQ++. Thanks to the explorative behavior during training, DreamWaQ++ also maximizes the hardware's capability and the reward functions are invariant to the hardware variations.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_multirobot_success.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Success rates for climbing different obstacles using various quadrupedal robots.} We trained DreamWaQ++ for \textbf{(A)} Unitree Go1, \textbf{(B)} ANYmal-C, and \textbf{(C)} Hound. The maximum stair rise imposed during training for all robots is $27~\mathrm{cm}$.}
	\label{figure:supp_multi_robot}
\end{figure}



This evaluation successfully highlights the versatility of DreamWaQ++ for its applications to various legged robots. Although deep RL algorithms are notoriously sensitive to reward parameters for different robots, we discovered that DreamWaQ++ can be easily adopted to different platforms with no further tuning effort. 

\subsection{Learning to overcome large obstacles}\label{supp:parkour}
Recently, there has been a growing interest in training quadrupedal robots for more complex tasks such as jumping and leaping~\cite{hoeller2023anymal,zhuang2023robot}. These skills require the quadruped robot to maximize its actuator limit and orchestrate highly-agile motions. We further assessed the scalability of DreamWaQ++ in learning a skill required for overcoming obstacles that are higher than the robot. We trained the Go1, ANYmal-C, and Hound robots in an environment with extreme obstacle heights, reaching up to $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, and $1.5~\mathrm{m}$, respectively. To allow learning of such an agile skill, we need to do some modifications, i.e., 1) relaxing the velocity tracking reward scale from $1.0$ to $0.1$, and 2) increasing the versatility gain scaling in the total loss function from $0.1$ to $0.2$. A snapshot of the learned obstacle climbing motion in simulation and the real world is shown in Fig.~\ref{figure:supp_parkour_sim} and \\mveight.

We found that the two modifications are complimentary. Relaxing the velocity tracking reward without scaling up the versatility gain ends up with a policy that resists moving forward. On the other hand, doubling the versatility gain without relaxing the velocity tracking reward results in a policy that moves forward but with a conservative gait due to lack of skill discovery. This modification allowed the policy to learn more flexible gaits, yielding higher agility for accomplishing more complex tasks such as parkour.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_parkour_sim_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Demonstration of a learned parkour skills in simulation.} We trained DreamWaQ++ for \textbf{(A)}~Unitree Go1, \textbf{(B)}~ANYmal-C, and \textbf{(C)}~Hound to climb obstacles with a height of $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, $1.5~\mathrm{m}$, respectively. \textbf{(D)}~A real world experiment was conducted using a Go1 robot with a $2.5~\mathrm{kg}$ payload on top of it.}
	\label{figure:supp_parkour_sim}
\end{figure}

The results in Fig.~\ref{figure:supp_parkour_sim} illustrate how controllers on different robots produce distinct motions when overcoming large obstacles. In Fig.~\ref{figure:supp_parkour_sim}A, Go1 utilizes a jumping motion to overcome the obstacle, given its small posture. In contrast, ANYmal-C employs its front legs to establish initial contacts with the wall of the obstacle (Fig.~\ref{figure:supp_parkour_sim}B-2) and then uses those legs as anchors to climb (Fig.~\ref{figure:supp_parkour_sim}B-3). Thanks to its large allowable joint positions and torque operation limits, ANYmal-C can climb obstacles as high as $1.5~\mathrm{m}$. Hound, on the other hand, firstly swings its right front leg widely and places it on top of the obstacle as an anchor. Subsequently, it uses its rear legs to propel its body upward (Fig.~\ref{figure:supp_parkour_sim}C-4) and successfully reaches the top of the obstacles.

The real-world experiment in Fig.~\ref{figure:supp_parkour_sim}D was conducted to validate the sim-to-real robustness of the learned controller. Utilizing a Go1 robot with an additional $2.5\mathrm{kg}$ payload, the controller successfully enables the robot to climb a $41~\mathrm{cm}$ obstacle. Notably, the obstacle is a soft sofa block, representing a deformable surface not encountered during training.



% \subsection{Extreme terrain retraining}\label{supp:extreme}
% We further evaluate the versatility of DreamWaQ++ in a more challenging training setting. We fine-tuned the learned controller in a new training setting, consisting of extremely challenging terrains that can push the limit of the robot's physical capabilities, such as large gaps and high stages.

\subsection{Ablation of backbone sequence model}\label{supp:model_ablation}
We conducted an ablation study to evaluate the impact of the backbone sequence model on the controller's performance. We compared the performance of the controller with and with different sequence models by measuring the accuracy of future joint position prediction. The results are shown in Fig.~\ref{figure:supp_nextstate}.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_nextstate_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Future state error comparison.} The comparison shows the future state prediction error using different models and varying robot velocities.}
	\label{figure:supp_nextstate}
\end{figure}

The results in Fig.~\ref{figure:supp_nextstate} show that the proposed MLP-mixer architecture model works as well as the Transformer model. The advantage of using the MLP mixer is that it is more lightweight and computationally efficient than the Transformer model. From the curve, we can see that the prediction error increases as the robot's velocity increases. This is because the robot's motion becomes more dynamic and the model has to predict the future state more accurately.

\subsection{Terrain reconstruction}\label{supp:recons}
We decoded the latent features from the context encoder recorded in the asynchronous stair race experiment to reconstruct the terrain map. The reconstructed terrain map is shown in Fig.~\ref{figure:supp_recons} and \mvone0. The reconstructed terrain map resembles the ground truth terrain map constructed using~\cite{oh2024trip}.

However, note that the reconstructed terrain map is not as accurate as the ground truth terrain map due to three reasons: 
\begin{enumerate}
	\item The robot's exteroception is limited to the front-facing 3D points, and the memory retained by the encoder is not a long term memory.
	\item The encoder-decoder structure does not use a residual connection, similar to~\cite{hoeller2023anymal} to allow learning of only relevant features to the latent representation.
	\item The regularization in the latent space using a variational autoencoder is expected to reduce the reconstruction accuracy while improving disentanglement of the latent features. 
\end{enumerate}
Nevertheless, a slight reduction in the reconstruction accuracy is acceptable because the primary goal of the context encoder is to learn a structured representation that can be used for control, rather than to reconstruct the complete terrain map accurately.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_recons_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Reconstructed terrain map.} The terrain map is reconstructed from the latent features recorded during the asynchronous stair race using DreamWaQ++. The ground truth terrain map is constructed using~\cite{oh2024trip}. The white points are the forward 3D scan input, while the reconstruction points surrounding the robots are colored based on the height relative to the robot's base.}
	\label{figure:supp_recons}
\end{figure}



==> accept/ablation/reconstruction_origin.tex <==
\subsection{Terrain Reconstruction}\label{supp:recons}
    We decoded the latent features from the context encoder recorded in the asynchronous stair race experiment to reconstruct the terrain map. The reconstructed terrain map is shown in Fig.~\ref{figure:supp_recons} and \mvone0. The reconstructed terrain map resembles the ground truth terrain map constructed using~\cite{oh2024trip}.

    However, note that the reconstructed terrain map is not as accurate as the ground truth terrain map due to three reasons: 
    \begin{enumerate}
        \item The robot's exteroception is limited to the front-facing 3D points, and the memory retained by the encoder is not a long term memory.
        \item The encoder-decoder structure does not use a residual connection, similar to~\cite{hoeller2023anymal} to allow learning of only relevant features to the latent representation.
        \item The regularization in the latent space using a variational autoencoder is expected to reduce the reconstruction accuracy while improving disentanglement of the latent features. 
    \end{enumerate}
    Nevertheless, a slight reduction in the reconstruction accuracy is acceptable because the primary goal of the context encoder is to learn a structured representation that can be used for control, rather than to reconstruct the complete terrain map accurately.

    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/supp/supp_recons_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{\textbf{Reconstructed terrain map.} The terrain map is reconstructed from the latent features recorded during the asynchronous stair race using DreamWaQ++. The ground truth terrain map is constructed using~\cite{oh2024trip}. The white points are the forward 3D scan input, while the reconstruction points surrounding the robots are colored based on the height relative to the robot's base.}
        \label{figure:supp_recons}
    \end{figure}

    We further evaluate the impact of the backbone sequence model on the controller's performance. We compared the performance of the controller with and with different sequence models by measuring the accuracy of future joint position prediction. The results are shown in Fig.~\ref{figure:supp_nextstate}.

    \begin{figure}[t!]
        \centering 
        \begin{subfigure}[b]{0.48\textwidth}
            \includegraphics[width=1.0\textwidth]{figures/reduced/recons_error_models_red.pdf}
        \end{subfigure}
        % \captionsetup{font=footnotesize}
        \caption{Future state prediction error using different models and varying robot velocities. The MLP-mixer model used in DreamWaQ++ shows comparable performance to the Transformer model while being more lightweight and computationally efficient.}
        \label{figure:supp_nextstate}
    \end{figure}

    The results in Fig.~\ref{figure:supp_nextstate} show that the proposed MLP-mixer architecture model works as well as the Transformer model. The advantage of using the MLP mixer is that it is more lightweight and computationally efficient than the Transformer model. From the curve, we can see that the prediction error increases as the robot's velocity increases. This is because the robot's motion becomes more dynamic and the model has to predict the future state more accurately.


==> accept/acknowledgments.tex <==
\section*{Acknowledgments}
\paragraph{Funding:} 
\begin{enumerate}
    \item Korea Evaluation Institute of Industrial Technology~(KEIT) grant funded by the Korea Government~(MOTIE) (No. 20018216, ``Development of Mobile Intelligence SW for Autonomous Navigation of Legged Robots in Dynamic and Atypical Environments for Real Application''
    \item BK21 FOUR funded by the Ministry of Science and ICT, Republic of Korea.
\end{enumerate}


\paragraph{Author contributions:}
\begin{enumerate}
    \item Conceptualization: IMAN, HM
    \item Methodology: IMAN
    \item Software: IMAN, MO, SHL
    \item Validation: IMAN, MO, BY, DL, HWL, SHL
    \item Formal analysis: IMAN, HL
    \item Baseline reproduction: IMAN, DL, HWL, SHL:
    \item Investigation: IMAN, MO, BY, DL, HWL, SHL
    \item Resources: HM
    \item Data curation: IMAN, MO, SHL, DL
    \item Writing - original draft: IMAN
    \item Writing - review \& editing: IMAN, MO, BY, DL, SHL, HWL, HL, HM
    \item Visualization: IMAN, MO, HL, SHL
    \item Supervision: HM
    \item Project administration: IMAN, HM
    \item Funding acquisition: HM
    
\end{enumerate}

\paragraph{Competing interests:}The authors declare that they have no competing interests.

\paragraph{Data and materials availability:}All data needed to support the conclusions of this manuscript are included in the main text or Supplementary Materials.\ref{section:supp}


==> accept/control/problem.tex <==
\subsection{Problem Formulation}
The control problem is formulated in a partially observable Markov decision process~(POMDP) setting with a goal to maximize the expected discounted future rewards, which in turn resulting in a policy:

\begin{equation}
    \pi=\argmax_{\textbf{a}} E\left[\sum_{t=0}^{\infty}\gamma^t r_t\right],
    \label{eq:pi}
\end{equation}
where $\textbf{a}$, $\gamma$, and $r$ are the action, discount factor, and rewards, respectively. This objective is optimized using the proximal policy optimization (PPO)~\cite{schulman2017proximal} algorithm, while also taking into account the auxiliary objectives related to the perception pipeline.

We leveraged a privileged learning setting using an asymmetric actor-critic architecture, following~\cite{nahrendra2023dreamwaq}. The actor, i.e. the policy receives partial and noisy observations ($\textbf{o}^\mathrm{p}_t$), akin to the real-world observations and the multi-modal context ($\textbf{z}^\mathrm{pe}_t$) as its input. The policy network runs at a rate of $50~\mathrm{Hz}$, generating a target joint position that is tracked by a low-level PD controller, running at $200~\mathrm{Hz}$, to generate the joint torque commands. 

==> accept/environment/curriculum.tex <==
\subsection{\textit{Curriculum}}
We leveraged three curricula during training, i.e., terrain, command, and reward curricula. For the terrain curriculum, various terrains were procedurally generated at the beginning of training to simulate obstacles the robot might encounter in real-world environments. The terrain curriculum utilized a game-inspired setting~\cite{rudin2021learning} with ten levels of difficulty. We primarily used terrains such as \texttt{rough}, \texttt{stairs}, \texttt{gaps}, and \texttt{discretized obstacle}, to introduce variation in exteroception, thereby increasing the diversity of training data for the multi-modal context encoder. An agent was promoted to the next level if it could traverse more than half the distance at the current level. If an agent failed to cover more than half the distance for ten consecutive episodes, it was demoted to the previous level. Agents that successfully completed all levels were randomly spawned within the ten levels, which prevented catastrophic forgetting and further diversified the training data.

The policy was trained to maximize command tracking rewards while satisfying style rewards (Table~\ref{table:reward_functions}), resulting in smooth and accurate robot motion. The curriculum followed a reward-based approach, automatically increasing the command velocity range when the velocity tracking reward, $r_{v_{x,y}} \in [0, 1]$, exceeded a set threshold, $r^\textrm{thres}_{v_{x,y}}$, which was defined as $0.9$.

Finally, the reward curriculum promotes safe behavior in real-world scenarios by gradually increasing the penalty for style rewards. Applying strong penalties to style rewards early in training can restrict exploration, leading to poor performance. However, without sufficient penalties, the robot may behave aggressively when noisy exteroceptive measurements are introduced in real-world settings. Therefore, a reward curriculum with exponentially increasing penalties over learning iterations was employed to facilitate stable learning. More details are provided in Section~\ref{supp:reward_functions}.


==> accept/results/large_obstacles_origin.tex <==
\subsection{\mveightref{Overcoming Large Obstacles}}\label{supp:parkour}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/reduced/results_large_obstacles_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{We trained DreamWaQ++ for (a)~Unitree Go1, (b)~ANYmal-C, and (c)~Hound to climb obstacles with a height of $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, $1.5~\mathrm{m}$, respectively. (d)~A real world experiment was conducted using a Go1 robot with a $2.5~\mathrm{kg}$ payload on top of it.}
	\label{figure:supp_parkour_sim}
\end{figure}

Recently, there has been a growing interest in training quadrupedal robots for more complex tasks such as jumping and leaping~\cite{hoeller2023anymal,zhuang2023robot}. These skills require the quadruped robot to maximize its actuator limit and orchestrate highly-agile motions. We further assessed the scalability of DreamWaQ++ in learning a skill required for overcoming obstacles that are higher than the robot. We trained the Go1, ANYmal-C, and Hound robots in an environment with extreme obstacle heights, reaching up to $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, and $1.5~\mathrm{m}$, respectively. To allow learning of such an agile skill, we need to do some modifications, i.e., 1) relaxing the velocity tracking reward scale from $1.0$ to $0.1$, and 2) increasing the versatility gain scaling in the total loss function from $0.1$ to $0.2$. A snapshot of the learned obstacle climbing motion in simulation and the real world is shown in Fig.~\ref{figure:supp_parkour_sim} and \mveight.

We found that the two modifications are complimentary. Relaxing the velocity tracking reward without scaling up the versatility gain ends up with a policy that resists moving forward. On the other hand, doubling the versatility gain without relaxing the velocity tracking reward results in a policy that moves forward but with a conservative gait due to lack of skill discovery. This modification allowed the policy to learn more flexible gaits, yielding higher agility for accomplishing more complex tasks such as parkour.

The results in Fig.~\ref{figure:supp_parkour_sim} illustrate how controllers on different robots produce distinct motions when overcoming large obstacles. In Fig.~\ref{figure:supp_parkour_sim}A, Go1 utilizes a jumping motion to overcome the obstacle, given its small posture. In contrast, ANYmal-C employs its front legs to establish initial contacts with the wall of the obstacle (Fig.~\ref{figure:supp_parkour_sim}B-2) and then uses those legs as anchors to climb (Fig.~\ref{figure:supp_parkour_sim}B-3). Thanks to its large allowable joint positions and torque operation limits, ANYmal-C can climb obstacles as high as $1.5~\mathrm{m}$. Hound, on the other hand, firstly swings its right front leg widely and places it on top of the obstacle as an anchor. Subsequently, it uses its rear legs to propel its body upward (Fig.~\ref{figure:supp_parkour_sim}C-4) and successfully reaches the top of the obstacles.

The real-world experiment in Fig.~\ref{figure:supp_parkour_sim}D was conducted to validate the sim-to-real robustness of the learned controller. Utilizing a Go1 robot with an additional $2.5\mathrm{kg}$ payload, the controller successfully enables the robot to climb a $41~\mathrm{cm}$ obstacle. Notably, the obstacle is a soft sofa block, representing a deformable surface not encountered during training.

In Fig.~\ref{figure:supp_parkour_sim}(e) and \mvfour, the robot was positioned on a $50~\mathrm{cm}$ stage, making it impossible for a small quadruped, with a calf length shorter than $30~\mathrm{cm}$, to simply probe the terrain. Therefore, when commanded to move forward, the robot made a leap motion, allowing it to move away from the stage while avoiding collision between the rear legs with the edges of the stage. This leap motion was also made possible by the velocity tracking relaxation strategy that allows the robot to stop at the edge of the stage~(Fig.~\ref{figure:supp_parkour_sim}(e-2)) for initiating the leap motion. Subsequently, the robot performs a kick using both front legs, then propels the movement forward using both rear legs~(Fig.~\ref{figure:supp_parkour_sim}(e-3)). Soon after, the robot also folds its rear legs to avoid collision with the stage~(Fig.~\ref{figure:supp_parkour_sim}(e-4)). This highlights the versatility of the learned controller as a prior that can be adapted for more complex tasks.

==> accept/supplementaries.tex <==
\section{Supplementaries}\label{section:supp}

\begingroup
% \renewcommand{\thesubsection}{S\arabic{subsection}}

% \renewcommand{\figurename}{Fig.}
% \renewcommand{\thefigure}{S\arabic{figure}}
% \captionsetup[figure]{labelfont=bf,labelsep=period,font=normalsize}

% \renewcommand{\thetable}{S\arabic{table}}
% \captionsetup[table]{labelfont=bf,labelsep=period,font=normalsize}

% \setcounter{figure}{0}


\subsection{Nomenclature}\label{supp:nomenclature}
\begin{table}[h!]
    \small
    \begin{tabular}{ll}
        \textbf{Notations} \\
        $(\cdot)^\textbf{des}$ & Target or desired value\\
        $(\cdot)^\textbf{cmd}$ & Command value\\
        $\textbf{g}$ & Gravity vector projected on the robot's body frame\\
    \end{tabular}
\end{table}

\begin{table}[h!]
    \small
    \begin{tabular}{ll}
        \textbf{Operators} \\
        $\mathrm{exp(\cdot)}$ & Exponential function\\
        $\mathrm{var(\cdot)}$ & Variance function\\
         $\mathrm{\sigma(\cdot)}$ & Standard deviation function\\
    \end{tabular}
\end{table}

\begin{table}[H]
    \small
    \begin{tabular}{ll}
        \textbf{Abbreviations} \\
        IMU & Inertial measurement unit\\
        HAA & Hip abduction/adduction\\
        HFE & Hip flexion/extension\\
        KFE & Knee flexion/extension\\
        FR & Front right\\
        FL & Front left\\
        RR & Rear right\\
        RL & Rear left\\
        MLP & Multi-layer perceptron\\
        PaCMAP & Pairwise controlled manifold approximation projection\\
        PD & Proportional and derivative\\
        POMDP & Partially observable Markov decision process\\
        PPO & Proximal policy optimization\\
        t-SNE & t-distributed stochastic neighbor embedding\\
        VAE & Variational autoencoder\\
    \end{tabular}
\end{table}


\begin{table*}[h!]
    \centering
    \caption{\textbf{Summary of state-of-the-art algorithms}. \textit{Versatility} indicates whether the learned controller can be flexibly used for various tasks, e.g.~using a teleoperation or with a high-level planner. \textit{Computation} indicates the number of onboard processor(s) used on the robot to infer the whole locomotion controller, including the processor(s) used for preprocessing the exteroceptive measurement. \textit{Exteroception} indicates what type of exteroceptive measurement is required as an input.  \textit{Training stage} indicates the number of separate training procedures. Training stage~$\!=\!1$ means that there is no pre-training or fine-tuning of the networks using additional training instances. Training stage~$\!>\!1$ means additional training instances are required such as distillation, fine-tuning, and pre-training of some auxiliary modules.}
    \small
    \begin{tabular}{|c|c|c|c|c|c|} \hline 
         \multirow{2}{*}{Algorithm}&   \multirow{2}{*}{Robot}& \multicolumn{2}{|c|}{Deployment}&  \multirow{2}{*}{Exteroception}& Training\\ \cline{3-4}
         \multirow{2}{*}{} & \multirow{2}{*}{} &  Versatility&Computation& \multirow{2}{*}{}&stage\\\hline
         Miki \textit{et al}.~\cite{miki2022learning}&   ANYmal-C& \cmark&  1 (GPU)&Elevation map&  2\\ \hline 
         Agarwal \textit{et al}.~\cite{agarwal2022legged}&   Unitree A1& \xmark&  1&Depth image&  2\\ \hline 
         Yang \textit{et al}.~\cite{yang2023neural}&   Unitree A1& \xmark&  1& Depth image&  2\\ \hline 
         Hoeller \textit{et al}.~\cite{hoeller2023anymal}&   ANYmal-D& \cmark&  2& Surround pointcloud& 6\\ \hline 
		 Cheng \textit{et al}.~\cite{cheng2023parkour}&   Unitree A1& \cmark&  2& Depth image& 2\\ \hline 
         DreamWaQ++ (ours)&   Unitree Go1& \cmark&  1& Forward pointcloud&  1\\ \hline
    \end{tabular}
    
    \label{table:comparison}
\end{table*}

\subsection{Problem formulation}
We formulate the problem as a partially observable Markov decision process (POMDP) because, in the real world, the robot has no direct access to the exact state of the environment. We try to solve the problem by leveraging few shot meta--reinforcement learning (meta--RL) via task inference, which trains a separate network that can predict the task or context of the environment leveraging a few data points in conjunction with the policy network.

The environment is a POMDP defined by the tuple $\mathcal{M}=(\mathcal{S},\mathcal{O},\mathcal{A},d_0,p,r,\gamma)$. The full state, partial observation, and action are continuous, and defined by $\mathcal{\textbf{s}\in\mathcal{S}}$, $\mathcal{\textbf{o}\in\mathcal{O}}$, and $\mathcal{\textbf{a}\in\mathcal{A}}$, respectively. Generally, every environment with different physical properties, such as the robot's hardware, terrain properties, and commanded velocity, is categorized as a different POMDP sampled from a task distribution $P(\mathcal{M})$.

The environment starts with an initial state distribution, $d_0(\textbf{s}_0)$; progresses with a system dynamics $p(\textbf{s}_{t+1}|\textbf{s}_{t},\textbf{a}_{t})$; and obtains a reward, $r:\mathcal{S}\times\mathcal{A}\to\mathcal{R}$ for every action at a given state. The discount factor is defined by $\gamma\in[0,1)$. 

The goal of meta--RL in our problem setting is to learn a context encoder network, $\phi(\textbf{z}|\textbf{o},\textbf{a})$, that can infer the task in a form of a context vector, $\textbf{z}$, given available observations and actions. 
% In this paper, we define a temporal observation at time $t$ over the past $H$ measurements as $\textbf{o}^H_t=\begin{bmatrix}\textbf{o}_t & \textbf{o}_{t-1} \dots \textbf{o}_{t-H} \end{bmatrix}^T$. 

Prior works have enjoyed the benefit of task inference for fast adaptation of the learned control policy in the real world by explicitly training a context encoder that predicts some physical properties of the world, such as ground friction and restitution~\cite{kumar2021rma,lee2020learning,miki2022learning}. However, those works assumed that the contexts were available in training time. Although this relaxed assumption can facilitate learning, it also limits the solution space of the context. Moreover, as some context might not be directly identifiable from a short history of observations, the context encoder may fail to generate an informative context~\cite{xie2022robust}. 

In contrast, we trained a context encoder in an unsupervised manner. In DreamWaQ~\cite{nahrendra2023dreamwaq}, the context encoder is built upon the $\beta$--variational autoencoder ($\beta$--VAE) architecture that predicts the future observations. The advantages of leveraging $\beta$--VAE in DreamWaQ's framework are twofold. First, a higher degree of latent disentanglement induced by the $\beta$--VAE enables distinguishable task inference, which significantly helps learning and adaptation. Second, the stochastic network architecture makes the context encoder more robust to epistemic uncertainty when given out of distribution (OOD) observations.

In this work, the context encoder is trained jointly with a height reconstructor network to build a map using a stream of historical proprioceptive and exteroceptive data. This method is theoretically possible because it is built on the idea of simultaneous localization and mapping~(SLAM) where accumulated geometrical feature points along with odometry can be fused to build a map around the robot. More specifically, the context encoder in DreamWaQ++ consists of three attention mechanisms, i.e.~cross--modal, temporal, and spatial attentions.




% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable} 
\centering
% \captionsetup{font=footnotesize, singlelinecheck=false}
\caption{\textbf{Hardware comparison}. The hardware parameters are obtained by measuring the official open-sourced 3D model of the corresponding robot~\cite{unitreea1,unitreego1}.}
\label{table:hardware_comparison}
\begin{center}
\begin{tabular}{lcc}
\hline \hline
Parameter           & Unitree A1~\cite{unitreea1} & Unitree Go1~\cite{unitreego1} \\ \hline 
Total weight (kg)       & $12$ & $13$      \\ 
Base length (m)         & $0.27$ & $0.38$      \\ 
Base width (m)          & $0.19$ & $0.19$      \\ 
Base height (m)         & $0.11$ & $0.11$      \\ 
Standing height (m)     & $0.4$ & $0.4$      \\ 
Thigh length (m)        & $0.2$ & $0.2$      \\ 
Calf length (m)         & $0.2$ & $0.2$      \\ 
Max. hip torque (Nm)    & $33.5$ & $23.7$      \\ 
Max. thigh torque (Nm)  & $33.5$ & $23.7$      \\ 
Max. calf torque (Nm)   & $33.5$ & $33.5$      \\ 
 

\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

\subsection{Real-world Stair-climbing Race}\label{supp:race}
The race experiment was conducted on a long-flight of stairs. \figinitref{supp:race} visualizes the stair characteristics used in the experiment.
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_race_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Geometrical details of the stairs used for robot race experiment.}}
	\label{figure:supp_race}
\end{figure}

To support the race experiments, we conducted additional asynchronous experiments where robot R4~(Fig.~\ref{figure:supp_hardware}C) was used to deploy the controllers. Robot~R4 was also controlled with an autonomous navigation module to ensure consistent path planning while climbing the stairs. The experiments videos are summarized in \mvone0, and a few snapshots of the experiments that highlight the robot's motions are shown in Fig.~\ref{figure:supp_async_race}. Robot~R4 was controlled using (\textbf{A})~DreamWaQ++, (\textbf{B})~DreamWaQ, and (\textbf{C})~Unitree Go1's built-in controller. The robot, controlled by DreamWaQ++, managed to climb the stairs with minimum leg and body collisions by adaptively raising its body and foot swing height. In contrast, the robot controlled with DreamWaQ experienced a series of stumbles, although it managed to climb the stairs due to the robust nature of the controller. The robot controlled by the Unitree Go1's built-in controller could climb the stairs but often got stuck due to the lack of adaptability in the controller.

One discernible behavior between DreamWaQ++ and DreamWaQ lies in its gait adaptation. DreamWaQ++ adapts its gait by raising its body and swinging its foot further to step on the stairs (see Fig.~\ref{figure:supp_async_race}A), while DreamWaQ tends to collide the robot foot with the stairs and then drag it along the stair's vertical surface before placing it on the next step (see Fig.~\ref{figure:supp_async_race}B). This behavior is less efficient and may cause the robot to stumble. On the other hand, the robot with Unitree Go1's built-in controller tends to use a fixed gait pattern, which is less adaptive to the stairs' geometry and lacks spatial memory, causing its rear leg to stumble multiple times (see Fig.~\ref{figure:supp_async_race}C).

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_async_race_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Asynchronous stair-climbing experiments.} The robot was controlled using (\textbf{A}) DreamWaQ++, (\textbf{B}) DreamWaQ, and (\textbf{C})  Unitree Go1's built-in controller. The white mask on the stair indicates the same stair plate that each robot interacted with over the four successive snapshots. The full asynchronous race experiment is available in \mvone0.}
	\label{figure:supp_async_race}
\end{figure}

We also measured the state estimation error of the robot controlled by DreamWaQ++ and DreamWaQ during the asynchronous experiments. The state estimation error is the absolute error between the ground truth and estimated velocities. The ground truth data was obtained using a LiDAR odometry algorithm~\cite{xu2022fast}. The results are shown in Fig.~\ref{figure:supp_error_track}. The robot controlled by DreamWaQ++ exhibits a lower state estimation error compared to the robot controlled by DreamWaQ with a significant difference. This result indicates that the robot controlled by DreamWaQ++ can better estimate its position and adapt its gait to the stairs' geometry, which is crucial for climbing stairs efficiently, yielding a more stable and robust locomotion.

\begin{figure}[h!]
	\centering 
	\begin{subfigure}[b]{0.38\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_vel_error_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Velocity estimation error comparison in the stair-climbing task.} The **** annotation indicates a significant difference between the two controllers as measured by a paired $t$-test.}
	\label{figure:supp_error_track}
\end{figure}

\subsection{Blind locomotion on stairs}\label{supp:dreamwaq}
We evaluate the performance of a blind locomotion controller trained using DreamWaQ~\cite{nahrendra2023dreamwaq} when traversing a series of stairs with $15\!\sim\!18~\mathrm{cm}$ high rise as shown in Fig.~\ref{figure:supp_dreamwaq}. Although the robot initially managed to climb the stairs, it became unstable due to a series of stumbles and eventually fell down before reaching the end of the stairs. We discovered that the most risky stumbles were when the two front legs stumbled at the same time, making the robot lose its balance. This result highlights the importance of exteroception for a legged robot to proficiently traverse through obstacles.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_stairs_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Illustrations of blind locomotion failure in a stair-climbing scenario.} A series of stumbles made the robot cannot preserve its stability and eventually fell down.}
	\label{figure:supp_dreamwaq}
\end{figure}

\subsection{Climbing a long flight of stairs}\label{supp:long_stairs}

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_long_stairs_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Stairs climbing experiments}. The robot is commanded to climb a long flight of (\textbf{A})~straight and (\textbf{B})~curved stairs.}
	\label{figure:supp_long_stairs}
\end{figure}

\figinitref{figure:supp_long_stairs}E shows snapshots of the robot climbing $39$ steps of stairs, yielding a total elevation of $5.46~\textrm{m}$ and inclination of $25.76^{\circ}$. We used a blind locomotion controller trained using DreamWaQ as a baseline comparison. While the blind locomotion controller initially managed to overcome the stairs, its performance quickly deteriorated due to numerous stumbles (see supplementary section~\ref{supp:dreamwaq}). In contrast, the controller trained using DreamWaQ++ (Fig.~\ref{figure:supp_long_stairs}E) allowed the robot to swiftly climb the stairs with minimum leg and body collisions by adaptively raising its body and foot swing height. The robot reached the top of the stairs in $47~\textrm{s}$, stressing the importance of exteroception on locomotion over a long flight of stairs that necessitates fast adaptation of the robot's gait to minimize stumbles.

\subsection{Paired $t$-test on slope climbing}\label{supp:t-test}
The significance of the difference between torque exertion of each joint in Fig.~\ref{figure:results_adaptation}F was measured using a paired $t$-test method. The annotations on the figure are defined based on the resulting $p$-values. We follow the standard rule defined in Table~\ref{table:t-test}. The $p$-values were corrected using the Bonferroni correction method~\cite{florian_charlier_2022_7213391} and presented in Table~\ref{table:p-value}.

% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\caption{Description for $p$-value annotation~\cite{florian_charlier_2022_7213391}.}
\centering
% \captionsetup{justification=centering}

\label{table:t-test}
\begin{center}
\begin{tabular}{lll}
\hline \hline
Annotation           & Criteria \\ \hline 
ns (not significant)  &                      $0.05 < p \leq 1.0$ \\
$*$  &                      $0.01 < p \leq 0.05$ \\
$**$  &                      $0.001 < p \leq 0.0$ \\
$***$  &                      $0.0001 < p \leq 0.001$ \\
$****$  &                      $ p \leq 0.0001$ \\
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\centering
% \captionsetup{justification=centering}
\caption{$p$-value results of data reported in Fig.~\ref{figure:results_adaptation}.}
\label{table:p-value}

\begin{center}
\begin{tabular}{llc}
\hline \hline
Joint           & $p$-value & Signficance \\ \hline 
FR Thigh  &                      $1.0$ 			& ns\\  
FR Calf  &                      $0.4464$ & ns\\  
FL Thigh  &                      $1.0$ & ns\\  
FL Calf  &                      $1.0$ & ns\\  
RR Thigh  &                      $0.001244$ & **\\  
RR Calf  &                      $0.00009325$ & ****\\  
RL Thigh  &                      $0.00001922$ & ****\\  
RL Calf  &                      $1.0$ & ns\\  
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================


\subsection{Exteroception preprocessing}\label{supp:exteroception_preprocessing}
In this work, we employ a voxel grid representation as the input for the policy. The voxel grid encompasses downsampled robot-centric 3D points obtained from an exteroceptive sensor mounted on the robot. The voxels are obtained via voxel-grid filtering with a leaf size of $0.05~\mathrm{m}$. We assume accurate extrinsic calibration parameters are available to transform the measured 3D points from the sensor frame to the body frame. We set the exteroceptive measurements to be within a grid with its row and column size of $w\!=\!1.1~\mathrm{m}$ and $h\!=\!0.5~\mathrm{m}$, respectively. The first row of the grid is located $0.9~\mathrm{m}$ in front of the robot, yielding a grid with 10 rows and 22 columns by dividing the size with the leaf size.

\subsection{Constrained reparameterization trick}\label{supp:constrained_reparam}
The multi-modal encoder architecture encompasses multiple stochastic layers within the encoders and multi-modal mixer networks, offering advantages such as enhanced robustness and increased exploration capabilities. However, a trade-off arises with numerical stability during the early stages of training. 

A straightforward solution is to balance the weight of the reconstruction loss and KL divergence in $\mathcal{L}_\mathrm{VAE}$. In variational inference, the prior distribution of the latent state is often assumed to follow a normal distribution. The stability issue can be mitigated by putting more emphasis on the latent loss during training. This approach ensures that the encoder learns a better approximation of the latent space while preserving the ability to reconstruct the input data accurately.

However, strongly matching the posterior and prior distributions via the latent loss can lead to another issue where the encoder tends to neglect important details in the input point cloud. This deficiency makes the policy unable to detect and respond to small obstacles in the environment effectively. To overcome this challenge, we introduced a constrained reparameterization trick, defined as

\begin{equation}
    \textbf{z} \sim N(g_{\mu}(\textbf{x}),g_{\sigma}(\textbf{x})),
\end{equation}
where $\textbf{z}$ is a stochastic latent vector and $\textbf{x}$ is the input of the encoder network $g$. The subscripts $\mu$ and $\sigma$ indicate the outputs of $g(x)$ that correspond to the mean and standard deviation of the latent distribution, respectively. $z$ is sampled from a Gaussian distribution $N(\cdot,\cdot)$ with mean $g_{\mu}(\textbf{x})$ and standard deviation $g_{\sigma}(\textbf{x})$. 

During this reparameterization step, we imposed hard constraints on the standard deviation of the distribution, such that $\sigma_\mathrm{min}\leq g_{\sigma}(\textbf{x}) \leq \sigma_\mathrm{max}$. This constraint ensures that the generated samples are numerically stable and can be reliably propagated to the subsequent layers of the network. By implementing this simple yet effective solution, the learning process becomes much more stable without compromising the final performance of the learned policy. Empirically, we set $\sigma_\mathrm{min}=0$ and $\sigma_\mathrm{max}=5$ to promote stable training. This constrained reparameterization trick is employed on all encoder networks that utilize a stochastic layer.


\subsection{Training environment details} \label{supp:training_env}
\subsubsection{\textit{Simulation}}
We used NVIDIA Isaac Gym~\cite{makoviychuk2021isaac} preview 3 as the simulator for training the controller and multi-modal context encoder networks. The training environments were built upon the Legged Gym library~\cite{rudin2021learning}. We employed domain randomization over $3,\!500$ agents, which took about 11 hours of training on an NVIDIA A5000 GPU. Afterwards, the trained networks were deployed without any fine-tuning on a real or simulated robot in the Gazebo simulation for the evaluations presented in this paper. 

\subsubsection{\textit{Control pipeline}}
The policy and multi-modal context encoder networks ran synchronously while receiving asynchronous observations. Proprioceptive measurements were sampled at $200~\textrm{Hz}$, whereas exteroceptive measurements were sampled at $10~\textrm{Hz}$. The controller integrated the most recent measurements, operating at $50~\textrm{Hz}$. To enhance the robustness of the controller against the asynchronous observations, we employed latency randomization during training. Detailed information regarding the randomized latency for all measurements is provided in Table~\ref{table:domain_randomization}.

The policy network generated target joint positions at a rate of $50~\textrm{Hz}$, which were subsequently transmitted to a low-level proportional-derivative (PD) controller operating at $200~\textrm{Hz}$. Within the PD controller, the target joint positions were converted into torque commands, employing proportional ($K_p$) and derivative ($K_d$) control gains of $25$ and $0.7$, respectively. These computed torque commands were subsequently relayed to the low-level motor controller integrated within our customized Unitree Legged SDK.


% \begin{itemize}
%     \item \textbf{Rough slopes} are generated by
%     \item \textbf{Stairs}
%     \item \textbf{Gaps}
%     \item \textbf{Random discrete}
% \end{itemize}

\subsubsection{\textit{Curriculum}}
We leveraged three curriculums during training, i.e.~terrain, command, and reward curriculums. For the terrain curriculum, several terrains were procedurally generated at the beginning of training to simulate various obstacles the robot might encounter in the real world. The terrain curriculum utilized the game-inspired curriculum setting~\cite{rudin2021learning} with ten different levels of difficulty. We generally utilized \texttt{rough}, \texttt{stairs}, \texttt{gaps}, and \texttt{discretized obstacle} terrains to introduce variations in the exteroception, which could induce diversity in the training data for the multi-modal context encoder. An agent was promoted to the next level if it could traverse more than half of the distance at the current level. When an agent failed to traverse more than half of the distance at the current level for more than ten episodes, it was demoted to the previous level. If an agent successfully walked through all levels, it will be randomly spawned within the ten levels, preventing catastrophic forgetting and diversifying the training data.
 
The policy was trained to maximize the command tracking rewards while satisfying style rewards (Table~\ref{table:reward_functions}), resulting in smooth and accurate robot motion. The curriculum was a reward-based one, which automatically increased the command velocity range when the velocity tracking reward, $r_{v_{x,y}}\in[0, 1]$, surpassed a given threshold, $r^\textrm{thres}_{v_{x,y}}$, which was set to $0.9$. 

Finally, the reward curriculum ensures safe behavior in the real world by gradually increasing the penalty for the style rewards. Applying strong penalties to the style rewards at early training can restrict exploration, resulting in poor performance. However, without a strong penalty, the robot tends to behave aggressively once noisy exteroceptive measurements are taken as inputs in the real world. Hence, a reward curriculum that exponentially grows over learning iteration was utilized to facilitate stable learning. More details are provided in section~\ref{supp:reward_functions}.

\subsubsection{\textit{Domain randomization}}
We randomized multiple physical properties of the robot and the environment to facilitate sim--to--real transfer. Additionally, we employed Roll-Drop~\cite{campanaro2023roll} to encourage exploration and robustness on top of physics randomization. Details of the physical properties and its randomization ranges are provided in Table~\ref{table:domain_randomization}.

\begin{table}[t!]
\centering
% \captionsetup{justification=centering}
\caption{Domain randomization ranges applied in the simulation.}
\label{table:domain_randomization}
\begin{center}
\begin{tabular}{lccc}
\hline\hline
Parameter                        & Randomization range & Unit \\\hline
Payload                     & $[-1, 2]$ & $\mathrm{~kg}$     \\ 
$K_p$ factor   & $[0.9, 1.1]$ & $\mathrm{~Nm~rad^{-1}}$    \\ 
$K_d$ factor        & $[0.9, 1.1]$ & $\mathrm{~Nms~rad^{-1}}$   \\ 
Motor strength factor        & $[0.9, 1.1]$ & $\mathrm{~Nm}$   \\ 
Center of mass shift        & $[-50,50]$ & $\mathrm{~mm}$    \\
Friction coefficient        & $[0.2, 1.25]$ & -    \\
System delay                        & $[0.0, 15.0]$ &  $\mathrm{~ms}$   \\


\hline\hline
\end{tabular}
\end{center}
\vspace{-0.cm}
\end{table}


\subsubsection{\textit{Adversarial observation}}
We injected noises into the proprioceptive and exteroceptive observations. For the proprioceptive observations, a uniform noise was injected at each time step. 
% The magnitude of noises for each observation \rvc{is} summarized in Table~\ref{table:observation_noise}. 
For the exteroceptive data, we classified three different noise ranges, constituting low, medium, and high noises. The proportion of these exteroceptive noise scales was set to $30\%$, $50\%$, and $20\%$, respectively.
The magnitude of noises for each observation is summarized in Table~\ref{table:observation_noise}. 

\begin{table}[t!]
\centering
% \captionsetup{justification=centering}
\caption{Noise parameters injected into the observation for the policy network during training.}
\label{table:observation_noise}
\begin{center}
\begin{tabular}{lccc}
\hline\hline
Observation                        & Noise range ($\mu$) & Unit \\\hline
Joint position  &                      $[-0.01, 0.01]$ & $\mathrm{rad}$     \\ 
Joint velocity  &                      $[-1.5, 1.5]$ & $\mathrm{rad/s}$    \\ % $\mathrm{rad~s^{-1}}$    \\ 
Body linear velocity &                 $[-0.1, 0.1]$ & $\mathrm{m/s}$   \\ % $\mathrm{m~s^{-1}}$   \\ 
Body angular velocity &                $[-0.2, 0.2]$ & $\mathrm{rad~^{-1}}$   \\ 
Gravity vector        &                $[-0.05, 0.5]$ & $\mathrm{m/s^{2}}$    \\ % $\mathrm{m~s^{-2}}$    \\
Exteroceptive measurement (low)  &     $[0.0, 0.03]$ & $\mathrm{m}$\\
Exteroceptive measurement (medium)  &     $[0.03, 0.1]$ & $\mathrm{m}$    \\
Exteroceptive measurement (high)  &     $[0.1, 0.3]$ & $\mathrm{m}$    \\


\hline\hline
\end{tabular}
\end{center}
\vspace{-0.cm}
\end{table}


Although observation noise is often easily handled by a controller that leverages only proprioception if trained with sufficient domain randomization,  the learned controller exhibited increased sensitivity to disturbances in exteroception, primarily attributed to the rich information contained within exteroceptive measurements. Several issues, such as inaccurate extrinsic calibration and sensor noise, significantly deteriorated the controller's robustness. In robotics, auto-calibration is a highly desirable attribute, capable of enhancing system robustness. Consequently, we aimed to integrate this capability into the proposed multi-modal context encoder.

To achieve this, we trained the multi-modal context encoder to explicitly predict extrinsic calibration errors within the exteroception data. This explicit error prediction serves a dual purpose within our framework. First, it provides guidance to human operators, enabling them to recalibrate the extrinsic parameters effectively. Concurrently, the multi-modal context encoder learns to discern and mitigate the impact of this calibration error, thus producing more accurate exteroception reconstructions. This proactive approach enhances the overall performance and resilience of the proposed system in the presence of exteroceptive disturbances.

Throughout the training process, we introduced a randomization procedure for the extrinsic calibration parameters within the $SE(3)$ coordinate system at the beginning of each episode. These calibration parameters served as ground-truth values, challenging the multi-modal context encoder to predict them accurately. We proposed a customized perturbation model for the exteroception because we are exploiting the robot-centric height scan as the input for the encoder. The perturbation model consists of i) noise, ii) sensor alignment error, and iii) pruning.

\paragraph{Noise model}
The noise model is designed to mimic the characteristics of range measurement sensors such as LiDAR \rvc{sensors} or depth cameras. First, the distance between the sampled 3D robot-centric points to the body frame of the robot is measured as $\textbf{d}_t=[d^1_t\;\cdots{}\;d^i_t\;\cdots{}\;d^I_t] \in \mathbb{R}^{1 \times I}$, where $i$ indicates the $i$-th element and $I$~is the number of points per scan. 
Then, for the $i$-th point, an anisotropic Gaussian noise is applied to the point set $\textbf{p}_t=[\textbf{p}^1_t\;\cdots\;\textbf{p}^i_t\;\cdots\;\textbf{p}^I_t]\in\mathbb{R}^{3 \times I}$, where $\textbf{p}^i_t=\begin{bmatrix} x^i_t & y^i_t &  z^i_t \end{bmatrix}$. The Gaussian noise is centered at the nominal noise level, and the variance is scaled according to the distance of each point to the robot. Practically, exteroceptive measurements in the real world exhibit higher noise when the terrains are very close to the sensor. Therefore, we formulate each noisy point as

\begin{equation}
    \textbf{p}^i_t = 
    \begin{bmatrix}
    x^i_t + \mathcal{N}\left(\mu_x, \sigma^2_x\right)\\
    y^i_t + \mathcal{N}\left(\mu_y, \sigma^2_y\right)\\
    z^i_t + \mathcal{N}\left(\mu_z, \sigma^2_z\right)\\
    \end{bmatrix},
    \label{eq:noise_model}
\end{equation}
where $\mu$  and $\sigma^2$ are the nominal noise level and noise variance, respectively, with the subscripts $x$, $y$, and $z$ indicating that the elements correspond to the $x$, $y$, and $z$ axes. These noise parameters were sampled from a uniform distribution within the range specified in Table~\ref{table:point_noise} at the beginning of every episode. Afterwards, the point-wise noise in~\eqref{eq:noise_model} was sampled at every time step.

\begin{table}[t!]
\centering
% \captionsetup{justification=centering}
\caption{Point noise parameters during training.}
\label{table:point_noise}
\begin{center}
\begin{tabular}{cccc}
\hline\hline
Parameter                        & Range & Unit \\\hline
$\mu_x$  &                      $[0.0, 2.0]$ & $\mathrm{cm}$     \\ 
$\mu_y$  &                      $[0.0, 2.0]$ & $\mathrm{cm}$    \\ % $\mathrm{rad~s^{-1}}$    \\ 
$\mu_z$ &                       $[0.0, 5.0]$ & $\mathrm{cm}$   \\ % $\mathrm{m~s^{-1}}$   \\ 
$\sigma_x$ &                    $[0.0, 1.0]$ & $\mathrm{cm}$   \\ 
$\sigma_y$        &             $[0.0, 1.0]$ & $\mathrm{cm}$    \\ % $\mathrm{m~s^{-2}}$    \\
$\sigma_z$  &                   $[0.0, 3.0]$ & $\mathrm{cm}$\\


\hline\hline
\end{tabular}
\end{center}
\vspace{-0.cm}
\end{table}


\paragraph{Sensor alignment bias}
We applied sensor alignment bias at the beginning of each episode to simulate extrinsic calibration error. This error included positional and rotational errors, i.e. $\begin{bmatrix} \Delta x, & \Delta y, & \Delta z, & \Delta \mathrm{roll}, & \Delta \mathrm{pitch}, & \Delta \mathrm{yaw} \end{bmatrix}$. The alignment errors were sampled from a uniform distribution and consistently applied to the measured points throughout the episode. The alignment bias parameters are summarized in Table~\ref{table:alignment_bias}.


% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\centering
\captionsetup{singlelinecheck=false}
\caption{Sensor alignment bias between the body frame of exteroceptive sensor and robot.}
\label{table:alignment_bias}

\begin{center}
\begin{tabular}{ccc}
\hline \hline
\multicolumn{1}{c}{Parameter} & Error range & Unit  \\\hline 
$\mathrm{roll}$             & $[-0.2, 0.2]$ &  $\mathrm{rad}$   \\
$\mathrm{pitch}$            & $[-0.15, 0.15]$ &  $\mathrm{rad}$   \\
$\mathrm{yaw}$              & $[-0.1, 0.1]$ &  $\mathrm{rad}$   \\
$\mathrm{x}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
$\mathrm{y}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
$\mathrm{z}$             & $[-0.1, 0.1]$ &  $\mathrm{m}$   \\
\hline \hline      
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

\paragraph{Pruning}
The major distinction between the height scans sampled in simulation and those obtained from real-world exteroceptive sensors is the presence of inherent blind spots in the latter. These blind spots can result from either the sensor's specifications or its placement on the robot, leading to occlusion by certain robot parts. One of the possible solutions to this problem is by employing raycasting from the sensor pose to the sampled height scan. However, this solution can be computationally expensive and greatly affect simulation time. In this work, we employed a simpler solution to eliminate or \textit{prune} parts of the exteroceptive data before it was fed into the multi-modal context encoder.

First, we construct a probability masking layer to prune the exteroceptive measurement that has been preprocessed using the method detailed in section~\ref{supp:exteroception_preprocessing}. During locomotion on the flat terrain, appropriately positioned exteroceptive sensors should effectively measure the terrain within a pre-defined grid area. However, the reliability of these measurements diminishes when the robot encounters obstacles or pits. To address this challenge, we introduced a probability masking technique that assigns a higher pruning probability to points that are distant and elevated or close and low to the robot. This pruning strategy makes a setting that allows the multi-modal context encoder to learn point completion from sparse exteroceptive inputs.

\subsubsection{\textit{Privileged states}}
For the privileged exteroception, we use a robot-centric local height map sampled around the robot. The local map is a 2.5D grid, where each value of the grid represents the height of the terrain on the corresponding grid. The grid is constructed with its row and column size of $w\!=\!1.1~\mathrm{m}$ and $h\!=\!1.7~\mathrm{m}$, respectively. The first row of the grid is located $0.9~\mathrm{m}$ in front of the robot's body frame, similar to the 3D voxel grid for the multi-modal encoder's input. The resolution of the grid is set to $5~\mathrm{cm}$.

For the privileged proprioception, we provide ground truth and noiseless measurements as follows:
\begin{enumerate}
    \item Gravity vector on the robot's body frame.
    \item Body linear and angular velocities.
    \item Joint positions and angular velocities.
    \item External disturbance force and torque applied to the robot's body frame.
    \item Physical properties (friction, motor damping, motor stiffness, motor strength ratio, additional payload, and the robot's center of mass).
    \item Foot position relative to the robot's body frame.
\end{enumerate}


\subsection{Reward functions}\label{supp:reward_functions}
Table~\ref{table:reward_functions} lists all the reward functions,~$\textbf{r}$, used in DreamWaQ++, which are mainly based on the rewards used in~\cite{nahrendra2023dreamwaq}. On top of these rewards, we also employed a reward curriculum to exponentially anneal some style rewards, i.e.~joint torque, joint velocity, joint acceleration, action rate, and smoothness rewards. The annealing rule follows the following formula:

\begin{equation}
    w_{i+1}=\lambda w_{i},
\end{equation}
where $w$ is the reward weight, $i$ is the learning iteration, and $\lambda$ is the annealing rate. We set $\lambda\!=0.998$
and $w_0$ for the selected skill rewards are summarized in Table~\ref{table:reward_init}.
% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable} 
\centering
\captionsetup{singlelinecheck=false}
\caption{Reward function elements and their corresponding weights. $\mathrm{exp(\cdot)}$ and $\mathrm{var(\cdot)}$ are exponential and variance operators, respectively. $(\cdot)^\mathrm{des}$ and $(\cdot)^\mathrm{cmd}$ indicate the desired and commanded values, respectively. $x, y,$ and $z$ are defined on the robot's body frame, with $x$ and $z$ pointing forward and upward, respectively. $\textbf{g}$, $\textbf{v}_{xy}$, $\omega_\mathrm{yaw}$, $h$, $p_{f,z,k}$, $v_{f,xy,k}$, and $\boldsymbol{\tau}$ are the gravity vector projected into the robot's body frame, linear velocity vector in the $xy$ plane, yaw rate, body height w.r.t. the ground, foot height, foot lateral velocity, and joint torque, respectively.}
\label{table:reward_functions}



\begin{center}
\begin{tabular}{lll}
\hline \hline
Reward           & Equation ($\textbf{r}$) & Weight ($w$) \\ \hline 
\multicolumn{3}{l} {\textit{Task rewards}}           \\ 
Lin. velocity tracking  & $\exp{\{-4(\textbf{v}^\mathrm{cmd}_{xy}-\textbf{v}_{xy})^{2}\}}$ & $1.0$      \\ 
Ang. velocity tracking & $\exp{\{-4(\omega^\mathrm{cmd}_\mathrm{yaw}-\omega_\mathrm{yaw})^{2}\}}$ & $0.5$ \\ \hline
\multicolumn{3}{l} {\textit{Style rewards}}           \\ 
Linear velocity ($z$) & $v^2_z$ & $-2.0$ \\
Angular velocity ($xy$) & $\boldsymbol{\omega}^2_{xy}$ & $-0.05$ \\
Uprightness & $|\textbf{g}|^2$ & $-0.2$ \\
Joint acceleration & $\boldsymbol{\ddot{\theta}}^2$ & $-2.5\!\times\!10^{-7}$ \\
Joint power & $|\boldsymbol{\tau}||\boldsymbol{\dot{\theta}}|$ & $-2\!\times\!10^{-5}$ \\
Body height & $(h^\text{des}-h)^2$ & $-1.0$ \\
Foot clearance & $(p^\text{des}_{f,z,k}-p_{f,z,k})^2\cdot v_{f,xy,k}$& $-0.01$ \\
Action rate & $(\textbf{a}_t - \textbf{a}_{t-1})^2$ & $-0.01$ \\
Smoothness & $(\textbf{a}_t - 2\textbf{a}_{t-1} + \textbf{a}_{t-2})^2$& $-0.01$ \\
Power distribution &$\mathrm{var}(\boldsymbol{\tau}\cdot\boldsymbol{\dot{\theta}})^2$ & $-10^{-5}$ \\ 
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================

% ===================================================================================
\begin{table}[t!]
% \begin{threeparttable}
\centering
\captionsetup{singlelinecheck=false}
\caption{Initial weight $w_0$ for selected style rewards that were annealed using the reward curriculum.}
\label{table:reward_init}



\begin{center}
\begin{tabular}{lll}
\hline \hline
Reward           & Weight ($w_0$)\\ \hline 
Joint torque & $-5\!\times\!10^{-6}$ \\
Joint velocity & $-6\!\times\!10^{-6}$ \\
Joint acceleration & $-7.5\!\times\!10^{-8}$ \\
Action rate & $-1.5\!\times\!10^{-5}$ \\
Smoothness & $-1.5\!\times\!10^{-5}$ \\
\hline \hline
\end{tabular}
\end{center}
\end{table}
% ===================================================================================


\subsection{Embedding analysis}\label{supp:embedding_analysis}
\subsubsection{Evaluation setting}
We conducted an embedding analysis on the context vector generated by the encoder. This analysis was carried out using data acquired within a simulation-to-simulation (sim-to-sim) setup. In this setup, both the fully trained encoder and policy networks were deployed within a Gazebo simulator. We implemented four distinct terrain types to facilitate this evaluation, as depicted in Fig.~\ref{figure:supp_gazebo_terrain}. In this setting, the stair difficulties are parameterized by its \textit{rise} and \textit{run}, i.e.~its vertical and horizontal dimensions, respectively~\cite{barasuolstair}. Easy stairs have low rise and high run values, while hard stairs have high rise and low run values.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/gazebo_terrain_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Illustrations of terrains used for evaluation in the Gazebo simulator.} Four types of terrains were constructed to evaluate the change in values of the context features. 
    % Four types of terrains were constructed to evaluate the changes in values of the context features. 
    The world model employed for this evaluation is an adapted version of the simulation model utilized in the IEEE ICRA 2023 Autonomous Quadrupedal Robot Challenge~\cite{jacoff2023taking}.}
	\label{figure:supp_gazebo_terrain}
\end{figure}

\subsubsection{Visualization via dimension reduction}
We performed dimensionality reduction on the proprioceptive, exteroceptive, and multi-modal contexts to depict their distributions within a 2D space. While one of the prevailing approaches for embedding visualization involves t-distributed stochastic neighbor embedding (t-SNE)~\cite{van2008visualizing}, it is worth noting that t-SNE, despite yielding satisfactory cluster visualizations, is notably less efficient at capturing overarching embedding structures. Its emphasis lies predominantly on local structures, potentially leading to inadequate comprehension of meaningful information within multi-modal data. Consequently, this limitation of t-SNE may hinder the comprehensive insights required for thorough analysis.

Hence, we extended our approach to dimensionality reduction by employing PaCMAP~\cite{wang2021understanding}, a recently introduced technique that offers a more balanced preservation of both local and global embedding structures. In this manner, we achieved visualizations of the embeddings within a 2D space for diverse terrains (as exemplified in Fig.~\ref{figure:supp_gazebo_terrain}). The visualization results are presented in Fig.~\ref{figure:supp_embedding_noblind}.


\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_noblind_embedding_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{2D visualization of the embeddings after dimensionality reduction.}}
	\label{figure:supp_embedding_noblind}
\end{figure}


As anticipated, the t-SNE method effectively portrays the exteroceptive context, revealing discernible clusters that imply the disentangled latent representation of different terrains. However, interpreting the proprioceptive context poses challenges in providing a coherent understanding. Consequently, the visualization of the multi-modal context fails to yield significant insights, aside from distant clusters indicative of varying terrains encoded in the exteroceptive context.

Meanwhile, PaCMAP more explicitly captures fundamental intrinsic characteristics of the embedding~\cite{wang2021understanding}. Within the proprioceptive context, PaCMAP effectively illustrates circular clusters, which plausibly correspond to the cyclic gait patterns exhibited by the robot's feet. An interesting observation arises as the circular radius expands on less challenging terrains. Our conjecture aligns with the notion that this radius could indicate the gait's duty cycle or swing time, as on smoother terrains without obstacles, the robot's feet undergo extended swing durations.

Our embedding analysis showcases that the structured representation learning facilitated by our context encoder yields informative latent variables without necessitating explicit estimation of physical attributes. As postulated by Nahrendra \textit{et al.}~\cite{nahrendra2023dreamwaq}, the unsupervised representation learning mechanism empowers the encoder to encode informative latent features while maintaining dynamic feature interactions selectively. The mechanism inherent in our context encoder thus amalgamates the best of both approaches, eliminating the requirement for manual and explicit selection of estimated variables while concurrently generating structured and disentangled latent representations.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_blind_embedding_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{2D visualization of the dimension-reduced embeddings during blind locomotion.}}
	\label{figure:supp_embedding_blind}
\end{figure}

We extended our embedding analysis to the blind locomotion scenario using our framework. In this assessment, we collected data by disabling exteroception, providing constant flat terrain points, and commanding the robot to walk across various terrains, as depicted in Fig.~\ref{figure:supp_embedding_blind}. The t-SNE visualization outcomes, while potentially sufficient for the policy network, remain less straightforward for practical interpretation. Such results could mislead practitioners into erroneously concluding that the encoder has not effectively learned a disentangled context vector.

In contrast, the PaCMAP visualization method successfully captures meaningful structures within the proprioceptive context. During blind locomotion, the proprioceptive context plays an important role because it remains the sole modality that the policy can rely on. As illustrated in Fig.~\ref{figure:supp_embedding_blind}, the proprioceptive context captures local structures induced by the robot's feet motions similar to the non-blind scenario. This distinctiveness becomes more discernible upon mixing into a multi-modal context, even when fused with the false exteroceptive context obtained in the blind locomotion scenario.

\subsubsection{Effect of contrastive loss}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_contrastive_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Effect of contrastive loss in the learned embedding.} The embeddings are recorded from locomotion on flat, irregular, easy stairs, and hard stairs terrains. The comparison shows the nature of the embedding when the contrastive loss is removed or retained.}
	\label{figure:supp_contrastive}
\end{figure}

We further investigated the impact of the contrastive loss on the learned embedding. The contrastive loss is a crucial component in training the multi-modal context encoder because it encourages the encoder to learn a structured representation. To evaluate the effect of the contrastive loss, we trained the encoder without the contrastive loss and compared the learned embeddings with those obtained from the full training setup using the contrastive loss. The results are depicted in Fig.~\ref{figure:supp_contrastive}.

The comparison showed that the contrastive loss significantly influences the learned embedding. The embeddings obtained from the full training setup exhibit more structured and disentangled latent variables than those obtained without contrastive loss. Indeed, some structured patterns in the embeddings are still discernible without the contrastive loss, mostly attributed to the exteroceptive data that provides spatial information. However, it fails to capture lower-level circular patterns in the proprioceptive data, which is crucial for the robot's locomotion. This observation underscores the importance of contrastive loss in the training of the multi-modal context encoder, as it facilitates the learning of structured and disentangled latent variables essential for the robot's locomotion.


\subsubsection{Attribution of latent variables}
\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_attribution_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Boxplot of each embedding variable in the multi-modal context vector.} The embeddings are recorded from locomotion on \textbf{(A)} flat, \textbf{(B)} irregular, \textbf{(C)} easy stairs, and \textbf{(D)} hard stairs terrains.}
	\label{figure:supp_embedding_attribution}
\end{figure}
We utilized boxplots to portray the raw embedding values, facilitating the analysis of their distribution as the robot navigates diverse terrains. The boxplot depicted in Fig.~\ref{figure:supp_embedding_attribution} reveals intriguing trends within the exteroceptive context. Particularly noteworthy are four embedding variables ($41$, $42$, $55$, and $64$th embeddings) exhibiting significantly expansive distributions. We posit that these characteristics are closely tied to the robot's foot motion while traversing terrains of varying complexities. To substantiate this hypothesis, we conducted an experiment involving scaling these four embedding variables before being fed to the policy network. This scaling operation involved adjustments of $0.1$ and $3.0$ times their original values to investigate the effect that it may bring to the robot's foot motions.


\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/latent_modulation_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Latent modulation on some of the exteroceptive embedding proportionally affects the gait height.} The robot exhibits different locomotion styles when particular latent variables ($41$, $42$, $55$, and $64$th embeddings) were scaled with (\textbf{A}) $0.1$, (\textbf{B}) $1.0$, and (\textbf{C}) $3.0$ times of its original value. The difference resulted from this modulation is observable from the FR foot's $z$ position w.r.t. the base as shown in Fig.~\ref{figure:results_terrain}C.}
	\label{figure:supp_latent_modulation}
\end{figure}

This discovery shown in Fig.~\ref{figure:supp_latent_modulation} emphatically underscores the efficacy of structured representation learning, wherein essential physical attributes are embodied via an unsupervised approach. Moreover, this behavior offers a novel insight into the realm of interpretable learning-based control, countering the conventional notion of modern deep reinforcement learning as a ``black box'' system devoid of user-accessible modulations. Our findings demonstrate that structured representation learning engenders the acquisition of structured embeddings that can be flexibly modulated, enabling the generation of diverse behaviors by manipulating the intermediate embedding variables. This property opens up compelling possibilities for bridging the gap between learned locomotion controllers and their model-based counterparts. It also enables intuitive tuning by a human operator or a higher-level planner. 

Importantly, this property naturally emerged and was not explicitly specified during training or in the input command for the controller, distinguishing our work from that of Margolis~\textit{et al}.~\cite{margolis2022walk} that explicitly gives a style command into the policy network. Instead, this interpretable latent structure arose from the structured representation learning facilitated by the multi-modal context encoder within the proposed framework. 

However, we note that while the observed trend remains consistent, the indices of the modulated latent and its scale consistently change with different training seeds. This variability is expected because we do not enforce the learning of these variables in a supervised manner. 

% Instead, these variables are acquired through an unsupervised yet structured learning framework of the multi-modal context encoder, which enables the discovery of interpretable latent variables.

\subsubsection{Embedding feature-wise cross-correlation}
The heatmap plots shown in Fig.~\ref{figure:results_terrain}D underscore the efficiency of the multi-modal context encoder, which dynamically encodes multi-modal perception without any bias toward a particular modality. The multi-modal context encoder adaptively shifts its attention to modalities that provide the most informative priors for the policy. Furthermore, the notion of cross-modal correlation introduces interpretability on the uncertainties faced by the context encoder. This uncertainty measurement is particularly beneficial for higher-level modules. For instance, the uncertainty measurement can be leveraged by a traversability mapping module to adaptively shift its reliance on different sensor modalities for map update.


\subsection{Sensor--agnostic deployment}\label{supp:sensor_agnostic}
A fundamental strength of the policy trained using DreamWaQ++ is its sensor-agnostic property. The policy and context encoder were jointly trained in the simulation without any specific sensor model but only leveraged 3D points scan in front of the robot. Hence, the learned networks can be deployed on the real robot without any further training procedure. The only calibration required is the extrinsic parameters that transform 3D points from the sensor to the robot's body frame. This approach makes our method more simple and efficient than other existing works that rely on distilling a teacher policy into a student policy to bridge the gap between simulation and real-world exteroception. Furthermore, given that the context encoder was trained using 3D points as its input, it does not require any assumption on the number of points or grids. Instead, it will learn to infer the reliability of the exteroception and construct an informative latent feature for the policy. 

We performed an experiment using robot R3 to verify the adaptability of the learned controller to different sensor configurations. In this experiment, we built a local map surrounding the robot because we had access to stronger computation power, as well as an onboard LiDAR sensor on robot~R3. We constructed a local map of size $1.7\;\mathrm{m}\times1.1\;\mathrm{m}$ with a $0.1\;\mathrm{m}$ resolution. 

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_sensor_agnostic_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Sensor agnostic deployment.} (\textbf{A}) Adaptability of the perception networks in different exteroceptive data settings. Despite the controller being trained solely with front-facing points, as depicted in Fig.~\ref{figure:dreamwaqpp}, it demonstrates adaptability to 3D point inputs that encompass the robot (illustrated with red points). The reconstruction of these points (represented by blue points) accurately captures the geometric properties of the robot's surroundings.} (\textbf{B})~A real-world stair-climbing experiment, which validates the adaptability of the controller when different exteroceptive configurations are used for the controller.
	\label{figure:supp_sensor_agnostic}
\end{figure}

\figinitref{figure:supp_sensor_agnostic}A shows the local map input (red dots) and its reconstruction (blue dots). Despite never trained with such exteroceptive setting, the encoder and decoder networks can still reconstruct the map with a satisfactory accuracy. The adaptability of the controller was further verified through a stair-climbing experiment in Fig.~\ref{figure:supp_sensor_agnostic}B. The robot can resiliently climb the stairs and by utilizing a wider, yet sparse exteroceptive information, which has never been encountered during training.

\subsection{Details of hierarchical memory}\label{supp:hierarchical_memory}
The closest approach to our hierarchical memory approach is the neural scene representation method~\cite{hoeller2022neural}, where the robot's local map is reconstructed by introducing an autoregressive structure for predicting and generating the 3D reconstruction of the local map. The neural scene representation network receives the robot frame's transformation from a separate odometry module, current measured points, and previous 3D reconstruction. The key difference in our method is that we employed autoregression solely for explicit estimation of the $SE(3)$ transformation of the body frame of the robot over time. Our proposed method does not require a complex reconstruction method with high capacity network, but still able to provide a temporally dense exteroception.

This estimated transformation is then utilized to transform the last observed points into the robot's current frame. The $SE(3)$ transformation is available at each control loop iteration via the state estimation network, enabling temporal interpolation of the latest exteroceptive measurements. This interpolation forms the basis of a memory structure, which is subsequently fed into the exteroceptive encoder. The exteroceptive observation is formally defined as

\begin{equation}
  \textbf{o}^{\mathrm{e},K}_t = \textbf{o}^\mathrm{e}_t \concat \hat{\textbf{o}}^\mathrm{e}_{t-1} \concat \cdots \concat \hat{\textbf{o}}^\mathrm{e}_{t-K}, 
\end{equation}
 where $\textbf{o}^\mathrm{e}_t$ is the most recent exteroceptive observation at time $t$. $\hat{\textbf{o}}^\mathrm{e}_{t-K}$ is the previous exteroceptive observation at $t-K$, which has been transformed to the robot's body frame at time $t$, which is defined as
\begin{equation}
  \hat{\textbf{o}}^\mathrm{e}_{t-K} = \prescript{t}{t-K}{T}^{-1}\cdot \textbf{o}^\mathrm{e}_{t-K},
\end{equation}
where $\textbf{o}^\mathrm{e}_{t-K}$ is the exteroceptive observation measured at time $t-K$, and $\prescript{t}{t-K}{T}$ is the $SE(3)$ transformation of the robot's pose from time $t$ to $t-K$. 
% 

% By doing so, our approach yields a lightweight architecture that retains some memory of the exteroceptions without necessitating memory-based networks.

\subsection{Scalability to other platforms}\label{supp:scalability}
We assessed the scalability of DreamWaQ++ with applications to legged robots with various morphologies and sizes. We used DreamWaQ++ to train a controller for an ANYmal-C~\cite{hutter2016anymal} and Hound~\cite{shin2022design} robots. Note that we used the same rewards and its corresponding weights as in supplementary section~\ref{supp:reward_functions} and only changed the robot's model as well as their motor's stiffness and damping parameter. A compilation of these robots navigating over stairs is provided in \mvseven. 

\figinitref{figure:supp_multi_robot} shows the success rates of three different robots on climbing stairs with various runs and rises. For the Go1 robot, we used a run value of $0.3~\mathrm{m}$ and $0.6~\mathrm{m}$, while for ANYmal-C and Hound, we used a run value of $0.6~\mathrm{m}$ and $1.0~\mathrm{m}$ to accommodate for their long trunk size. The success rates are measured from $1,\!000$ simulated robots, which is defined as the percentage of the number of robots that can reach the last stair within $10~\mathrm{s}$ over the total number of robots.
% , where a success is defined as when the robot can reach the last stairs within $10~\mathrm{s}$.

As expected, the large joint operation range of Hound enabled it to traverse more difficult terrains compared with the Go1 and ANYmal-C robot, allowing it to traverse up to $42~\mathrm{cm}$-high stairs with an $80\%$ success rate. It is also noteworthy that during training, the robots are faced only with a maximum obstacle height of $27~\mathrm{cm}$, and this result highlights the strong adaptability of the controller trained with DreamWaQ++. Thanks to the explorative behavior during training, DreamWaQ++ also maximizes the hardware's capability and the reward functions are invariant to the hardware variations.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_multirobot_success.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Success rates for climbing different obstacles using various quadrupedal robots.} We trained DreamWaQ++ for \textbf{(A)} Unitree Go1, \textbf{(B)} ANYmal-C, and \textbf{(C)} Hound. The maximum stair rise imposed during training for all robots is $27~\mathrm{cm}$.}
	\label{figure:supp_multi_robot}
\end{figure}



This evaluation successfully highlights the versatility of DreamWaQ++ for its applications to various legged robots. Although deep RL algorithms are notoriously sensitive to reward parameters for different robots, we discovered that DreamWaQ++ can be easily adopted to different platforms with no further tuning effort. 

\subsection{Learning to overcome large obstacles}\label{supp:parkour}
Recently, there has been a growing interest in training quadrupedal robots for more complex tasks such as jumping and leaping~\cite{hoeller2023anymal,zhuang2023robot}. These skills require the quadruped robot to maximize its actuator limit and orchestrate highly-agile motions. We further assessed the scalability of DreamWaQ++ in learning a skill required for overcoming obstacles that are higher than the robot. We trained the Go1, ANYmal-C, and Hound robots in an environment with extreme obstacle heights, reaching up to $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, and $1.5~\mathrm{m}$, respectively. To allow learning of such an agile skill, we need to do some modifications, i.e., 1) relaxing the velocity tracking reward scale from $1.0$ to $0.1$, and 2) increasing the versatility gain scaling in the total loss function from $0.1$ to $0.2$. A snapshot of the learned obstacle climbing motion in simulation and the real world is shown in Fig.~\ref{figure:supp_parkour_sim} and \\mveight.

We found that the two modifications are complimentary. Relaxing the velocity tracking reward without scaling up the versatility gain ends up with a policy that resists moving forward. On the other hand, doubling the versatility gain without relaxing the velocity tracking reward results in a policy that moves forward but with a conservative gait due to lack of skill discovery. This modification allowed the policy to learn more flexible gaits, yielding higher agility for accomplishing more complex tasks such as parkour.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_parkour_sim_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Demonstration of a learned parkour skills in simulation.} We trained DreamWaQ++ for \textbf{(A)}~Unitree Go1, \textbf{(B)}~ANYmal-C, and \textbf{(C)}~Hound to climb obstacles with a height of $0.6~\mathrm{m}$, $1.0~\mathrm{m}$, $1.5~\mathrm{m}$, respectively. \textbf{(D)}~A real world experiment was conducted using a Go1 robot with a $2.5~\mathrm{kg}$ payload on top of it.}
	\label{figure:supp_parkour_sim}
\end{figure}

The results in Fig.~\ref{figure:supp_parkour_sim} illustrate how controllers on different robots produce distinct motions when overcoming large obstacles. In Fig.~\ref{figure:supp_parkour_sim}A, Go1 utilizes a jumping motion to overcome the obstacle, given its small posture. In contrast, ANYmal-C employs its front legs to establish initial contacts with the wall of the obstacle (Fig.~\ref{figure:supp_parkour_sim}B-2) and then uses those legs as anchors to climb (Fig.~\ref{figure:supp_parkour_sim}B-3). Thanks to its large allowable joint positions and torque operation limits, ANYmal-C can climb obstacles as high as $1.5~\mathrm{m}$. Hound, on the other hand, firstly swings its right front leg widely and places it on top of the obstacle as an anchor. Subsequently, it uses its rear legs to propel its body upward (Fig.~\ref{figure:supp_parkour_sim}C-4) and successfully reaches the top of the obstacles.

The real-world experiment in Fig.~\ref{figure:supp_parkour_sim}D was conducted to validate the sim-to-real robustness of the learned controller. Utilizing a Go1 robot with an additional $2.5\mathrm{kg}$ payload, the controller successfully enables the robot to climb a $41~\mathrm{cm}$ obstacle. Notably, the obstacle is a soft sofa block, representing a deformable surface not encountered during training.



% \subsection{Extreme terrain retraining}\label{supp:extreme}
% We further evaluate the versatility of DreamWaQ++ in a more challenging training setting. We fine-tuned the learned controller in a new training setting, consisting of extremely challenging terrains that can push the limit of the robot's physical capabilities, such as large gaps and high stages.

\subsection{Ablation of backbone sequence model}\label{supp:model_ablation}
We conducted an ablation study to evaluate the impact of the backbone sequence model on the controller's performance. We compared the performance of the controller with and with different sequence models by measuring the accuracy of future joint position prediction. The results are shown in Fig.~\ref{figure:supp_nextstate}.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_nextstate_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Future state error comparison.} The comparison shows the future state prediction error using different models and varying robot velocities.}
	\label{figure:supp_nextstate}
\end{figure}

The results in Fig.~\ref{figure:supp_nextstate} show that the proposed MLP-mixer architecture model works as well as the Transformer model. The advantage of using the MLP mixer is that it is more lightweight and computationally efficient than the Transformer model. From the curve, we can see that the prediction error increases as the robot's velocity increases. This is because the robot's motion becomes more dynamic and the model has to predict the future state more accurately.

\subsection{Terrain reconstruction}\label{supp:recons}
We decoded the latent features from the context encoder recorded in the asynchronous stair race experiment to reconstruct the terrain map. The reconstructed terrain map is shown in Fig.~\ref{figure:supp_recons} and \mvone0. The reconstructed terrain map resembles the ground truth terrain map constructed using~\cite{oh2024trip}.

However, note that the reconstructed terrain map is not as accurate as the ground truth terrain map due to three reasons: 
\begin{enumerate}
	\item The robot's exteroception is limited to the front-facing 3D points, and the memory retained by the encoder is not a long term memory.
	\item The encoder-decoder structure does not use a residual connection, similar to~\cite{hoeller2023anymal} to allow learning of only relevant features to the latent representation.
	\item The regularization in the latent space using a variational autoencoder is expected to reduce the reconstruction accuracy while improving disentanglement of the latent features. 
\end{enumerate}
Nevertheless, a slight reduction in the reconstruction accuracy is acceptable because the primary goal of the context encoder is to learn a structured representation that can be used for control, rather than to reconstruct the complete terrain map accurately.

\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.48\textwidth}
		\includegraphics[width=1.0\textwidth]{figures/supp/supp_recons_red.pdf}
	\end{subfigure}
	% \captionsetup{font=footnotesize}
	\caption{\textbf{Reconstructed terrain map.} The terrain map is reconstructed from the latent features recorded during the asynchronous stair race using DreamWaQ++. The ground truth terrain map is constructed using~\cite{oh2024trip}. The white points are the forward 3D scan input, while the reconstruction points surrounding the robots are colored based on the height relative to the robot's base.}
	\label{figure:supp_recons}
\end{figure}


